The Next Generation Virgo Cluster Survey (NGVS). III. A Catalog of Surface Brightness Fluctuation Distances and the Three-Dimensional Distribution of Galaxies in the Virgo Cluster

The surface brightness fluctuation (SBF) method is a robust and efficient way of measuring distances to galaxies containing evolved stellar populations. Although many recent applications of the method have used space-based imaging, SBF remains a powerful technique for ground-based telescopes. Deep, wide-field imaging surveys with subarsecond seeing enable SBF measurements for numerous nearby galaxies. Using a preliminary calibration, Cantiello et al. (2018) presented SBF distances for 89 bright, mainly early-type galaxies observed in the Next Generation Virgo Cluster Survey (NGVS). Here, we present a refined calibration and SBF distances for 278 galaxies extending several magnitudes fainter than in previous work. The derived distances have uncertainties of 5-12\% depending on the properties of the individual galaxies, and our sample is more than three times larger than any previous SBF study of this region. Virgo has a famously complex structure with numerous subclusters, clouds and groups; we associate individual galaxies with the various substructures and map their three-dimensional spatial distribution. Curiously, subcluster A, centered around M87, appears to have two peaks in distance: the main peak at $\sim$16.5 Mpc and a smaller one at $\sim$19.4 Mpc. Subclusters B and C have distances of $\sim$15.8 Mpc. The W and W' groups form a filament-like structure, extending more than 15~Mpc behind the cluster with a commensurate velocity increase of $\sim$1000 \kms\ along its length. These measurements are a valuable resource for future studies of the relationship between galaxy properties and local environment within a dynamic and evolving region.

==> Tables/tab_clouds.tex <==
\begin{deluxetable*}{lcccccc}
  \label{tab_clouds}
  \tablecaption{Main characteristics of the  Virgo cluster substructures inspected.} 
\tablewidth{0pt}
\tablehead{
\colhead{Structure} & \colhead{R.A. (J2000)} & \colhead{Dec. (J2000)} & \colhead{Radius (deg)} & \colhead{$N_\mathrm{sel}$} & \colhead{$\langle d \rangle$ (Mpc)} & \colhead{$rms$ (Mpc)}}
\startdata
Cluster A (M\,87) & 187.7 & 12.4 & 2.7 & 113 & 16.9 & 1.2 \\
Cluster B (M\,49) & 187.4 &  8.0 & 1.7 & 16 & 15.9 & 0.9 \\
Cluster C (M\,60) & 190.9 & 11.4 & 0.7 & 9 & 15.9 & 1.2 \\
\Wprime~cloud     & 185.7 & 7.2   & 1.4 & 9 & 22.8 & 4.1 \\
W  cloud          & 184.5 &  6.5   & 1.2 & 7 & 29.2 & 2.4 \\
Low Velocity cloud & 184.0 & 13.4 & 1.5 & 3   & 16.0 & 1.2 \\
M cloud            & 183.0 & 13.4 & 1.5 & 1  & 32.5  & \nodata \\
\enddata
\end{deluxetable*}


==> Tables/table1_ref.tex <==
\begin{sidewaystable*}
\vspace{-9cm}
\startlongtable
\begin{deluxetable}{llcccccccccccccccc}
%\tabletypesize{\footnotesize}
\tabletypesize{\scriptsize}
\tablecaption{Sample basic properties, colors, SBF and distances (Excerpt)}
\tablehead{
  \colhead{VCC} &
  \colhead{Alt. Name} &
  \colhead{RA (J2000)} &
  \colhead{Dec (J2000)} &
  \colhead{$B_T$} &
  \colhead{\tiny{$E(B{-}V)$}} &
  \colhead{$v_{Helio}$} &
  \colhead{$T_{Type}$} &
  \colhead{\uz} &
  \colhead{\gi} &
  \colhead{\gz} &
  \colhead{$\overline{m_i}$} &
  \colhead{Flag} &
  \colhead{$(m{-}M)_{Ref}$} &
  \colhead{\dref} &
  \colhead{\dmean} &
  \colhead{Area} &
  \colhead{$\langle Rad\rangle$} 
  \\
  \colhead{   } &
  \colhead{         } &
  \colhead{   (deg)  } &
  \colhead{  (deg)    } &
  \colhead{(mag)} &
  \colhead{ (mag)           } &
  \colhead{\kms       } &
  \colhead{          } &
  \colhead{(mag) } &
  \colhead{(mag)} &
  \colhead{(mag)} &
  \colhead{ (mag)          } &
  \colhead{} &
  \colhead{      (mag)                      } &
  \colhead{ (Mpc)    } &
  \colhead{ (Mpc)    } &
  \colhead{\tiny{(arcmin$^2$)}} &
  \colhead{ (arcsec)    } 
  } \startdata
      (1)&   (2)      &     (3)      &        (4)   &    (5)   &  (6)   &    (7)  &      (8)     &      (9)           &            (10)   &    (11)           & (12)              &  (13)  &   (14)           &  (15)           & (16)            & (17) & (18)   \\   
\hline
      32 & IC0767     &  182.7613724 &   12.1039918 &    14.00 &  0.027 &    1877 &   -5.0 (  1.0) &    2.152 ( 0.031) &    0.801 ( 0.008) &    1.009 ( 0.031) &   29.788 ( 0.057) &     B  &   31.162 ( 0.113) &    17.08 ( 0.89) &    17.34 ( 1.04)  &  0.85 & 23.80  \\
      33 & IC3032     &  182.7823394 &   14.2748006 &    14.70 &  0.038 &    1179 &   -4.0 (  1.8) &    2.140 ( 0.038) &    0.819 ( 0.010) &    0.991 ( 0.038) &   29.489 ( 0.143) &     A  &   30.910 ( 0.179) &    15.20 ( 1.25) &    15.17 ( 1.31)  &  1.34 & 27.40  \\
      49 & NGC4168    &  183.0719332 &   13.2051960 &    12.20 &  0.037 &    2273 &   -4.9 (  0.4) &    2.623 ( 0.007) &    0.983 ( 0.002) &    1.214 ( 0.007) &   31.628 ( 0.102) &     B  &   32.681 ( 0.129) &    34.37 ( 2.05) &    33.50 ( 2.33)  &  4.11 & 51.50  \\
      66 & NGC4178    &  183.1940241 &   10.8666242 &    11.90 &  0.028 &     374 &    6.9 (  1.2) &    1.032 ( 0.270) &    0.374 ( 0.046) &    0.125 ( 0.269) &   28.583 ( 0.162) &     C  &   33.422 ( 2.877) &    48.36 (64.13) &    25.36 (19.59)  &  0.73 & 60.70  \\
      89 & NGC4189    &  183.4468247 &   13.4248521 &    12.50 &  0.033 &    2098 &    5.9 (  0.9) &    2.011 ( 0.069) &    0.768 ( 0.020) &    0.978 ( 0.069) &   31.004 ( 0.363) &     C  &   32.437 ( 0.394) &    30.72 ( 5.58) &    31.75 ( 5.71)  &  0.36 & 63.60  \\
      92 & NGC4192    &  183.4512262 &   14.9005060 &    10.90 &  0.035 &    -142 &    2.6 (  0.8) &  \nodata          &    0.908 ( 0.017) &    1.190 ( 0.061) &   29.931 ( 0.163) &     C  &   31.024 ( 0.211) &    16.02 ( 1.56) &    16.61 ( 1.71)  &  0.78 & 78.60  \\
     107 & PGC039071  &  183.5406147 &   13.2334632 &    19.40 &  0.030 & \nodata &   -5.0 (  2.0) &    1.768 ( 0.147) &    0.707 ( 0.036) &    0.753 ( 0.145) &   29.158 ( 0.375) &     C  &   30.984 ( 0.549) &    15.73 ( 3.98) &    14.88 ( 3.12)  &  0.03 &  3.80  \\
     140 & IC3065     &  183.8023507 &   14.4328799 &    14.30 &  0.036 &     995 &   -2.2 (  1.2) &    2.270 ( 0.014) &    0.924 ( 0.004) &    1.120 ( 0.014) &   29.934 ( 0.093) &     A  &   31.150 ( 0.124) &    16.98 ( 0.97) &    17.29 ( 1.16)  &  1.31 & 27.20  \\
     145 & NGC4206    &  183.8200770 &   13.0239966 &    12.80 &  0.032 &     703 &    4.0 (  0.3) &    1.430 ( 0.535) &    0.791 ( 0.203) &    0.729 ( 0.533) &   28.557 ( 1.563) &     C  &   30.442 ( 2.195) &    12.26 (12.41) &    12.05 (10.28)  &  0.39 & 42.70  \\
     157 & NGC4212    &  183.9138976 &   13.9015055 &    11.90 &  0.033 &     -88 &    4.9 (  0.8) &    1.802 ( 0.071) &    0.764 ( 0.017) &    0.966 ( 0.071) &   30.066 ( 0.136) &     C  &   31.517 ( 0.208) &    20.11 ( 1.93) &    21.61 ( 1.96)  &  0.85 & 67.10  \\
     167 & NGC4216    &  183.9766077 &   13.1494566 &    11.00 &  0.032 &     131 &    3.0 (  0.5) &    2.501 ( 0.030) &    0.999 ( 0.013) &    1.234 ( 0.029) &   30.303 ( 0.227) &     B  &   31.304 ( 0.246) &    18.23 ( 2.07) &    18.53 ( 2.19)  &  1.05 & 59.20  \\
     199 & NGC4224    &  184.1407813 &    7.4620674 &    12.90 &  0.024 &    2584 &    1.0 (  0.3) &    2.568 ( 0.012) &    0.989 ( 0.005) &    1.211 ( 0.010) &   30.761 ( 0.082) &     B  &   31.786 ( 0.115) &    22.76 ( 1.21) &    22.43 ( 1.43)  &  0.38 & 31.20  \\
     200 & PGC039331  &  184.1404477 &   13.0315970 &    14.70 &  0.030 &       8 &   -4.3 (  1.6) &    2.328 ( 0.033) &    0.854 ( 0.014) &    1.073 ( 0.032) &   29.815 ( 0.169) &     A  &   31.095 ( 0.195) &    16.56 ( 1.49) &    16.58 ( 1.58)  &  1.36 & 27.50  \\
     220 & NGC4233    &  184.2820056 &    7.6242759 &    13.00 &  0.024 &    2275 &   -2.0 (  0.5) &    2.737 ( 0.008) &    1.033 ( 0.004) &    1.302 ( 0.007) &   31.751 ( 0.145) &     B  &   32.575 ( 0.165) &    32.74 ( 2.50) &    32.43 ( 2.74)  &  1.02 & 32.90  \\
     222 & NGC4235    &  184.2911844 &    7.1915747 &    12.70 &  0.019 &    2263 &    1.0 (  0.4) &    2.545 ( 0.015) &    0.965 ( 0.006) &    1.209 ( 0.012) &   31.233 ( 0.122) &     B  &   32.245 ( 0.147) &    28.12 ( 1.91) &    28.21 ( 2.17)  &  0.37 & 28.00  \\
     226 & NGC4237    &  184.2976068 &   15.3240384 &    12.50 &  0.030 &     864 &    4.0 (  0.5) &    2.171 ( 0.042) &    0.816 ( 0.012) &    1.069 ( 0.041) &   30.040 ( 0.107) &     B  &   31.326 ( 0.152) &    18.42 ( 1.29) &    19.26 ( 1.44)  &  0.64 & 54.50  \\
     230 & IC3101     &  184.3318761 &   11.9434644 &    15.20 &  0.028 &    1430 &   -5.0 (  1.4) &    2.267 ( 0.014) &    0.875 ( 0.007) &    1.064 ( 0.014) &   30.167 ( 0.158) &     A  &   31.457 ( 0.178) &    19.56 ( 1.60) &    19.58 ( 1.76)  &  0.27 & 12.70  \\
     263 & PGC039475  &  184.4868025 &   11.9960324 &    18.20 &  0.030 &\nodata  &   -5.0 (  3.0) &    1.969 ( 0.026) &    0.784 ( 0.014) &    0.892 ( 0.024) &   29.498 ( 0.402) &     B  &   31.063 ( 0.413) &    16.31 ( 3.10) &    16.00 ( 3.09)  &  0.02 &  3.90  \\
     308 & IC3131     &  184.7120270 &    7.8619797 &    13.70 &  0.021 &    1530 &   -3.5 (  1.8) &    2.218 ( 0.013) &    0.859 ( 0.007) &    1.036 ( 0.012) &   29.875 ( 0.169) &     B  &   31.196 ( 0.187) &    17.34 ( 1.50) &    17.36 ( 1.63)  &  1.64 & 30.10  \\
     315 & PGC039606  &  184.7523115 &    6.0946187 &    14.80 &  0.023 &    1589 &    0.5 (  1.0) &  \nodata          &    0.935 ( 0.004) &    1.157 ( 0.023) &   31.462 ( 0.097) &     B  &   32.587 ( 0.131) &    32.92 ( 1.99) &    33.11 ( 2.43)  &  0.19 & 13.90  \\
     341 & NGC4260    &  184.8427241 &    6.0986724 &    12.70 &  0.023 &    1776 &    1.0 (  0.5) &    2.632 ( 0.027) &    1.002 ( 0.004) &    1.266 ( 0.025) &   31.315 ( 0.122) &     B  &   32.222 ( 0.152) &    27.83 ( 1.95) &    28.04 ( 2.17)  &  0.64 & 39.60  \\
     345 & NGC4261    &  184.8467458 &    5.8248971 &    11.30 &  0.018 &    2177 &   -4.8 (  0.4) &    2.796 ( 0.007) &    1.075 ( 0.001) &    1.378 ( 0.007) &   31.718 ( 0.136) &     B  &   32.309 ( 0.158) &    28.96 ( 2.11) &    29.75 ( 2.42)  &  6.18 & 64.30  \\
     355 & NGC4262    &  184.8773845 &   14.8776534 &    12.40 &  0.036 &    1359 &   -2.6 (  0.7) &    2.667 ( 0.009) &    1.013 ( 0.003) &    1.281 ( 0.008) &   29.874 ( 0.060) &     A  &   30.790 ( 0.100) &    14.39 ( 0.66) &    14.43 ( 0.84)  &  0.48 & 33.00  \\
     369 & NGC4267    &  184.9386693 &   12.7982620 &    11.80 &  0.047 &    1021 &   -2.7 (  0.7) &    2.815 ( 0.005) &    1.106 ( 0.002) &    1.346 ( 0.005) &   30.316 ( 0.051) &     A  &   31.122 ( 0.094) &    16.76 ( 0.73) &    16.08 ( 0.89)  &  2.96 & 45.40  \\
     397 & PGC039772  &  185.0507418 &    6.6231923 &    14.90 &  0.019 &    2442 &   -5.0 (  1.2) &    2.406 ( 0.009) &    0.899 ( 0.002) &    1.111 ( 0.008) &   31.201 ( 0.085) &     B  &   32.397 ( 0.117) &    30.16 ( 1.62) &    29.96 ( 1.94)  &  0.10 &  7.70  \\
     465 & NGC4294    &  185.3243502 &   11.5106643 &    12.60 &  0.034 &     355 &    5.9 (  0.5) &    1.682 ( 0.048) &    0.662 ( 0.026) &    0.837 ( 0.046) &   29.424 ( 0.143) &     B  &   31.094 ( 0.196) &    16.55 ( 1.50) &    17.31 ( 1.63)  &  0.39 & 44.30  \\
     483 & NGC4298    &  185.3865368 &   14.6061371 &    12.10 &  0.035 &    1124 &    5.1 (  0.6) &    2.183 ( 0.036) &    0.749 ( 0.014) &    0.978 ( 0.035) &   29.586 ( 0.088) &     B  &   31.023 ( 0.136) &    16.02 ( 1.01) &    16.10 ( 1.12)  &  1.26 & 64.60  \\
     490 & IC0783     &  185.4115379 &   15.7451112 &    13.40 &  0.022 &    1267 &   -0.2 (  0.8) &    2.345 ( 0.030) &    0.877 ( 0.007) &    1.086 ( 0.029) &   29.866 ( 0.107) &     B  &   31.108 ( 0.142) &    16.66 ( 1.09) &    16.65 ( 1.21)  &  2.85 & 39.90  \\
     491 & NGC4299    &  185.4180145 &   11.5031588 &    12.90 &  0.033 &     237 &    8.4 (  1.3) &    1.725 ( 0.042) &    0.632 ( 0.019) &    0.749 ( 0.041) &   29.624 ( 0.236) &     B  &   31.469 ( 0.274) &    19.67 ( 2.48) &    19.19 ( 2.43)  &  0.62 & 53.20  \\
     497 & NGC4302    &  185.4266475 &   14.5949500 &    12.60 &  0.035 &    1098 &    5.3 (  0.8) &    2.276 ( 0.041) &    0.898 ( 0.014) &    1.080 ( 0.039) &   29.641 ( 0.168) &     B  &   30.919 ( 0.198) &    15.27 ( 1.40) &    15.28 ( 1.46)  &  1.11 & 44.00 
 \\
\enddata
\end{deluxetable}
\label{tab_all}
\tablecomments{This table is available in its entirety in a machine-readable form in the online journal. A portion is shown here for guidance regarding its form and content. All magnitudes are in $AB$ mag.}
\end{sidewaystable*}




==> Tables/table_measures_ref_full_v2.tex <==
\begin{deluxetable*}{llcccccccccccccccc}
%\tabletypesize{\footnotesize}
\tabletypesize{\scriptsize}
\tablecaption{SBF, colors and distances for the 278 galaxies in our sample}
\tablehead{
  \colhead{VCC} &
  \colhead{\uz} &
  \colhead{\gi} &
  \colhead{\gz} &
  \colhead{$\overline{m}_i$} &
  \colhead{\mMbarref} &
  \colhead{\dref} &
  \colhead{\dmean} &
  \colhead{Area} &
  \colhead{$\langle Rad\rangle$} &
  \colhead{Flag} 
  \\
  \colhead{   } &
  \colhead{(mag) } &
  \colhead{(mag)} &
  \colhead{(mag)} &
  \colhead{ (mag)          } &
  \colhead{      (mag)                      } &
  \colhead{ (Mpc)    } &
  \colhead{ (Mpc)    } &
  \colhead{(arcmin$^2$)} &
  \colhead{ (arcsec)    } &
   \colhead{} 
 } \startdata
      (1)&   (2)      &     (3)      &        (4)   &    (5)   &  (6)   &    (7)  &      (8)     &      (9)           &            (10)   &    (11)           \\   
\hline
      32 &    2.152 ( 0.031) &    0.801 ( 0.008) &    1.009 ( 0.031) &   29.788 ( 0.057) &   31.133 ( 0.091) &    16.85 ( 0.71) &    16.95 ( 0.90)  &  0.85 & 23.8  &	q2   \\
      33 &    2.140 ( 0.038) &    0.819 ( 0.010) &    0.991 ( 0.038) &   29.489 ( 0.143) &   30.855 ( 0.162) &    14.82 ( 1.11) &    14.85 ( 1.22)  &  1.34 & 27.4  &	q1   \\
      49 &    2.623 ( 0.007) &    0.983 ( 0.002) &    1.214 ( 0.007) &   31.628 ( 0.102) &   32.539 ( 0.128) &    32.20 ( 1.90) &    32.92 ( 1.83)  &  4.11 & 51.5  &	q2   \\
      66 &    1.032 ( 0.270) &    0.374 ( 0.046) &    0.125 ( 0.269) &   28.583 ( 0.162) &   31.405 ( 0.814) &    19.10 ( 7.17) &    19.40 ( 6.23)  &  0.73 & 60.7  &	q3   \\
      89 &    2.011 ( 0.069) &    0.768 ( 0.020) &    0.978 ( 0.069) &   31.004 ( 0.363) &   32.475 ( 0.376) &    31.26 ( 5.42) &    31.37 ( 5.51)  &  0.36 & 63.6  &	q3   \\
      92 &    \nodata        &    0.908 ( 0.017) &    1.190 ( 0.061) &   29.931 ( 0.163) &   31.056 ( 0.203) &    16.26 ( 1.52) &    16.26 ( 1.52)  &  0.78 & 78.6  &	q3   \\
     107 &    1.768 ( 0.147) &    0.707 ( 0.036) &    0.753 ( 0.145) &   29.158 ( 0.375) &   30.848 ( 0.424) &    14.78 ( 2.89) &    14.49 ( 2.82)  &  0.03 &  3.8  &	q3   \\
     140 &    2.270 ( 0.014) &    0.924 ( 0.004) &    1.120 ( 0.014) &   29.934 ( 0.093) &   31.188 ( 0.114) &    17.28 ( 0.90) &    16.95 ( 1.00)  &  1.31 & 27.2  &	q1   \\
     145 &    1.430 ( 0.535) &    0.791 ( 0.203) &    0.729 ( 0.533) &   28.557 ( 1.563) &   30.657 ( 1.855) &    13.53 (11.57) &    11.87 (10.14)  &  0.39 & 42.7  &	q3   \\
     157 &    1.802 ( 0.071) &    0.764 ( 0.017) &    0.966 ( 0.071) &   30.066 ( 0.136) &   31.727 ( 0.175) &    22.15 ( 1.78) &    21.33 ( 1.82)  &  0.85 & 67.1  &	q3   \\
     167 &    2.501 ( 0.030) &    0.999 ( 0.013) &    1.234 ( 0.029) &   30.303 ( 0.227) &   31.336 ( 0.242) &    18.50 ( 2.06) &    18.18 ( 2.01)  &  1.05 & 59.2  &	q2   \\
     199 &    2.568 ( 0.012) &    0.989 ( 0.005) &    1.211 ( 0.010) &   30.761 ( 0.082) &   31.710 ( 0.113) &    21.97 ( 1.15) &    21.94 ( 1.08)  &  0.38 & 31.2  &	q2   \\
     200 &    2.328 ( 0.033) &    0.854 ( 0.014) &    1.073 ( 0.032) &   29.815 ( 0.169) &   31.011 ( 0.183) &    15.93 ( 1.35) &    16.14 ( 1.47)  &  1.36 & 27.5  &	q1   \\
     220 &    2.737 ( 0.008) &    1.033 ( 0.004) &    1.302 ( 0.007) &   31.751 ( 0.145) &   32.491 ( 0.164) &    31.49 ( 2.39) &    31.81 ( 2.34)  &  1.02 & 32.9  &	q2   \\
     222 &    2.545 ( 0.015) &    0.965 ( 0.006) &    1.209 ( 0.012) &   31.233 ( 0.122) &   32.196 ( 0.145) &    27.49 ( 1.84) &    27.60 ( 1.78)  &  0.37 & 28.0  &	q2   \\
     226 &    2.171 ( 0.042) &    0.816 ( 0.012) &    1.069 ( 0.041) &   30.040 ( 0.107) &   31.372 ( 0.131) &    18.81 ( 1.14) &    19.06 ( 1.31)  &  0.64 & 54.5  &	q2   \\
     230 &    2.267 ( 0.014) &    0.875 ( 0.007) &    1.064 ( 0.014) &   30.167 ( 0.158) &   31.415 ( 0.171) &    19.18 ( 1.51) &    19.17 ( 1.62)  &  0.27 & 12.7  &	q1   \\
     263 &    1.969 ( 0.026) &    0.784 ( 0.014) &    0.892 ( 0.024) &   29.498 ( 0.402) &   31.001 ( 0.408) &    15.86 ( 2.98) &    15.66 ( 2.98)  &  0.02 &  3.9  &	q2   \\
     308 &    2.218 ( 0.013) &    0.859 ( 0.007) &    1.036 ( 0.012) &   29.875 ( 0.169) &   31.158 ( 0.181) &    17.05 ( 1.42) &    17.02 ( 1.51)  &  1.64 & 30.1  &	q2   \\
     315 &    \nodata        &    0.935 ( 0.004) &    1.157 ( 0.023) &   31.462 ( 0.097) &   32.554 ( 0.133) &    32.41 ( 1.98) &    32.41 ( 1.98)  &  0.19 & 13.9  &	q2   \\
     341 &    2.632 ( 0.027) &    1.002 ( 0.004) &    1.266 ( 0.025) &   31.315 ( 0.122) &   32.188 ( 0.146) &    27.40 ( 1.85) &    27.52 ( 1.80)  &  0.64 & 39.6  &	q2   \\
     345 &    2.796 ( 0.007) &    1.075 ( 0.001) &    1.378 ( 0.007) &   31.718 ( 0.136) &   32.356 ( 0.157) &    29.59 ( 2.14) &    29.01 ( 2.03)  &  6.18 & 64.3  &	q2   \\
     355 &    2.667 ( 0.009) &    1.013 ( 0.003) &    1.281 ( 0.008) &   29.874 ( 0.060) &   30.734 ( 0.098) &    14.02 ( 0.63) &    14.12 ( 0.58)  &  0.48 & 33.0  &	q1   \\
     369 &    2.815 ( 0.005) &    1.106 ( 0.002) &    1.346 ( 0.005) &   30.316 ( 0.051) &   31.013 ( 0.092) &    15.94 ( 0.68) &    15.71 ( 0.61)  &  2.96 & 45.4  &	q1   \\
     397 &    2.406 ( 0.009) &    0.899 ( 0.002) &    1.111 ( 0.008) &   31.201 ( 0.085) &   32.310 ( 0.107) &    28.98 ( 1.43) &    29.26 ( 1.69)  &  0.10 &  7.7  &	q2   \\
     465 &    1.682 ( 0.048) &    0.662 ( 0.026) &    0.837 ( 0.046) &   29.424 ( 0.143) &   31.210 ( 0.171) &    17.46 ( 1.37) &    17.11 ( 1.47)  &  0.39 & 44.3  &	q2   \\
     483 &    2.183 ( 0.036) &    0.749 ( 0.014) &    0.978 ( 0.035) &   29.586 ( 0.088) &   30.914 ( 0.115) &    15.23 ( 0.81) &    15.60 ( 0.99)  &  1.26 & 64.6  &	q2   \\
     490 &    2.345 ( 0.030) &    0.877 ( 0.007) &    1.086 ( 0.029) &   29.866 ( 0.107) &   31.037 ( 0.128) &    16.12 ( 0.95) &    16.25 ( 1.10)  &  2.85 & 39.9  &	q2   \\
     491 &    1.725 ( 0.042) &    0.632 ( 0.019) &    0.749 ( 0.041) &   29.624 ( 0.236) &   31.362 ( 0.251) &    18.73 ( 2.17) &    18.91 ( 2.31)  &  0.62 & 53.2  &	q2   \\
     497 &    2.276 ( 0.041) &    0.898 ( 0.014) &    1.080 ( 0.039) &   29.641 ( 0.168) &   30.889 ( 0.184) &    15.06 ( 1.28) &    14.97 ( 1.37)  &  1.11 & 44.0  &	q2   \\
     523 &    2.308 ( 0.010) &    0.895 ( 0.005) &    1.076 ( 0.010) &   30.108 ( 0.085) &   31.336 ( 0.107) &    18.50 ( 0.91) &    18.58 ( 1.07)  &  1.82 & 32.2  &	q2   \\
     524 &    2.323 ( 0.017) &    0.900 ( 0.008) &    1.104 ( 0.016) &   29.849 ( 0.107) &   31.041 ( 0.126) &    16.15 ( 0.94) &    16.15 ( 1.05)  &  0.54 & 27.8  &	q2   \\
     538 &    2.179 ( 0.017) &    0.856 ( 0.007) &    1.032 ( 0.016) &   30.615 ( 0.125) &   31.930 ( 0.142) &    24.33 ( 1.59) &    24.15 ( 1.72)  &  0.13 &  9.7  &	q1   \\
     543 &    2.325 ( 0.015) &    0.879 ( 0.013) &    1.086 ( 0.019) &   29.831 ( 0.166) &   31.032 ( 0.178) &    16.08 ( 1.32) &    16.17 ( 1.43)  &  1.36 & 27.5  &	q1   \\
     559 &    2.194 ( 0.015) &    0.866 ( 0.005) &    1.050 ( 0.014) &   29.722 ( 0.114) &   31.032 ( 0.131) &    16.08 ( 0.97) &    15.98 ( 1.07)  &  1.25 & 36.4  &	q2   \\
     570 &    2.351 ( 0.015) &    0.867 ( 0.011) &    1.104 ( 0.015) &   29.993 ( 0.148) &   31.176 ( 0.162) &    17.19 ( 1.28) &    17.38 ( 1.40)  &  0.46 & 30.1  &	q2   \\
     571 &    2.049 ( 0.034) &    0.815 ( 0.012) &    0.945 ( 0.033) &   30.066 ( 0.101) &   31.493 ( 0.125) &    19.89 ( 1.14) &    19.68 ( 1.31)  &  0.44 & 19.4  &	q1   \\
     575 &    2.460 ( 0.015) &    0.931 ( 0.005) &    1.149 ( 0.015) &   30.347 ( 0.104) &   31.411 ( 0.130) &    19.16 ( 1.15) &    19.30 ( 1.14)  &  0.74 & 22.1  &	q1   \\
     596 &    2.088 ( 0.036) &    0.767 ( 0.012) &    1.052 ( 0.036) &   29.750 ( 0.088) &   31.148 ( 0.115) &    16.97 ( 0.90) &    17.28 ( 1.06)  &  4.11 & 179.0  &	q2   \\
     613 &    2.225 ( 0.020) &    0.876 ( 0.009) &    1.083 ( 0.018) &   29.681 ( 0.102) &   30.961 ( 0.122) &    15.56 ( 0.88) &    15.46 ( 0.98)  &  0.33 & 33.3  &	q2   \\
     648 &    2.764 ( 0.004) &    1.061 ( 0.001) &    1.320 ( 0.004) &   31.068 ( 0.063) &   31.777 ( 0.100) &    22.67 ( 1.04) &    22.59 ( 0.96)  &  1.01 & 28.9  &	q2   \\
     654 &  \nodata          &    1.020 ( 0.003) &    1.281 ( 0.010) &   30.251 ( 0.048) &   31.090 ( 0.068) &    16.52 ( 0.52) &    16.52 ( 0.52)  &  3.37 & 54.7  &	q2   \\
     657 &    2.435 ( 0.072) &    0.857 ( 0.017) &    1.070 ( 0.069) &   30.415 ( 0.191) &   31.497 ( 0.218) &    19.92 ( 2.00) &    20.58 ( 2.14)  &  0.35 & 27.1  &	q2   \\
     685 &  \nodata          &    0.983 ( 0.005) &    1.230 ( 0.020) &   30.020 ( 0.069) &   30.985 ( 0.087) &    15.74 ( 0.63) &    15.74 ( 0.63)  &  3.67 & 55.3  &	q2   \\
     692 &    1.936 ( 0.040) &    0.737 ( 0.030) &    0.866 ( 0.040) &   29.373 ( 0.154) &   30.904 ( 0.173) &    15.16 ( 1.21) &    15.19 ( 1.34)  &  0.54 & 43.0  &	q2   \\
     698 &    2.472 ( 0.018) &    0.932 ( 0.008) &    1.149 ( 0.017) &   30.233 ( 0.123) &   31.288 ( 0.146) &    18.10 ( 1.22) &    18.29 ( 1.22)  &  2.55 & 42.5  &	q1   \\
     731 &    2.811 ( 0.003) &    1.067 ( 0.001) &    1.311 ( 0.003) &   31.152 ( 0.059) &   31.778 ( 0.097) &    22.68 ( 1.01) &    22.61 ( 0.93)  &  3.96 & 52.2  &	q1   \\
     750 &    2.310 ( 0.011) &    0.894 ( 0.003) &    1.092 ( 0.010) &   30.740 ( 0.137) &   31.949 ( 0.152) &    24.54 ( 1.72) &    24.55 ( 1.86)  &  0.21 & 11.5  &	q2   \\
     759 &    2.717 ( 0.008) &    1.069 ( 0.006) &    1.340 ( 0.007) &   30.301 ( 0.101) &   31.099 ( 0.127) &    16.59 ( 0.97) &    16.35 ( 0.91)  &  0.83 & 54.3  &	q1   \\
     763 &    2.866 ( 0.002) &    1.114 ( 0.001) &    1.371 ( 0.001) &   30.613 ( 0.044) &   31.224 ( 0.089) &    17.57 ( 0.72) &    17.35 ( 0.64)  &  5.91 & 61.5  &	q1   \\
     778 &    2.625 ( 0.016) &    1.010 ( 0.006) &    1.240 ( 0.014) &   30.326 ( 0.061) &   31.240 ( 0.099) &    17.70 ( 0.81) &    17.76 ( 0.75)  &  3.26 & 48.2  &	q1   \\
     784 &    2.650 ( 0.011) &    1.036 ( 0.004) &    1.259 ( 0.011) &   30.218 ( 0.047) &   31.070 ( 0.091) &    16.37 ( 0.68) &    16.21 ( 0.61)  &  3.22 & 46.0  &	q1   \\
     785 &    1.804 ( 0.044) &    0.731 ( 0.027) &    0.952 ( 0.041) &   31.276 ( 0.988) &   32.912 ( 0.992) &    38.24 (17.48) &    37.33 (17.13)  &  1.55 & 95.3  &	q3   \\
     792 &    2.480 ( 0.017) &    0.963 ( 0.008) &    1.160 ( 0.016) &   30.014 ( 0.083) &   31.057 ( 0.114) &    16.27 ( 0.86) &    16.19 ( 0.81)  &  0.41 & 54.1  &	q2   \\
     801 &    1.772 ( 0.026) &    0.715 ( 0.007) &    0.868 ( 0.026) &   29.627 ( 0.112) &   31.303 ( 0.133) &    18.22 ( 1.12) &    17.72 ( 1.20)  &  0.34 & 30.8  &	q2   \\
     828 &    2.639 ( 0.012) &    1.049 ( 0.006) &    1.261 ( 0.012) &   30.497 ( 0.107) &   31.381 ( 0.132) &    18.88 ( 1.15) &    18.65 ( 1.09)  &  1.20 & 33.3  &	q1   \\
     836 &    1.936 ( 0.020) &    0.785 ( 0.010) &    0.956 ( 0.020) &   29.659 ( 0.124) &   31.195 ( 0.142) &    17.34 ( 1.13) &    17.00 ( 1.22)  &  0.28 & 42.8  &	q2   \\
     856 &    2.299 ( 0.011) &    0.894 ( 0.005) &    1.073 ( 0.010) &   29.810 ( 0.092) &   31.025 ( 0.112) &    16.03 ( 0.83) &    16.02 ( 0.95)  &  1.20 & 26.3  &	q1   \\
     865 &    1.636 ( 0.108) &    0.745 ( 0.035) &    0.769 ( 0.107) &   29.430 ( 0.197) &   31.253 ( 0.260) &    17.81 ( 2.13) &    16.83 ( 1.99)  &  0.59 & 39.3  &	q2   \\
     873 &    2.168 ( 0.016) &    0.874 ( 0.007) &    1.039 ( 0.015) &   29.734 ( 0.071) &   31.068 ( 0.097) &    16.35 ( 0.73) &    16.11 ( 0.85)  &  0.52 & 34.4  &	q2   \\
     874 &    2.205 ( 0.011) &    0.829 ( 0.005) &    1.030 ( 0.011) &   29.859 ( 0.089) &   31.156 ( 0.110) &    17.03 ( 0.87) &    17.10 ( 1.01)  &  0.39 & 32.4  &	q2   \\
     881 &    2.777 ( 0.001) &    1.058 ( 0.001) &    1.335 ( 0.001) &   30.691 ( 0.100) &   31.390 ( 0.127) &    18.97 ( 1.11) &    19.01 ( 1.06)  &  2.82 & 46.3  &	q1   \\
     896 &    1.941 ( 0.039) &    0.789 ( 0.017) &    0.893 ( 0.038) &   29.553 ( 0.121) &   31.081 ( 0.144) &    16.45 ( 1.09) &    16.18 ( 1.22)  &  0.06 &  6.1  &	q2   \\
     898 &    1.951 ( 0.031) &    0.772 ( 0.015) &    0.913 ( 0.029) &   29.106 ( 0.426) &   30.625 ( 0.432) &    13.34 ( 2.66) &    13.14 ( 2.66)  &  0.03 &  3.9  &	q3   \\
     912 &    2.278 ( 0.037) &    0.898 ( 0.017) &    1.063 ( 0.036) &   29.820 ( 0.119) &   31.063 ( 0.140) &    16.31 ( 1.05) &    16.22 ( 1.19)  &  0.96 & 52.5  &	q2   \\
     916 &    2.830 ( 0.007) &    1.069 ( 0.003) &    1.332 ( 0.006) &   30.831 ( 0.142) &   31.459 ( 0.162) &    19.58 ( 1.46) &    19.74 ( 1.44)  &  0.14 &  8.8  &	q2   \\
     928 &    2.132 ( 0.013) &    0.868 ( 0.007) &    0.983 ( 0.013) &   30.318 ( 0.177) &   31.685 ( 0.189) &    21.73 ( 1.89) &    21.44 ( 1.97)  &  0.18 & 10.5  &	q2   \\
     929 &    2.469 ( 0.013) &    0.909 ( 0.004) &    1.149 ( 0.012) &   29.973 ( 0.044) &   31.024 ( 0.090) &    16.02 ( 0.66) &    16.26 ( 0.66)  &  2.67 & 39.2  &	q2   \\
     930 &    2.020 ( 0.050) &    0.834 ( 0.023) &    0.938 ( 0.048) &   29.719 ( 0.880) &   31.177 ( 0.884) &    17.20 ( 7.00) &    16.89 ( 6.91)  &  0.04 &  4.5  &	q3   \\
     938 &    2.305 ( 0.024) &    0.791 ( 0.013) &    1.019 ( 0.021) &   30.167 ( 0.161) &   31.377 ( 0.175) &    18.86 ( 1.52) &    19.44 ( 1.68)  &  0.16 & 43.2  &	q3   \\
     939 &    1.762 ( 0.012) &    0.708 ( 0.004) &    0.858 ( 0.012) &   29.095 ( 0.082) &   30.790 ( 0.105) &    14.39 ( 0.70) &    13.98 ( 0.78)  &  0.46 & 24.9  &	q2   \\
     940 &    2.370 ( 0.013) &    0.983 ( 0.006) &    1.182 ( 0.012) &   29.912 ( 0.088) &   31.070 ( 0.110) &    16.37 ( 0.83) &    15.94 ( 0.79)  &  0.67 & 20.1  &	q2   \\
     942 &    1.812 ( 0.157) &    0.771 ( 0.029) &    0.945 ( 0.156) &   29.510 ( 0.167) &   31.153 ( 0.263) &    17.01 ( 2.06) &    16.36 ( 1.86)  &  0.02 &  2.9  &	q3   \\
     944 &    2.371 ( 0.021) &    0.955 ( 0.007) &    1.181 ( 0.020) &   29.949 ( 0.157) &   31.099 ( 0.171) &    16.59 ( 1.30) &    16.21 ( 1.27)  &  2.11 & 49.5  &	q1   \\
     950 &    1.344 ( 0.223) &    0.426 ( 0.038) &    0.665 ( 0.222) &   28.068 ( 0.182) &   30.297 ( 0.498) &    11.46 ( 2.63) &    11.65 ( 2.73)  &  0.22 & 24.9  &	q3   \\
     951 &    2.044 ( 0.109) &    0.826 ( 0.017) &    0.919 ( 0.108) &   29.669 ( 0.088) &   31.105 ( 0.158) &    16.63 ( 1.21) &    16.36 ( 1.16)  &  1.19 & 34.2  &	q2   \\
     958 &    2.205 ( 0.025) &    0.918 ( 0.010) &    1.139 ( 0.024) &   29.994 ( 0.083) &   31.300 ( 0.108) &    18.20 ( 0.91) &    17.66 ( 1.01)  &  0.85 & 40.8  &	q2   \\
     962 &    2.091 ( 0.041) &    0.850 ( 0.020) &    1.034 ( 0.039) &   30.620 ( 0.231) &   32.017 ( 0.243) &    25.31 ( 2.84) &    24.85 ( 2.90)  &  0.05 &  6.3  &	q3   \\
     965 &    2.172 ( 0.025) &    0.877 ( 0.011) &    1.040 ( 0.025) &   30.024 ( 0.221) &   31.355 ( 0.231) &    18.66 ( 1.99) &    18.39 ( 2.03)  &  0.68 & 20.2  &	q2   \\
     966 &  \nodata          &    0.947 ( 0.002) &    1.229 ( 0.005) &   30.087 ( 0.064) &   31.095 ( 0.079) &    16.56 ( 0.60) &    16.56 ( 0.60)  &  1.78 & 38.7  &	q2   \\
     967 &    2.083 ( 0.036) &    0.846 ( 0.016) &    0.987 ( 0.033) &   30.069 ( 0.276) &   31.474 ( 0.285) &    19.71 ( 2.59) &    19.40 ( 2.61)  &  0.04 &  4.4  &	q2   \\
     968 &    1.729 ( 0.038) &    0.670 ( 0.018) &    0.789 ( 0.037) &   29.475 ( 0.334) &   31.199 ( 0.343) &    17.37 ( 2.75) &    17.07 ( 2.77)  &  0.05 &  5.0  &	q2   \\
     972 &    2.094 ( 0.025) &    0.833 ( 0.011) &    0.986 ( 0.023) &   29.817 ( 0.195) &   31.209 ( 0.207) &    17.45 ( 1.66) &    17.25 ( 1.72)  &  0.07 &  5.9  &	q2   \\
     977 &    1.906 ( 0.070) &    0.880 ( 0.011) &    0.859 ( 0.069) &   30.361 ( 0.146) &   31.915 ( 0.178) &    24.16 ( 1.98) &    23.25 ( 1.95)  &  0.06 &  5.9  &	q3   \\
     978 &    1.659 ( 0.243) &    0.850 ( 0.027) &    0.705 ( 0.243) &   29.413 ( 0.506) &   31.211 ( 0.615) &    17.47 ( 4.95) &    16.33 ( 4.30)  &  0.05 &  6.0  &	q3   \\
     979 &    2.019 ( 0.020) &    0.812 ( 0.007) &    0.970 ( 0.020) &   29.528 ( 0.123) &   30.978 ( 0.141) &    15.69 ( 1.02) &    15.41 ( 1.09)  &  0.25 & 43.3  &	q2   \\
     984 &    2.285 ( 0.046) &    0.946 ( 0.018) &    1.123 ( 0.045) &   29.788 ( 0.104) &   31.021 ( 0.131) &    16.00 ( 0.97) &    15.64 ( 1.07)  &  3.04 & 53.7  &	q2   \\
     990 &    2.321 ( 0.012) &    0.909 ( 0.006) &    1.089 ( 0.011) &   29.856 ( 0.088) &   31.057 ( 0.110) &    16.27 ( 0.82) &    16.21 ( 0.95)  &  0.67 & 20.3  &	q2   \\
     996 &    2.008 ( 0.052) &    0.828 ( 0.023) &    0.953 ( 0.051) &   29.375 ( 0.500) &   30.844 ( 0.507) &    14.75 ( 3.45) &    14.44 ( 3.42)  &  0.06 &  5.9  &	q3   \\
     997 &    1.950 ( 0.083) &    0.834 ( 0.014) &    0.941 ( 0.082) &   29.993 ( 0.280) &   31.509 ( 0.301) &    20.03 ( 2.78) &    19.40 ( 2.76)  &  0.06 &  6.1  &	q2   \\
     998 &    1.976 ( 0.117) &    0.844 ( 0.018) &    0.934 ( 0.116) &   29.500 ( 0.213) &   30.996 ( 0.257) &    15.82 ( 1.87) &    15.39 ( 1.80)  &  0.07 &  6.1  &	q3   \\
    1000 &    2.218 ( 0.042) &    0.881 ( 0.019) &    1.017 ( 0.039) &   30.141 ( 0.203) &   31.439 ( 0.217) &    19.40 ( 1.94) &    19.25 ( 2.05)  &  0.04 &  4.5  &	q3   \\
    1003 &    2.767 ( 0.004) &    1.074 ( 0.002) &    1.388 ( 0.003) &   30.382 ( 0.044) &   31.107 ( 0.088) &    16.65 ( 0.68) &    16.38 ( 0.59)  &  4.68 & 61.1  &	q2   \\
    1010 &    2.500 ( 0.006) &    1.031 ( 0.001) &    1.193 ( 0.006) &   30.181 ( 0.091) &   31.211 ( 0.119) &    17.46 ( 0.96) &    17.13 ( 0.89)  &  0.45 & 16.0  &	q2   \\
    1017 &    1.814 ( 0.053) &    0.673 ( 0.017) &    0.796 ( 0.053) &   29.062 ( 0.144) &   30.697 ( 0.170) &    13.78 ( 1.08) &    13.86 ( 1.21)  &  0.27 & 12.3  &	q2   \\
    1020 &    2.092 ( 0.046) &    0.834 ( 0.009) &    0.979 ( 0.046) &   29.970 ( 0.191) &   31.363 ( 0.207) &    18.74 ( 1.78) &    18.53 ( 1.87)  &  0.06 &  6.2  &	q2   \\
    1025 &    2.612 ( 0.009) &    0.976 ( 0.003) &    1.218 ( 0.009) &   30.778 ( 0.049) &   31.673 ( 0.092) &    21.61 ( 0.91) &    21.94 ( 0.83)  &  2.42 & 38.1  &	q1   \\
    1027 &    2.058 ( 0.072) &    0.780 ( 0.032) &    0.968 ( 0.068) &   30.132 ( 0.457) &   31.558 ( 0.468) &    20.49 ( 4.42) &    20.55 ( 4.49)  &  0.05 &  5.6  &	q3   \\
    1030 &    2.461 ( 0.005) &    0.975 ( 0.002) &    1.172 ( 0.005) &   30.101 ( 0.068) &   31.170 ( 0.103) &    17.14 ( 0.81) &    17.02 ( 0.74)  &  1.21 & 37.5  &	q1   \\
    1035 &    1.875 ( 0.032) &    0.786 ( 0.005) &    0.868 ( 0.032) &   29.325 ( 0.112) &   30.910 ( 0.135) &    15.20 ( 0.94) &    14.82 ( 1.03)  &  0.11 &  8.0  &	q2   \\
    1036 &    2.314 ( 0.032) &    0.917 ( 0.006) &    1.092 ( 0.032) &   29.860 ( 0.104) &   31.065 ( 0.127) &    16.33 ( 0.95) &    16.22 ( 1.07)  &  1.42 & 30.8  &	q2   \\
    1040 &    2.250 ( 0.014) &    0.907 ( 0.006) &    1.063 ( 0.013) &   29.184 ( 0.075) &   30.446 ( 0.100) &    12.28 ( 0.56) &    12.14 ( 0.65)  &  0.11 &  8.2  &	q3   \\
    1043 &    2.398 ( 0.024) &    0.911 ( 0.011) &    1.231 ( 0.023) &   29.993 ( 0.091) &   31.122 ( 0.114) &    16.76 ( 0.88) &    16.95 ( 1.02)  &  1.84 & 77.5  &	q2   \\
    1049 &    2.150 ( 0.032) &    0.817 ( 0.009) &    0.973 ( 0.031) &   29.539 ( 0.058) &   30.881 ( 0.092) &    15.01 ( 0.64) &    15.12 ( 0.81)  &  1.17 & 27.6  &	q1   \\
    1052 &    1.825 ( 0.426) &    0.793 ( 0.057) &    0.753 ( 0.424) &   29.384 ( 0.437) &   31.015 ( 0.679) &    15.96 ( 4.99) &    15.29 ( 4.13)  &  0.11 &  7.9  &	q3   \\
    1059 &    2.062 ( 0.065) &    0.846 ( 0.011) &    0.965 ( 0.065) &   29.985 ( 0.087) &   31.404 ( 0.128) &    19.09 ( 1.13) &    18.77 ( 1.23)  &  0.06 &  5.9  &	q2   \\
    1062 &    2.654 ( 0.005) &    1.045 ( 0.002) &    1.305 ( 0.005) &   29.983 ( 0.038) &   30.826 ( 0.086) &    14.63 ( 0.58) &    14.37 ( 0.50)  &  2.21 & 46.6  &	q1   \\
    1069 &    2.134 ( 0.018) &    0.842 ( 0.007) &    0.969 ( 0.017) &   29.835 ( 0.083) &   31.192 ( 0.106) &    17.32 ( 0.85) &    17.19 ( 0.99)  &  0.13 &  8.5  &	q2   \\
    1073 &    2.526 ( 0.041) &    1.024 ( 0.006) &    1.202 ( 0.040) &   30.105 ( 0.088) &   31.106 ( 0.124) &    16.65 ( 0.95) &    16.39 ( 0.91)  &  1.67 & 31.3  &	q2   \\
    1075 &    2.352 ( 0.022) &    0.899 ( 0.008) &    1.084 ( 0.021) &   29.609 ( 0.113) &   30.780 ( 0.132) &    14.32 ( 0.87) &    14.44 ( 0.98)  &  0.91 & 22.7  &	q1   \\
    1076 &    1.987 ( 0.040) &    0.805 ( 0.015) &    0.883 ( 0.039) &   29.833 ( 0.153) &   31.321 ( 0.172) &    18.37 ( 1.45) &    18.04 ( 1.58)  &  0.08 &  7.9  &	q2   \\
    1079 &    2.175 ( 0.036) &    0.884 ( 0.014) &    1.018 ( 0.034) &   29.880 ( 0.352) &   31.206 ( 0.359) &    17.43 ( 2.89) &    17.20 ( 2.89)  &  0.07 &  6.3  &	q3   \\
    1087 &    2.598 ( 0.010) &    0.932 ( 0.002) &    1.277 ( 0.010) &   29.901 ( 0.100) &   30.822 ( 0.127) &    14.60 ( 0.85) &    15.06 ( 0.87)  &  0.39 & 16.5  &	q2   \\
    1093 &    2.157 ( 0.060) &    0.867 ( 0.010) &    1.012 ( 0.059) &   29.777 ( 0.080) &   31.118 ( 0.119) &    16.74 ( 0.92) &    16.55 ( 1.06)  &  0.11 &  8.1  &	q2   \\
    1100 &    1.829 ( 0.122) &    0.725 ( 0.020) &    0.843 ( 0.121) &   29.797 ( 0.183) &   31.426 ( 0.243) &    19.28 ( 2.16) &    18.94 ( 2.06)  &  0.06 &  6.1  &	q2   \\
    1101 &    2.028 ( 0.020) &    0.783 ( 0.008) &    0.920 ( 0.019) &   29.893 ( 0.103) &   31.338 ( 0.123) &    18.52 ( 1.05) &    18.50 ( 1.19)  &  0.10 &  8.2  &	q2   \\
    1104 &    2.055 ( 0.018) &    0.796 ( 0.007) &    0.939 ( 0.017) &   29.653 ( 0.065) &   31.074 ( 0.093) &    16.40 ( 0.70) &    16.37 ( 0.86)  &  0.45 & 16.3  &	q2   \\
    1110 &    2.507 ( 0.016) &    0.961 ( 0.004) &    1.244 ( 0.015) &   30.142 ( 0.078) &   31.162 ( 0.110) &    17.08 ( 0.87) &    17.17 ( 0.81)  &  1.62 & 80.4  &	q2   \\
    1115 &    1.963 ( 0.164) &    0.795 ( 0.026) &    1.027 ( 0.163) &   29.336 ( 0.227) &   30.845 ( 0.297) &    14.76 ( 2.02) &    14.49 ( 1.91)  &  0.03 &  4.6  &	q3   \\
    1122 &    1.987 ( 0.054) &    0.778 ( 0.020) &    0.930 ( 0.053) &   29.584 ( 0.151) &   31.062 ( 0.174) &    16.31 ( 1.31) &    16.15 ( 1.44)  &  0.64 & 25.2  &	q2   \\
    1123 &    2.090 ( 0.027) &    0.822 ( 0.012) &    0.979 ( 0.025) &   29.912 ( 0.261) &   31.304 ( 0.270) &    18.23 ( 2.27) &    18.06 ( 2.32)  &  0.06 &  6.0  &	q2   \\
    1125 &    2.305 ( 0.039) &    0.928 ( 0.006) &    1.091 ( 0.039) &   29.773 ( 0.138) &   30.989 ( 0.157) &    15.77 ( 1.14) &    15.60 ( 1.23)  &  1.44 & 36.5  &	q2   \\
    1129 &    1.925 ( 0.032) &    0.772 ( 0.013) &    0.903 ( 0.030) &   29.444 ( 0.219) &   30.976 ( 0.231) &    15.67 ( 1.67) &    15.38 ( 1.70)  &  0.06 &  6.0  &	q2   \\
    1131 &    1.901 ( 0.148) &    0.763 ( 0.023) &    0.887 ( 0.147) &   29.611 ( 0.281) &   31.171 ( 0.334) &    17.15 ( 2.64) &    16.83 ( 2.51)  &  0.04 &  4.5  &	q2   \\
    1136 &    1.890 ( 0.221) &    0.716 ( 0.034) &    0.854 ( 0.220) &   29.264 ( 0.171) &   30.834 ( 0.313) &    14.68 ( 2.12) &    14.71 ( 1.89)  &  0.04 &  5.0  &	q3   \\
    1146 &    2.415 ( 0.011) &    0.955 ( 0.004) &    1.172 ( 0.010) &   30.042 ( 0.056) &   31.148 ( 0.086) &    16.97 ( 0.67) &    16.76 ( 0.64)  &  4.91 & 53.0  &	q1   \\
    1148 &    2.897 ( 0.011) &    1.093 ( 0.005) &    1.373 ( 0.009) &   29.862 ( 0.130) &   30.352 ( 0.151) &    11.76 ( 0.82) &    11.75 ( 0.81)  &  0.09 &  8.4  &	q2   \\
    1149 &    1.630 ( 0.138) &    0.679 ( 0.048) &    0.685 ( 0.136) &   29.757 ( 0.637) &   31.574 ( 0.669) &    20.64 ( 6.37) &    19.88 ( 6.17)  &  0.07 &  6.0  &	q3   \\
    1153 &    2.234 ( 0.036) &    0.874 ( 0.014) &    1.027 ( 0.034) &   29.923 ( 0.191) &   31.192 ( 0.205) &    17.31 ( 1.64) &    17.24 ( 1.73)  &  0.06 &  6.1  &	q3   \\
    1154 &    2.925 ( 0.001) &    1.094 ( 0.001) &    1.442 ( 0.001) &   30.383 ( 0.067) &   30.915 ( 0.102) &    15.24 ( 0.72) &    15.57 ( 0.66)  &  2.29 & 38.3  &	q1   \\
    1158 &    2.746 ( 0.004) &    1.017 ( 0.002) &    1.256 ( 0.004) &   30.484 ( 0.113) &   31.208 ( 0.137) &    17.45 ( 1.10) &    17.90 ( 1.08)  &  3.07 & 42.1  &	q2   \\
    1173 &    2.088 ( 0.014) &    0.833 ( 0.006) &    0.885 ( 0.014) &   29.677 ( 0.100) &   31.069 ( 0.119) &    16.36 ( 0.90) &    16.16 ( 1.03)  &  0.19 & 10.1  &	q2   \\
    1177 &    1.984 ( 0.138) &    0.802 ( 0.025) &    1.004 ( 0.136) &   29.127 ( 0.195) &   30.611 ( 0.253) &    13.25 ( 1.55) &    13.01 ( 1.48)  &  0.03 &  4.5  &	q3   \\
    1178 &    2.673 ( 0.008) &    0.999 ( 0.003) &    1.230 ( 0.008) &   29.981 ( 0.047) &   30.799 ( 0.090) &    14.45 ( 0.60) &    14.72 ( 0.55)  &  0.48 & 20.8  &	q1   \\
    1185 &    2.484 ( 0.013) &    0.923 ( 0.005) &    1.174 ( 0.012) &   30.145 ( 0.169) &   31.181 ( 0.186) &    17.23 ( 1.48) &    17.40 ( 1.49)  &  0.10 &  7.6  &	q1   \\
    1190 &    2.563 ( 0.014) &    1.003 ( 0.005) &    1.239 ( 0.014) &   30.100 ( 0.110) &   31.046 ( 0.135) &    16.19 ( 1.01) &    16.05 ( 0.96)  &  0.76 & 38.6  &	q2   \\
    1191 &    1.983 ( 0.034) &    0.750 ( 0.016) &    0.917 ( 0.033) &   29.725 ( 0.398) &   31.208 ( 0.404) &    17.44 ( 3.25) &    17.44 ( 3.29)  &  0.04 &  5.3  &	q3   \\
    1192 &    2.776 ( 0.009) &    1.043 ( 0.003) &    1.303 ( 0.008) &   30.282 ( 0.086) &   30.964 ( 0.116) &    15.59 ( 0.83) &    15.76 ( 0.79)  &  0.38 & 14.9  &	q1   \\
    1199 &    2.942 ( 0.014) &    1.064 ( 0.006) &    1.364 ( 0.011) &   30.666 ( 0.091) &   31.084 ( 0.120) &    16.47 ( 0.91) &    17.25 ( 0.90)  &  0.04 &  6.3  &	q3   \\
    1205 &    1.856 ( 0.038) &    0.782 ( 0.010) &    0.843 ( 0.038) &   29.495 ( 0.136) &   31.093 ( 0.157) &    16.54 ( 1.20) &    16.16 ( 1.28)  &  0.45 & 33.8  &	q2   \\
    1212 &    1.915 ( 0.178) &    0.848 ( 0.024) &    0.815 ( 0.177) &   29.856 ( 0.173) &   31.416 ( 0.277) &    19.19 ( 2.45) &    18.41 ( 2.09)  &  0.06 &  6.2  &	q3   \\
    1213 &    2.168 ( 0.020) &    0.818 ( 0.009) &    0.993 ( 0.019) &   29.904 ( 0.100) &   31.231 ( 0.120) &    17.63 ( 0.98) &    17.70 ( 1.13)  &  0.11 &  8.1  &	q2   \\
    1216 &    1.931 ( 0.227) &    0.793 ( 0.033) &    0.805 ( 0.225) &   29.387 ( 0.131) &   30.922 ( 0.293) &    15.29 ( 2.07) &    14.92 ( 1.71)  &  0.04 &  4.6  &	q3   \\
    1219 &    1.849 ( 0.038) &    0.722 ( 0.017) &    0.863 ( 0.037) &   28.983 ( 0.162) &   30.582 ( 0.180) &    13.07 ( 1.09) &    12.87 ( 1.16)  &  0.04 &  5.1  &	q3   \\
    1226 &    2.863 ( 0.002) &    1.059 ( 0.001) &    1.369 ( 0.002) &   30.657 ( 0.072) &   31.208 ( 0.105) &    17.44 ( 0.85) &    17.82 ( 0.80)  & 15.51 & 98.0  &	q1   \\
    1231 &    2.680 ( 0.004) &    1.028 ( 0.002) &    1.302 ( 0.004) &   30.329 ( 0.032) &   31.154 ( 0.083) &    17.01 ( 0.65) &    17.00 ( 0.57)  &  5.11 & 57.2  &	q1   \\
    1239 &    1.727 ( 0.034) &    0.778 ( 0.008) &    0.930 ( 0.034) &   29.357 ( 0.354) &   31.087 ( 0.362) &    16.50 ( 2.76) &    15.43 ( 2.62)  &  0.02 &  3.8  &	q3   \\
    1242 &    2.322 ( 0.019) &    0.904 ( 0.009) &    1.118 ( 0.018) &   29.857 ( 0.076) &   31.072 ( 0.101) &    16.38 ( 0.77) &    16.42 ( 0.91)  &  3.61 & 55.7  &	q1   \\
    1244 &    2.061 ( 0.056) &    0.688 ( 0.024) &    1.002 ( 0.052) &   28.981 ( 0.197) &   30.400 ( 0.215) &    12.02 ( 1.19) &    12.38 ( 1.29)  &  0.01 &  3.0  &	q3   \\
    1250 &    2.291 ( 0.013) &    0.904 ( 0.002) &    1.124 ( 0.013) &   30.004 ( 0.035) &   31.229 ( 0.074) &    17.61 ( 0.60) &    17.48 ( 0.76)  &  0.61 & 22.2  &	q1   \\
    1253 &    2.841 ( 0.003) &    1.076 ( 0.002) &    1.368 ( 0.003) &   30.587 ( 0.085) &   31.202 ( 0.115) &    17.40 ( 0.92) &    17.56 ( 0.87)  &  3.66 & 54.0  &	q2   \\
    1259 &    1.900 ( 0.121) &    0.742 ( 0.020) &    0.863 ( 0.120) &   28.991 ( 0.213) &   30.553 ( 0.262) &    12.90 ( 1.56) &    12.80 ( 1.52)  &  0.07 &  6.0  &	q3   \\
    1261 &    2.261 ( 0.014) &    0.892 ( 0.005) &    1.070 ( 0.013) &   30.055 ( 0.155) &   31.309 ( 0.168) &    18.27 ( 1.42) &    18.15 ( 1.50)  &  3.26 & 43.1  &	q1   \\
    1264 &    1.956 ( 0.071) &    0.797 ( 0.011) &    0.901 ( 0.071) &   29.642 ( 0.127) &   31.152 ( 0.163) &    17.00 ( 1.27) &    16.71 ( 1.30)  &  0.06 &  6.2  &	q2   \\
    1279 &    2.615 ( 0.003) &    1.014 ( 0.001) &    1.310 ( 0.002) &   30.318 ( 0.091) &   31.210 ( 0.119) &    17.46 ( 0.96) &    17.29 ( 0.88)  &  0.51 & 24.6  &	q1   \\
    1283 &    2.630 ( 0.008) &    1.030 ( 0.004) &    1.271 ( 0.008) &   30.239 ( 0.132) &   31.126 ( 0.153) &    16.80 ( 1.19) &    16.69 ( 1.14)  &  2.17 & 39.8  &	q1   \\
    1289 &    1.883 ( 0.095) &    0.766 ( 0.029) &    0.887 ( 0.093) &   29.297 ( 0.626) &   30.873 ( 0.639) &    14.95 ( 4.40) &    14.61 ( 4.36)  &  0.07 &  7.3  &	q3   \\
    1297 &    2.660 ( 0.012) &    1.041 ( 0.005) &    1.373 ( 0.010) &   30.367 ( 0.183) &   31.200 ( 0.198) &    17.38 ( 1.59) &    16.99 ( 1.51)  &  0.15 & 14.1  &	q1   \\
    1298 &    1.951 ( 0.048) &    0.750 ( 0.017) &    0.886 ( 0.046) &   30.050 ( 0.156) &   31.559 ( 0.176) &    20.50 ( 1.67) &    20.46 ( 1.83)  &  0.05 &  5.0  &	q3   \\
    1300 &    1.672 ( 0.081) &    0.786 ( 0.021) &    0.600 ( 0.079) &   29.214 ( 0.375) &   30.989 ( 0.396) &    15.77 ( 2.88) &    14.66 ( 2.67)  &  0.03 &  4.5  &	q3   \\
    1303 &    2.560 ( 0.022) &    0.939 ( 0.006) &    1.217 ( 0.021) &   29.980 ( 0.055) &   30.929 ( 0.097) &    15.34 ( 0.69) &    15.55 ( 0.65)  &  1.31 & 37.2  &	q1   \\
    1308 &    2.242 ( 0.022) &    0.871 ( 0.006) &    1.047 ( 0.022) &   29.808 ( 0.052) &   31.085 ( 0.085) &    16.48 ( 0.65) &    16.51 ( 0.82)  &  0.50 & 16.8  &	q2   \\
    1314 &    1.796 ( 0.044) &    0.731 ( 0.013) &    0.841 ( 0.043) &   29.517 ( 0.109) &   31.173 ( 0.137) &    17.16 ( 1.09) &    16.71 ( 1.22)  &  0.09 &  8.7  &	q2   \\
    1316 &    2.890 ( 0.001) &    1.091 ( 0.001) &    1.529 ( 0.000) &   30.607 ( 0.040) &   31.116 ( 0.087) &    16.72 ( 0.67) &    16.72 ( 0.60)  &  9.13 & 82.8  &	q1   \\
    1317 &    1.880 ( 0.049) &    0.700 ( 0.016) &    0.844 ( 0.048) &   29.574 ( 0.116) &   31.148 ( 0.144) &    16.97 ( 1.13) &    17.02 ( 1.31)  &  0.09 &  7.0  &	q2   \\
    1318 &    2.438 ( 0.009) &    0.910 ( 0.003) &    1.141 ( 0.008) &   29.949 ( 0.040) &   31.028 ( 0.087) &    16.06 ( 0.65) &    16.20 ( 0.64)  &  1.52 & 33.9  &	q2   \\
    1321 &     \nodata       &    0.946 ( 0.002) &    1.171 ( 0.009) &   29.751 ( 0.055) &   30.825 ( 0.101) &    14.62 ( 0.68) &    14.62 ( 0.68)  &  2.44 & 37.8  &	q1   \\
    1324 &    1.708 ( 0.063) &    0.706 ( 0.021) &    0.795 ( 0.061) &   29.829 ( 0.329) &   31.573 ( 0.345) &    20.63 ( 3.28) &    19.95 ( 3.24)  &  0.12 &  7.9  &	q3   \\
    1327 &    2.694 ( 0.007) &    0.987 ( 0.004) &    1.296 ( 0.006) &   30.361 ( 0.080) &   31.156 ( 0.111) &    17.03 ( 0.87) &    17.33 ( 0.82)  &  0.13 & 18.3  &	q1   \\
    1331 &    1.882 ( 0.075) &    0.751 ( 0.032) &    0.869 ( 0.072) &   29.733 ( 0.225) &   31.316 ( 0.250) &    18.33 ( 2.11) &    18.03 ( 2.20)  &  0.06 &  5.9  &	q3   \\
    1336 &    1.905 ( 0.071) &    0.769 ( 0.028) &    0.864 ( 0.069) &   30.172 ( 0.250) &   31.729 ( 0.270) &    22.18 ( 2.76) &    21.84 ( 2.81)  &  0.06 &  5.9  &	q3   \\
    1340 &    1.929 ( 0.069) &    0.755 ( 0.022) &    0.877 ( 0.068) &   30.156 ( 0.132) &   31.686 ( 0.166) &    21.74 ( 1.66) &    21.55 ( 1.81)  &  0.08 &  7.0  &	q3   \\
    1341 &    1.907 ( 0.062) &    0.728 ( 0.020) &    0.809 ( 0.061) &   29.391 ( 0.232) &   30.941 ( 0.251) &    15.43 ( 1.78) &    15.42 ( 1.85)  &  0.06 &  5.9  &	q2   \\
    1343 &    1.852 ( 0.048) &    0.737 ( 0.015) &    0.810 ( 0.047) &   29.557 ( 0.194) &   31.158 ( 0.212) &    17.05 ( 1.66) &    16.78 ( 1.73)  &  0.07 &  6.0  &	q2   \\
    1348 &    2.551 ( 0.011) &    1.002 ( 0.005) &    1.247 ( 0.010) &   29.954 ( 0.059) &   30.919 ( 0.098) &    15.27 ( 0.69) &    15.04 ( 0.62)  &  0.18 & 11.2  &	q2   \\
    1352 &    2.090 ( 0.027) &    0.823 ( 0.009) &    0.949 ( 0.026) &   30.083 ( 0.226) &   31.475 ( 0.236) &    19.72 ( 2.15) &    19.58 ( 2.23)  &  0.08 &  7.3  &	q2   \\
    1353 &    1.900 ( 0.017) &    0.742 ( 0.006) &    0.863 ( 0.016) &   30.048 ( 0.081) &   31.605 ( 0.105) &    20.95 ( 1.01) &    20.77 ( 1.18)  &  0.13 &  8.8  &	q2   \\
    1355 &    2.290 ( 0.021) &    0.911 ( 0.007) &    1.084 ( 0.021) &   29.773 ( 0.101) &   31.008 ( 0.121) &    15.91 ( 0.89) &    15.79 ( 1.00)  &  1.33 & 27.3  &	q1   \\
    1366 &    2.158 ( 0.033) &    0.885 ( 0.014) &    1.053 ( 0.031) &   30.108 ( 0.237) &   31.469 ( 0.248) &    19.67 ( 2.24) &    19.31 ( 2.28)  &  0.06 &  6.0  &	q3   \\
    1368 &    2.399 ( 0.018) &    0.936 ( 0.008) &    1.175 ( 0.017) &   29.799 ( 0.050) &   30.946 ( 0.083) &    15.46 ( 0.59) &    15.48 ( 0.74)  &  2.96 & 47.6  &	q2   \\
    1369 &    2.015 ( 0.023) &    0.808 ( 0.009) &    0.971 ( 0.021) &   29.748 ( 0.048) &   31.211 ( 0.084) &    17.46 ( 0.67) &    17.19 ( 0.83)  &  0.06 &  6.1  &	q2   \\
    1379 &    1.449 ( 0.149) &    0.710 ( 0.031) &    0.770 ( 0.148) &   29.101 ( 0.143) &   31.166 ( 0.311) &    17.11 ( 2.45) &    15.30 ( 1.94)  &  0.64 & 52.3  &	q3   \\
    1386 &    2.269 ( 0.036) &    0.935 ( 0.009) &    1.086 ( 0.035) &   29.741 ( 0.087) &   30.985 ( 0.113) &    15.74 ( 0.82) &    15.45 ( 0.93)  &  1.55 & 29.8  &	q2   \\
    1389 &    2.144 ( 0.017) &    0.824 ( 0.006) &    1.020 ( 0.016) &   30.059 ( 0.065) &   31.408 ( 0.093) &    19.13 ( 0.82) &    19.19 ( 0.99)  &  0.19 & 10.9  &	q2   \\
    1392 &    2.398 ( 0.024) &    0.908 ( 0.009) &    1.199 ( 0.022) &   29.720 ( 0.118) &   30.848 ( 0.136) &    14.78 ( 0.93) &    14.97 ( 1.03)  &  1.05 & 25.4  &	q2   \\
    1396 &    2.189 ( 0.037) &    0.890 ( 0.014) &    1.058 ( 0.034) &   29.739 ( 0.165) &   31.054 ( 0.181) &    16.25 ( 1.36) &    15.97 ( 1.41)  &  0.10 &  8.3  &	q2   \\
    1399 &    2.099 ( 0.023) &    0.807 ( 0.008) &    0.944 ( 0.022) &   29.665 ( 0.067) &   31.054 ( 0.096) &    16.25 ( 0.72) &    16.29 ( 0.88)  &  0.11 &  8.0  &	q2   \\
    1407 &    2.312 ( 0.006) &    0.929 ( 0.003) &    1.118 ( 0.005) &   29.875 ( 0.133) &   31.089 ( 0.147) &    16.51 ( 1.12) &    16.30 ( 1.19)  &  0.15 &  9.6  &	q1   \\
    1411 &    1.763 ( 0.056) &    0.689 ( 0.021) &    0.803 ( 0.054) &   29.797 ( 0.077) &   31.497 ( 0.124) &    19.93 ( 1.14) &    19.61 ( 1.37)  &  0.20 & 17.7  &	q2   \\
    1412 &    2.845 ( 0.007) &    1.098 ( 0.002) &    1.350 ( 0.007) &   30.437 ( 0.053) &   31.105 ( 0.094) &    16.63 ( 0.72) &    16.57 ( 0.65)  &  1.07 & 38.7  &	q2   \\
    1414 &    2.033 ( 0.020) &    0.816 ( 0.007) &    0.922 ( 0.019) &   30.093 ( 0.246) &   31.535 ( 0.255) &    20.28 ( 2.38) &    20.01 ( 2.44)  &  0.06 &  6.0  &	q2   \\
    1417 &    2.276 ( 0.024) &    0.870 ( 0.009) &    1.074 ( 0.023) &   29.889 ( 0.153) &   31.132 ( 0.168) &    16.84 ( 1.30) &    16.89 ( 1.41)  &  0.49 & 17.0  &	q2   \\
    1418 &    2.091 ( 0.031) &    0.796 ( 0.011) &    0.953 ( 0.029) &   30.436 ( 0.158) &   31.834 ( 0.174) &    23.26 ( 1.86) &    23.37 ( 2.02)  &  0.05 &  6.2  &	q2   \\
    1419 &    2.264 ( 0.033) &    0.840 ( 0.010) &    1.097 ( 0.032) &   29.917 ( 0.152) &   31.168 ( 0.168) &    17.12 ( 1.33) &    17.37 ( 1.45)  &  2.64 & 44.2  &	q2   \\
    1420 &    2.210 ( 0.013) &    0.888 ( 0.006) &    1.042 ( 0.012) &   29.934 ( 0.080) &   31.232 ( 0.103) &    17.63 ( 0.84) &    17.44 ( 0.96)  &  0.09 &  7.4  &	q2   \\
    1422 &    2.288 ( 0.025) &    0.888 ( 0.006) &    1.049 ( 0.024) &   29.749 ( 0.083) &   30.982 ( 0.108) &    15.72 ( 0.78) &    15.74 ( 0.93)  &  2.88 & 40.2  &	q1   \\
    1426 &    1.978 ( 0.052) &    0.786 ( 0.019) &    0.932 ( 0.050) &   29.239 ( 0.176) &   30.738 ( 0.196) &    14.05 ( 1.27) &    13.84 ( 1.36)  &  0.30 & 19.9  &	q2   \\
    1431 &    2.601 ( 0.013) &    1.012 ( 0.004) &    1.230 ( 0.013) &   29.970 ( 0.109) &   30.933 ( 0.134) &    15.37 ( 0.95) &    15.39 ( 0.91)  &  0.84 & 22.9  &	q1   \\
    1438 &    1.711 ( 0.196) &    0.666 ( 0.050) &    0.623 ( 0.192) &   29.293 ( 0.265) &   31.035 ( 0.378) &    16.10 ( 2.81) &    15.89 ( 2.75)  &  0.44 & 16.3  &	q3   \\
    1440 &    2.298 ( 0.020) &    0.882 ( 0.005) &    1.111 ( 0.019) &   29.742 ( 0.144) &   30.962 ( 0.159) &    15.58 ( 1.14) &    15.67 ( 1.23)  &  0.81 & 21.3  &	q1   \\
    1448 &    2.131 ( 0.031) &    0.823 ( 0.009) &    0.940 ( 0.030) &   29.533 ( 0.087) &   30.895 ( 0.113) &    15.10 ( 0.79) &    15.13 ( 0.94)  &  1.46 & 36.6  &	q2   \\
    1449 &    2.014 ( 0.059) &    0.779 ( 0.019) &    0.900 ( 0.057) &   29.784 ( 0.214) &   31.245 ( 0.232) &    17.74 ( 1.90) &    17.71 ( 1.99)  &  0.07 &  5.9  &	q3   \\
    1463 &    1.985 ( 0.042) &    0.784 ( 0.015) &    0.899 ( 0.040) &   29.650 ( 0.166) &   31.138 ( 0.184) &    16.89 ( 1.43) &    16.73 ( 1.54)  &  0.03 &  4.7  &	q3   \\
    1475 &    2.282 ( 0.021) &    0.892 ( 0.005) &    1.102 ( 0.021) &   29.862 ( 0.091) &   31.100 ( 0.114) &    16.59 ( 0.87) &    16.57 ( 0.99)  &  1.88 & 35.3  &	q1   \\
    1488 &    1.899 ( 0.011) &    0.696 ( 0.003) &    0.841 ( 0.010) &   29.659 ( 0.088) &   31.214 ( 0.109) &    17.49 ( 0.88) &    17.62 ( 1.03)  &  0.14 & 10.9  &	q1   \\
    1489 &    2.056 ( 0.031) &    0.806 ( 0.008) &    0.916 ( 0.031) &   29.647 ( 0.085) &   31.078 ( 0.111) &    16.43 ( 0.84) &    16.35 ( 1.01)  &  0.40 & 15.3  &	q1   \\
    1491 &    2.405 ( 0.007) &    0.942 ( 0.002) &    1.134 ( 0.006) &   29.854 ( 0.124) &   30.980 ( 0.140) &    15.70 ( 1.01) &    15.64 ( 1.11)  &  0.17 & 10.0  &	q2   \\
    1499 &    1.778 ( 0.054) &    0.691 ( 0.017) &    0.778 ( 0.053) &   29.283 ( 0.171) &   30.962 ( 0.195) &    15.57 ( 1.40) &    15.41 ( 1.48)  &  0.07 & 15.9  &	q2   \\
    1509 &    2.077 ( 0.059) &    0.742 ( 0.013) &    0.878 ( 0.059) &   29.735 ( 0.088) &   31.138 ( 0.125) &    16.89 ( 0.97) &    17.35 ( 1.17)  &  0.27 & 12.5  &	q2   \\
    1512 &    2.530 ( 0.028) &    1.017 ( 0.008) &    1.217 ( 0.027) &   30.400 ( 0.078) &   31.434 ( 0.113) &    19.36 ( 1.01) &    19.19 ( 0.98)  &  0.20 & 12.1  &	q1   \\
    1514 &    2.110 ( 0.035) &    0.819 ( 0.013) &    0.944 ( 0.034) &   29.634 ( 0.115) &   31.007 ( 0.137) &    15.90 ( 1.00) &    15.87 ( 1.14)  &  1.23 & 26.7  &	q2   \\
    1516 &    1.685 ( 0.028) &    0.604 ( 0.006) &    0.762 ( 0.028) &   29.180 ( 0.062) &   30.940 ( 0.097) &    15.41 ( 0.69) &    15.36 ( 0.86)  &  0.42 & 30.1  &	q2   \\
    1522 &    1.774 ( 0.144) &    0.834 ( 0.047) &    0.716 ( 0.140) &   29.152 ( 0.347) &   30.852 ( 0.400) &    14.81 ( 2.73) &    13.93 ( 2.52)  &  0.03 &  4.5  &	q3   \\
    1523 &    2.135 ( 0.028) &    0.857 ( 0.010) &    0.989 ( 0.025) &   30.125 ( 0.166) &   31.488 ( 0.180) &    19.84 ( 1.65) &    19.65 ( 1.74)  &  0.04 &  5.0  &	q2   \\
    1528 &    2.407 ( 0.005) &    0.943 ( 0.002) &    1.125 ( 0.004) &   29.948 ( 0.137) &   31.069 ( 0.151) &    16.36 ( 1.14) &    16.26 ( 1.23)  &  0.22 & 12.1  &	q1   \\
    1535 &    2.637 ( 0.005) &    1.021 ( 0.002) &    1.308 ( 0.005) &   30.504 ( 0.098) &   31.368 ( 0.124) &    18.78 ( 1.08) &    18.57 ( 1.00)  &  1.57 & 54.4  &	q2   \\
    1536 &    2.056 ( 0.064) &    0.820 ( 0.027) &    0.971 ( 0.061) &   29.560 ( 0.233) &   30.997 ( 0.251) &    15.83 ( 1.83) &    15.63 ( 1.92)  &  0.07 &  6.8  &	q3   \\
    1537 &    2.403 ( 0.032) &    0.942 ( 0.009) &    1.154 ( 0.031) &   30.041 ( 0.110) &   31.188 ( 0.131) &    17.29 ( 1.05) &    17.27 ( 1.18)  &  2.70 & 44.3  &	q1   \\
    1539 &    2.273 ( 0.014) &    0.899 ( 0.005) &    1.069 ( 0.012) &   30.237 ( 0.144) &   31.484 ( 0.158) &    19.80 ( 1.44) &    19.68 ( 1.54)  &  0.10 &  8.2  &	q1   \\
    1545 &    2.524 ( 0.004) &    0.970 ( 0.002) &    1.174 ( 0.003) &   29.771 ( 0.060) &   30.797 ( 0.098) &    14.43 ( 0.65) &    14.55 ( 0.64)  &  0.10 &  8.0  &	q1   \\
    1552 &    2.492 ( 0.007) &    0.965 ( 0.003) &    1.194 ( 0.007) &   30.086 ( 0.171) &   31.147 ( 0.183) &    16.96 ( 1.43) &    16.98 ( 1.52)  &  2.20 & 45.6  &	q2   \\
    1561 &    2.172 ( 0.037) &    0.838 ( 0.014) &    1.033 ( 0.037) &   29.732 ( 0.116) &   31.065 ( 0.138) &    16.33 ( 1.04) &    16.37 ( 1.17)  &  0.25 & 13.0  &	q2   \\
    1563 &    2.094 ( 0.028) &    0.826 ( 0.011) &    0.932 ( 0.027) &   29.633 ( 0.089) &   31.039 ( 0.114) &    16.14 ( 0.85) &    16.06 ( 1.00)  &  0.23 & 11.3  &	q2   \\
    1588 &    2.134 ( 0.024) &    0.827 ( 0.006) &    1.018 ( 0.024) &   29.834 ( 0.034) &   31.203 ( 0.077) &    17.40 ( 0.62) &    17.42 ( 0.81)  &  0.50 & 47.7  &	q2   \\
    1615 &    2.514 ( 0.024) &    0.911 ( 0.012) &    1.248 ( 0.023) &   30.370 ( 0.109) &   31.401 ( 0.136) &    19.06 ( 1.19) &    19.61 ( 1.33)  &  2.64 & 129.3  &	q2   \\
    1619 &    2.291 ( 0.016) &    0.924 ( 0.007) &    1.104 ( 0.015) &   29.590 ( 0.073) &   30.831 ( 0.099) &    14.66 ( 0.67) &    14.48 ( 0.77)  &  2.06 & 40.7  &	q1   \\
    1627 &    2.702 ( 0.005) &    1.020 ( 0.003) &    1.276 ( 0.005) &   30.158 ( 0.070) &   30.979 ( 0.104) &    15.70 ( 0.75) &    15.94 ( 0.71)  &  0.13 &  9.3  &	q1   \\
    1630 &    2.792 ( 0.008) &    1.086 ( 0.004) &    1.314 ( 0.008) &   30.454 ( 0.060) &   31.161 ( 0.098) &    17.07 ( 0.77) &    16.80 ( 0.70)  &  2.43 & 39.4  &	q1   \\
    1632 &    2.822 ( 0.002) &    1.085 ( 0.001) &    1.383 ( 0.002) &   30.458 ( 0.087) &   31.129 ( 0.116) &    16.82 ( 0.90) &    16.74 ( 0.84)  &  4.07 & 51.3  &	q1   \\
    1661 &    2.392 ( 0.019) &    0.938 ( 0.008) &    1.101 ( 0.018) &   29.942 ( 0.249) &   31.065 ( 0.258) &    16.33 ( 1.94) &    16.19 ( 1.93)  &  0.28 & 12.5  &	q1   \\
    1664 &    2.579 ( 0.012) &    0.981 ( 0.004) &    1.251 ( 0.012) &   30.192 ( 0.081) &   31.147 ( 0.112) &    16.96 ( 0.88) &    17.12 ( 0.83)  &  3.81 & 54.0  &	q1   \\
    1690 &    2.039 ( 0.042) &    0.701 ( 0.017) &    1.052 ( 0.041) &   29.750 ( 0.106) &   31.211 ( 0.132) &    17.47 ( 1.06) &    18.09 ( 1.23)  &  2.98 & 132.0  &	q2   \\
    1692 &    2.345 ( 0.044) &    0.937 ( 0.012) &    1.204 ( 0.041) &   30.040 ( 0.106) &   31.210 ( 0.131) &    17.46 ( 1.05) &    17.15 ( 1.13)  &  3.20 & 61.5  &	q1   \\
    1695 &    2.210 ( 0.017) &    0.849 ( 0.007) &    1.024 ( 0.017) &   29.776 ( 0.086) &   31.090 ( 0.109) &    16.52 ( 0.83) &    16.60 ( 0.98)  &  1.29 & 26.9  &	q1   \\
    1696 &    2.119 ( 0.034) &    0.834 ( 0.014) &    1.122 ( 0.033) &   30.061 ( 0.152) &   31.454 ( 0.168) &    19.53 ( 1.52) &    19.47 ( 1.62)  &  1.80 & 99.8  &	q2   \\
    1720 &    2.609 ( 0.008) &    0.970 ( 0.003) &    1.232 ( 0.008) &   30.276 ( 0.082) &   31.170 ( 0.113) &    17.14 ( 0.89) &    17.36 ( 0.84)  &  5.56 & 56.3  &	q1   \\
    1727 &    2.457 ( 0.012) &    0.934 ( 0.005) &    1.221 ( 0.011) &   30.474 ( 0.119) &   31.565 ( 0.136) &    20.56 ( 1.29) &    20.87 ( 1.43)  &  1.24 & 114.7  &	q2   \\
    1730 &    2.435 ( 0.018) &    0.936 ( 0.009) &    1.203 ( 0.017) &   30.140 ( 0.080) &   31.228 ( 0.113) &    17.60 ( 0.91) &    17.66 ( 1.02)  &  2.71 & 57.8  &	q2   \\
    1743 &    2.209 ( 0.022) &    0.831 ( 0.009) &    1.008 ( 0.021) &   29.729 ( 0.174) &   31.016 ( 0.187) &    15.97 ( 1.38) &    16.07 ( 1.47)  &  0.54 & 17.6  &	q1   \\
    1779 &    1.865 ( 0.084) &    0.724 ( 0.030) &    0.798 ( 0.083) &   29.172 ( 0.151) &   30.765 ( 0.192) &    14.22 ( 1.26) &    14.12 ( 1.34)  &  0.56 & 26.2  &	q1   \\
    1809 &    2.135 ( 0.056) &    0.835 ( 0.019) &    0.942 ( 0.052) &   29.617 ( 0.169) &   30.986 ( 0.190) &    15.75 ( 1.38) &    15.72 ( 1.49)  &  0.78 & 29.2  &	q2   \\
    1811 &    1.767 ( 0.033) &    0.636 ( 0.013) &    0.822 ( 0.033) &   29.215 ( 0.063) &   30.917 ( 0.100) &    15.25 ( 0.70) &    15.26 ( 0.88)  &  0.30 & 36.5  &	q2   \\
    1813 &    2.705 ( 0.007) &    0.993 ( 0.003) &    1.257 ( 0.006) &   30.390 ( 0.101) &   31.166 ( 0.127) &    17.11 ( 1.00) &    17.53 ( 0.97)  &  7.66 & 74.8  &	q2   \\
    1826 &    2.255 ( 0.014) &    0.882 ( 0.005) &    1.033 ( 0.013) &   29.748 ( 0.089) &   30.993 ( 0.110) &    15.80 ( 0.80) &    15.72 ( 0.93)  &  0.28 & 12.7  &	q1   \\
    1828 &    2.368 ( 0.018) &    0.914 ( 0.006) &    1.098 ( 0.017) &   29.795 ( 0.073) &   30.964 ( 0.098) &    15.59 ( 0.71) &    15.68 ( 0.85)  &  0.60 & 18.8  &	q1   \\
    1833 &    2.387 ( 0.018) &    0.889 ( 0.004) &    1.106 ( 0.018) &   29.978 ( 0.050) &   31.128 ( 0.083) &    16.81 ( 0.64) &    17.01 ( 0.83)  &  0.58 & 19.2  &	q1   \\
    1851 &    2.068 ( 0.039) &    0.800 ( 0.016) &    0.941 ( 0.037) &   29.309 ( 0.241) &   30.720 ( 0.252) &    13.93 ( 1.62) &    13.92 ( 1.69)  &  0.04 &  6.6  &	q3   \\
    1857 &    1.615 ( 0.045) &    0.592 ( 0.017) &    0.755 ( 0.044) &   29.241 ( 0.122) &   31.085 ( 0.153) &    16.48 ( 1.16) &    16.40 ( 1.30)  &  0.81 & 28.0  &	q2   \\
    1859 &    2.116 ( 0.021) &    0.791 ( 0.006) &    0.981 ( 0.021) &   29.591 ( 0.101) &   30.971 ( 0.122) &    15.64 ( 0.88) &    15.68 ( 1.01)  &  0.68 & 39.3  &	q2   \\
    1861 &    2.459 ( 0.008) &    0.946 ( 0.003) &    1.143 ( 0.008) &   29.774 ( 0.063) &   30.847 ( 0.099) &    14.77 ( 0.68) &    14.83 ( 0.67)  &  0.73 & 20.0  &	q1   \\
    1869 &    2.832 ( 0.004) &    1.037 ( 0.001) &    1.297 ( 0.003) &   30.590 ( 0.083) &   31.172 ( 0.113) &    17.16 ( 0.89) &    17.74 ( 0.86)  &  1.76 & 54.7  &	q2   \\
    1870 &    2.036 ( 0.028) &    0.750 ( 0.010) &    0.912 ( 0.027) &   29.585 ( 0.104) &   31.029 ( 0.126) &    16.07 ( 0.93) &    16.21 ( 1.08)  &  0.30 & 13.4  &	q2   \\
    1871 &    2.704 ( 0.026) &    0.987 ( 0.010) &    1.259 ( 0.024) &   29.906 ( 0.209) &   30.707 ( 0.224) &    13.85 ( 1.43) &    14.23 ( 1.45)  &  2.91 & 40.0  &	q1   \\
    1879 &    2.073 ( 0.046) &    0.791 ( 0.016) &    0.931 ( 0.044) &   29.904 ( 0.253) &   31.317 ( 0.265) &    18.34 ( 2.24) &    18.43 ( 2.35)  &  0.20 & 10.9  &	q2   \\
    1883 &    2.444 ( 0.002) &    0.953 ( 0.001) &    1.182 ( 0.002) &   30.151 ( 0.128) &   31.232 ( 0.150) &    17.63 ( 1.22) &    17.54 ( 1.17)  &  0.80 & 23.7  &	q1   \\
    1886 &    2.097 ( 0.029) &    0.743 ( 0.009) &    0.943 ( 0.029) &   29.059 ( 0.112) &   30.457 ( 0.132) &    12.34 ( 0.75) &    12.52 ( 0.87)  &  0.59 & 19.8  &	q1   \\
    1895 &    2.133 ( 0.025) &    0.840 ( 0.007) &    0.985 ( 0.024) &   29.413 ( 0.088) &   30.763 ( 0.112) &    14.21 ( 0.73) &    14.11 ( 0.85)  &  0.79 & 21.1  &	q1   \\
    1903 &    2.759 ( 0.002) &    1.057 ( 0.001) &    1.353 ( 0.002) &   30.263 ( 0.046) &   30.999 ( 0.090) &    15.84 ( 0.65) &    15.81 ( 0.58)  &  2.63 & 49.3  &	q1   \\
    1910 &    2.586 ( 0.009) &    0.991 ( 0.003) &    1.251 ( 0.008) &   29.964 ( 0.121) &   30.907 ( 0.143) &    15.18 ( 1.00) &    15.26 ( 0.96)  &  0.82 & 22.2  &	q1   \\
    1938 &    2.558 ( 0.019) &    0.937 ( 0.006) &    1.226 ( 0.019) &   30.212 ( 0.066) &   31.174 ( 0.103) &    17.17 ( 0.82) &    17.45 ( 0.82)  &  3.08 & 55.8  &	q1   \\
    1943 &    1.927 ( 0.069) &    0.665 ( 0.023) &    0.929 ( 0.067) &   30.014 ( 0.194) &   31.549 ( 0.219) &    20.41 ( 2.06) &    20.81 ( 2.23)  &  0.94 & 63.7  &	q2   \\
    1948 &    2.005 ( 0.026) &    0.753 ( 0.008) &    0.899 ( 0.025) &   29.549 ( 0.095) &   31.017 ( 0.118) &    15.97 ( 0.87) &    16.08 ( 1.01)  &  0.61 & 19.1  &	q1   \\
    1978 &    2.964 ( 0.001) &    1.098 ( 0.000) &    1.427 ( 0.001) &   30.638 ( 0.067) &   31.034 ( 0.102) &    16.10 ( 0.76) &    16.48 ( 0.71)  &  3.04 & 47.2  &	q1   \\
    1987 &    1.754 ( 0.056) &    0.612 ( 0.019) &    0.959 ( 0.054) &   29.386 ( 0.109) &   31.084 ( 0.145) &    16.48 ( 1.10) &    16.93 ( 1.22)  &  1.29 & 91.7  &	q2   \\
    1993 &    2.301 ( 0.023) &    0.884 ( 0.007) &    1.056 ( 0.021) &   29.904 ( 0.088) &   31.120 ( 0.111) &    16.75 ( 0.86) &    16.83 ( 1.01)  &  0.56 & 17.4  &	q1   \\
    1999 &    2.487 ( 0.007) &    0.934 ( 0.002) &    1.195 ( 0.007) &   30.070 ( 0.083) &   31.107 ( 0.113) &    16.65 ( 0.87) &    16.83 ( 0.87)  &  1.00 & 26.3  &	q1   \\
    2000 &    2.242 ( 0.023) &    0.894 ( 0.007) &    1.060 ( 0.022) &   29.606 ( 0.055) &   30.881 ( 0.087) &    15.01 ( 0.60) &    14.88 ( 0.74)  &  3.57 & 55.1  &	q1   \\
    2019 &    2.271 ( 0.029) &    0.854 ( 0.006) &    1.045 ( 0.028) &   29.888 ( 0.083) &   31.125 ( 0.109) &    16.79 ( 0.84) &    16.88 ( 1.01)  &  1.38 & 27.7  &	q1   \\
    2048 &    2.230 ( 0.028) &    0.872 ( 0.014) &    1.029 ( 0.027) &   29.693 ( 0.106) &   30.977 ( 0.127) &    15.68 ( 0.92) &    15.66 ( 1.05)  &  2.44 & 38.5  &	q2   \\
    2050 &    2.264 ( 0.020) &    0.864 ( 0.008) &    1.012 ( 0.019) &   29.707 ( 0.053) &   30.952 ( 0.085) &    15.50 ( 0.61) &    15.61 ( 0.78)  &  0.63 & 18.9  &	q1   \\
    2058 &    2.189 ( 0.027) &    0.863 ( 0.010) &    1.109 ( 0.026) &   29.911 ( 0.112) &   31.220 ( 0.132) &    17.54 ( 1.07) &    17.41 ( 1.17)  &  2.08 & 88.2  &	q2   \\
    2066 &    1.986 ( 0.037) &    0.751 ( 0.017) &    0.911 ( 0.037) &   29.643 ( 0.129) &   31.142 ( 0.150) &    16.92 ( 1.17) &    16.95 ( 1.31)  &  1.65 & 63.0  &	q2   \\
    2087 &    2.473 ( 0.015) &    0.944 ( 0.004) &    1.179 ( 0.014) &   30.211 ( 0.070) &   31.253 ( 0.105) &    17.81 ( 0.86) &    17.88 ( 0.80)  &  3.71 & 49.4  &	q2   \\
    2092 &  \nodata          &    1.053 ( 0.002) &    1.325 ( 0.007) &   30.255 ( 0.061) &   30.994 ( 0.077) &    15.81 ( 0.56) &    15.81 ( 0.56)  &  3.67 & 55.0  &	q1   \\
    2095 &  \nodata          &    0.875 ( 0.005) &    1.223 ( 0.015) &   30.022 ( 0.080) &   31.129 ( 0.119) &    16.82 ( 0.93) &    16.82 ( 0.93)  &  2.63 & 53.3  &	q2   \\
    NGVSJ12:31:52.90+12:15:59.1 &    2.415 ( 0.040) &    0.956 ( 0.018) &    1.224 ( 0.036) &   30.300 ( 0.102) &   31.409 ( 0.127) &    19.13 ( 1.12) &    18.87 ( 1.11)  &  0.03 &  4.3  &	    q2 	\\
    NGVSJ12:29:33.61+13:11:44.6 &    1.154 ( 0.048) &    0.376 ( 0.019) &    0.455 ( 0.047) &   28.638 ( 0.144) &   31.180 ( 0.199) &    17.22 ( 1.58) &    17.72 ( 2.04)  &  0.03 &  4.1  &	    q3   \\
    NGVSJ12:33:40.31+12:44:13.6 &    2.043 ( 0.041) &    0.814 ( 0.016) &    0.990 ( 0.039) &   30.386 ( 0.211) &   31.825 ( 0.225) &    23.17 ( 2.40) &    22.92 ( 2.47)  &  0.04 &  4.6  &	    q3   \\
\\
\enddata
\tablecomments{This table is available in its entirety in a machine-readable form in the online journal. A portion is shown here for guidance regarding its form and content. All magnitudes are  AB~mag.}
\label{tab_measures}
\end{deluxetable*}




==> Tables/table_models.tex <==
\begin{table*}{lcccccc}
\tablecaption{Integrated colors and SBF magnitudes from the SPoT Simple Stellar Population models.}
\tablehead{
  \colhead{$[Fe/H]$} &
  \colhead{Age (Gyr)} &
  \colhead{$u^*{-}i$} &
  \colhead{$g{-}i$} &
  \colhead{$u^*{-}z$} &
  \colhead{$g{-}z$} &
  \colhead{$\overline{M}_i$} 
  } \startdata
      (1)&   (2)      &     (3)      &        (4)   &    (5)   &  (6)   &    (7)     \\   
\hline
   -0.35 &      1 &     1.518 &     0.588 &     1.676 &     0.746 &    -2.083  \\
   -0.35 &      2 &     1.730 &     0.707 &     1.878 &     0.855 &    -1.581  \\
   -0.35 &      3 &     1.887 &     0.789 &     2.052 &     0.954 &    -1.482  \\
   -0.35 &      4 &     1.961 &     0.825 &     2.135 &     0.999 &    -1.348  \\
   -0.35 &      6 &     2.044 &     0.858 &     2.221 &     1.035 &    -1.344  \\
   -0.35 &      8 &     2.143 &     0.907 &     2.339 &     1.103 &    -1.084  \\
   -0.35 &     10 &     2.214 &     0.937 &     2.418 &     1.141 &    -1.035  \\
   -0.35 &     12 &     2.256 &     0.952 &     2.466 &     1.162 &    -0.996  \\
   -0.35 &     14 &     2.309 &     0.974 &     2.525 &     1.190 &    -0.977  \\
   \hline
    0.00 &      1 &     1.638 &     0.640 &     1.813 &     0.815 &    -1.262  \\
    0.00 &      2 &     1.950 &     0.804 &     2.154 &     1.008 &    -1.067  \\
    0.00 &      3 &     2.113 &     0.880 &     2.339 &     1.106 &    -0.950  \\
    0.00 &      4 &     2.218 &     0.925 &     2.459 &     1.166 &    -0.859  \\
    0.00 &      6 &     2.332 &     0.968 &     2.574 &     1.210 &    -0.796  \\
    0.00 &      8 &     2.427 &     1.009 &     2.686 &     1.268 &    -0.732  \\
    0.00 &     10 &     2.505 &     1.041 &     2.777 &     1.313 &    -0.586  \\
    0.00 &     12 &     2.575 &     1.068 &     2.855 &     1.348 &    -0.497  \\
    0.00 &     14 &     2.638 &     1.094 &     2.925 &     1.381 &    -0.485  \\
    \hline
    0.40 &      1 &     1.889 &     0.762 &     2.104 &     0.977 &    -0.828  \\
    0.40 &      2 &     2.120 &     0.867 &     2.351 &     1.098 &    -0.448  \\
    0.40 &      3 &     2.282 &     0.934 &     2.525 &     1.177 &    -0.263  \\
    0.40 &      4 &     2.377 &     0.973 &     2.629 &     1.225 &    -0.149  \\
    0.40 &      6 &     2.507 &     1.027 &     2.770 &     1.290 &    -0.191  \\
    0.40 &      8 &     2.614 &     1.070 &     2.887 &     1.343 &    -0.115  \\
    0.40 &     10 &     2.705 &     1.109 &     2.992 &     1.396 &    -0.008  \\
    0.40 &     12 &     2.775 &     1.139 &     3.070 &     1.434 &     0.090  \\
    0.40 &     14 &     2.837 &     1.165 &     3.139 &     1.467 &     0.118  \\
\\
\enddata
\label{tab_models}
\end{table*}


==> table_data_ref_full.tex <==
\startlongtable
\begin{deluxetable}{lllcccccc}
%\tabletypesize{\footnotesize}
\tabletypesize{\scriptsize}
\tablecaption{Sample basic properties, colors, SBF and distances (Excerpt)}
\tablehead{
  \colhead{VCC} &
  \colhead{Alt. Name} &
  \colhead{IAU Name} &
  \colhead{RA (J2000)} &
  \colhead{Dec (J2000)} &
  \colhead{$B_T$} &
  \colhead{\tiny{$E(B{-}V)$}} &
  \colhead{$v_{Helio}$} &
  \colhead{$T_{Type}$} &
  \\
  \colhead{   } &
  \colhead{         } &
  \colhead{   (deg)  } &
  \colhead{  (deg)    } &
  \colhead{(mag)} &
  \colhead{ (mag)           } &
  \colhead{\kms       } &
  \colhead{          } &
  } \startdata
      (1)&   (2)      &     (3)      &        (4)   &    (5)   &  (6)   &    (7)  &      (8)     \\   
\hline
      32 & IC0767    & NGVSJ12:11:02.73+12:06:14.4  182.7613724 &   12.1039918 &    14.00 &  0.027 &    1877 &   -5.0 (  1.0) \\
      33 & IC3032    & NGVSJ12:11:07.76+14:16:29.3  182.7823394 &   14.2748006 &    14.70 &  0.038 &    1179 &   -4.0 (  1.8) \\
      49 & NGC4168   & NGVSJ12:12:17.26+13:12:18.7  183.0719332 &   13.2051960 &    12.20 &  0.037 &    2273 &   -4.9 (  0.4) \\
      66 & NGC4178   & NGVSJ12:12:46.57+10:51:59.8  183.1940241 &   10.8666242 &    11.90 &  0.028 &     374 &    6.9 (  1.2) \\
      89 & NGC4189   & NGVSJ12:13:47.24+13:25:29.5  183.4468247 &   13.4248521 &    12.50 &  0.033 &    2098 &    5.9 (  0.9) \\
      92 & NGC4192   & NGVSJ12:13:48.29+14:54:01.8  183.4512262 &   14.9005060 &    10.90 &  0.035 &    -142 &    2.6 (  0.8) \\
     107 & PGC039071 & NGVSJ12:14:09.75+13:14:00.5  183.5406147 &   13.2334632 &    19.40 &  0.030 & \nodata &   -5.0 (  2.0) \\
     140 & IC3065    & NGVSJ12:15:12.56+14:25:58.4  183.8023507 &   14.4328799 &    14.30 &  0.036 &     995 &   -2.2 (  1.2) \\
     145 & NGC4206   & NGVSJ12:15:16.82+13:01:26.4  183.8200770 &   13.0239966 &    12.80 &  0.032 &     703 &    4.0 (  0.3) \\
     157 & NGC4212   & NGVSJ12:15:39.34+13:54:05.4  183.9138976 &   13.9015055 &    11.90 &  0.033 &     -88 &    4.9 (  0.8) \\
     167 & NGC4216   & NGVSJ12:15:54.39+13:08:58.0  183.9766077 &   13.1494566 &    11.00 &  0.032 &     131 &    3.0 (  0.5) \\
     199 & NGC4224   & NGVSJ12:16:33.79+07:27:43.4  184.1407813 &    7.4620674 &    12.90 &  0.024 &    2584 &    1.0 (  0.3) \\
     200 & PGC039331 & NGVSJ12:16:33.71+13:01:53.7  184.1404477 &   13.0315970 &    14.70 &  0.030 &       8 &   -4.3 (  1.6) \\
     220 & NGC4233   & NGVSJ12:17:07.68+07:37:27.4  184.2820056 &    7.6242759 &    13.00 &  0.024 &    2275 &   -2.0 (  0.5) \\
     222 & NGC4235   & NGVSJ12:17:09.88+07:11:29.7  184.2911844 &    7.1915747 &    12.70 &  0.019 &    2263 &    1.0 (  0.4) \\
     226 & NGC4237   & NGVSJ12:17:11.43+15:19:26.5  184.2976068 &   15.3240384 &    12.50 &  0.030 &     864 &    4.0 (  0.5) \\
     230 & IC3101    & NGVSJ12:17:19.65+11:56:36.5  184.3318761 &   11.9434644 &    15.20 &  0.028 &    1430 &   -5.0 (  1.4) \\
     263 & PGC039475 & NGVSJ12:17:56.83+11:59:45.7  184.4868025 &   11.9960324 &    18.20 &  0.030 & \nodata &   -5.0 (  3.0) \\
     308 & IC3131    & NGVSJ12:18:50.89+07:51:43.1  184.7120270 &    7.8619797 &    13.70 &  0.021 &    1530 &   -3.5 (  1.8) \\
     315 & PGC039606 & NGVSJ12:19:00.55+06:05:40.6  184.7523115 &    6.0946187 &    14.80 &  0.023 &    1589 &    0.5 (  1.0) \\
     341 & NGC4260   & NGVSJ12:19:22.25+06:05:55.2  184.8427241 &    6.0986724 &    12.70 &  0.023 &    1776 &    1.0 (  0.5) \\
     345 & NGC4261   & NGVSJ12:19:23.22+05:49:29.6  184.8467458 &    5.8248971 &    11.30 &  0.018 &    2177 &   -4.8 (  0.4) \\
     355 & NGC4262   & NGVSJ12:19:30.57+14:52:39.6  184.8773845 &   14.8776534 &    12.40 &  0.036 &    1359 &   -2.6 (  0.7) \\
     369 & NGC4267   & NGVSJ12:19:45.28+12:47:53.7  184.9386693 &   12.7982620 &    11.80 &  0.047 &    1021 &   -2.7 (  0.7) \\
     397 & PGC039772 & NGVSJ12:20:12.18+06:37:23.5  185.0507418 &    6.6231923 &    14.90 &  0.019 &    2442 &   -5.0 (  1.2) \\
     465 & NGC4294   & NGVSJ12:21:17.84+11:30:38.4  185.3243502 &   11.5106643 &    12.60 &  0.034 &     355 &    5.9 (  0.5) \\
     483 & NGC4298   & NGVSJ12:21:32.77+14:36:22.1  185.3865368 &   14.6061371 &    12.10 &  0.035 &    1124 &    5.1 (  0.6) \\
     490 & IC0783    & NGVSJ12:21:38.77+15:44:42.4  185.4115379 &   15.7451112 &    13.40 &  0.022 &    1267 &   -0.2 (  0.8) \\
     491 & NGC4299   & NGVSJ12:21:40.32+11:30:11.4  185.4180145 &   11.5031588 &    12.90 &  0.033 &     237 &    8.4 (  1.3) \\
     497 & NGC4302   & NGVSJ12:21:42.40+14:35:41.8  185.4266475 &   14.5949500 &    12.60 &  0.035 &    1098 &    5.3 (  0.8) \\
     523 & NGC4306   & NGVSJ12:22:04.12+12:47:15.0  185.5171828 &   12.7874979 &    13.10 &  0.042 &    1524 &   -2.0 (  0.8) \\
     524 & NGC4307   & NGVSJ12:22:05.66+09:02:37.2  185.5235656 &    9.0436564 &    12.80 &  0.023 &    1055 &    3.2 (  0.7) \\
     538 & PGC040059 & NGVSJ12:22:14.74+07:10:01.7  185.5614014 &    7.1671499 &    15.40 &  0.020 &     755 &   -5.0 (  1.2) \\
     543 & UGC07436  & NGVSJ12:22:19.53+14:45:38.8  185.5813776 &   14.7607696 &    14.40 &  0.031 &     977 &   -2.7 (  2.3) \\
     559 & NGC4312   & NGVSJ12:22:31.34+15:32:16.5  185.6305649 &   15.5379150 &    12.60 &  0.027 &     158 &    2.1 (  0.9) \\
     570 & NGC4313   & NGVSJ12:22:38.54+11:48:03.2  185.6606025 &   11.8008999 &    12.70 &  0.036 &    1431 &    2.1 (  0.4) \\
     571 & PGC040115 & NGVSJ12:22:41.10+07:57:01.4  185.6712666 &    7.9503803 &    14.70 &  0.022 &    1101 &   -1.8 (  1.3) \\
     575 & NGC4318   & NGVSJ12:22:43.29+08:11:53.8  185.6803578 &    8.1982639 &    14.10 &  0.025 &    1203 &   -4.7 (  0.9) \\
     596 & NGC4321   & NGVSJ12:22:54.91+15:49:20.2  185.7287922 &   15.8222817 &    10.10 &  0.026 &    1571 &    4.0 (  0.3) \\
     613 & NGC4324   & NGVSJ12:23:06.17+05:15:01.2  185.7757201 &    5.2503454 &    12.60 &  0.024 &    1667 &   -0.8 (  1.2) \\
     648 & NGC4339   & NGVSJ12:23:34.95+06:04:54.4  185.8956063 &    6.0817747 &    12.30 &  0.026 &    1266 &   -4.6 (  1.0) \\
     654 & NGC4340   & NGVSJ12:23:35.28+16:43:20.4  185.8970174 &   16.7223449 &    11.60 &  0.026 &     933 &   -1.2 (  0.6) \\
     657 & NGC4342   & NGVSJ12:23:39.00+07:03:14.4  185.9125041 &    7.0539981 &    12.60 &  0.020 &     761 &   -3.2 (  1.0) \\
     685 & NGC4350   & NGVSJ12:23:57.84+16:41:36.0  185.9910099 &   16.6933384 &    11.20 &  0.028 &    1210 &   -1.8 (  0.9) \\
     692 & NGC4351   & NGVSJ12:24:01.52+12:12:17.2  186.0063131 &   12.2047665 &    13.00 &  0.028 &    2325 &    2.8 (  1.7) \\
     698 & NGC4352   & NGVSJ12:24:05.03+11:13:05.1  186.0209443 &   11.2180718 &    13.60 &  0.026 &    2083 &   -2.0 (  0.4) \\
     731 & NGC4365   & NGVSJ12:24:28.26+07:19:04.0  186.1177300 &    7.3177697 &    10.50 &  0.021 &    1243 &   -4.8 (  0.4) \\
     750 & PGC040428 & NGVSJ12:24:49.57+06:45:34.4  186.2065252 &    6.7595615 &    14.80 &  0.028 &    1059 &   -5.0 (  1.0) \\
     759 & NGC4371   & NGVSJ12:24:55.43+11:42:15.1  186.2309734 &   11.7041966 &    11.80 &  0.036 &     933 &   -1.3 (  0.6) \\
     763 & NGC4374   & NGVSJ12:25:03.74+12:53:13.1  186.2656026 &   12.8869755 &    10.30 &  0.042 &    1017 &   -4.4 (  1.2) \\
     778 & NGC4377   & NGVSJ12:25:12.34+14:45:43.8  186.3014104 &   14.7621692 &    12.70 &  0.039 &    1338 &   -2.6 (  0.6) \\
     784 & NGC4379   & NGVSJ12:25:14.75+15:36:26.7  186.3114423 &   15.6074215 &    12.70 &  0.023 &    1074 &   -2.7 (  0.6) \\
     785 & NGC4378   & NGVSJ12:25:18.10+04:55:30.5  186.3254153 &    4.9251457 &    12.20 &  0.016 &    2559 &    1.0 (  0.3) \\
     792 & NGC4380   & NGVSJ12:25:22.17+10:01:00.5  186.3423910 &   10.0167929 &    12.40 &  0.024 &     963 &    2.4 (  0.9) \\
     801 & NGC4383   & NGVSJ12:25:25.46+16:28:11.8  186.3560921 &   16.4699454 &    12.70 &  0.024 &    1710 &    0.8 (  0.8) \\
     828 & NGC4387   & NGVSJ12:25:41.68+12:48:37.9  186.4236734 &   12.8105171 &    12.80 &  0.032 &     538 &   -4.8 (  0.6) \\
     836 & NGC4388   & NGVSJ12:25:46.72+12:39:42.9  186.4446712 &   12.6619044 &    11.80 &  0.033 &    2524 &    2.8 (  0.7) \\
     856 & IC3328    & NGVSJ12:25:57.92+10:03:13.6  186.4913357 &   10.0537778 &    14.20 &  0.024 &    1001 &   -3.8 (  1.7) \\
     865 & NGC4396   & NGVSJ12:25:59.15+15:40:13.6  186.4964753 &   15.6704560 &    13.00 &  0.026 &    -125 &    6.8 (  0.8) \\
     873 & NGC4402   & NGVSJ12:26:07.14+13:06:43.2  186.5297661 &   13.1119969 &    12.60 &  0.029 &     237 &    3.2 (  0.8) \\
     874 & NGC4405   & NGVSJ12:26:07.15+16:10:51.5  186.5298124 &   16.1809713 &    13.00 &  0.024 &    1735 &    0.3 (  1.1) \\
     881 & NGC4406   & NGVSJ12:26:11.76+12:56:46.5  186.5489811 &   12.9462404 &    10.10 &  0.029 &    -224 &   -4.8 (  0.5) \\
     896 & PGC040679 & NGVSJ12:26:22.61+12:47:11.0  186.5942075 &   12.7863945 &    17.70 &  0.030 &    2114 &   -5.0 (  1.2) \\
     898 & PGC040686 & NGVSJ12:26:23.64+13:22:24.7  186.5984901 &   13.3735172 &    18.30 &  0.030 &    1172 &   -5.0 (  3.0) \\
     912 & NGC4413   & NGVSJ12:26:32.25+12:36:38.5  186.6343910 &   12.6107082 &    12.40 &  0.032 &      69 &    2.1 (  1.1) \\
     916 & PGC040707 & NGVSJ12:26:33.21+12:44:34.7  186.6383646 &   12.7429799 &    15.60 &  0.030 &    1298 &   -5.0 (  1.2) \\
     923 & PGC040718 & NGVSJ12:26:36.32+12:48:10.0  186.6513420 &   12.8027898 &    18.20 &  0.030 &    1172 &   -5.0 (  1.4) \\
     928 & PGC040723 & NGVSJ12:26:39.81+12:30:48.8  186.6658930 &   12.5135530 &    15.90 &  0.032 &    -288 &   -5.0 (  1.0) \\
     929 & NGC4415   & NGVSJ12:26:40.49+08:26:08.5  186.6686939 &    8.4356972 &    13.10 &  0.022 &     907 &   -0.9 (  2.1) \\
     930 & PGC040725 & NGVSJ12:26:41.15+12:50:43.5  186.6714522 &   12.8454060 &    17.80 &  0.029 &    1172 &   -5.0 (  1.4) \\
     938 & NGC4416   & NGVSJ12:26:46.75+07:55:08.4  186.6947720 &    7.9189879 &    12.90 &  0.025 &    1399 &    5.9 (  0.5) \\
     939 & NGC4411B  & NGVSJ12:26:47.23+08:53:04.5  186.6968095 &    8.8845903 &    12.90 &  0.029 &    1272 &    6.2 (  0.9) \\
     940 & IC3349    & NGVSJ12:26:47.06+12:27:14.3  186.6961004 &   12.4539694 &    14.60 &  0.030 &    1392 &   -5.0 (  0.9) \\
     942 & PGC040753 & NGVSJ12:26:48.49+12:23:59.6  186.7020527 &   12.3998780 &    19.50 &  0.027 &    1172 &   -5.0 (  2.0) \\
     944 & NGC4417   & NGVSJ12:26:50.61+09:35:03.3  186.7108668 &    9.5842588 &    12.10 &  0.025 &     828 &   -1.9 (  0.5) \\
     950 & IC3356    & NGVSJ12:26:50.74+11:33:27.5  186.7114036 &   11.5576470 &    14.90 &  0.031 &    1100 &    9.7 (  1.0) \\
     951 & IC3358    & NGVSJ12:26:54.36+11:39:50.2  186.7265030 &   11.6639359 &    14.00 &  0.026 &    2106 &   -5.0 (  1.4) \\
     958 & NGC4419   & NGVSJ12:26:56.43+15:02:50.3  186.7351069 &   15.0473025 &    12.10 &  0.033 &    -261 &    1.2 (  0.9) \\
     962 & PGC040782 & NGVSJ12:26:59.05+12:30:20.5  186.7460570 &   12.5056882 &    16.90 &  0.028 &    1172 &   -5.0 (  2.0) \\
     965 & IC3363    & NGVSJ12:27:03.08+12:33:38.8  186.7628443 &   12.5607787 &    15.10 &  0.030 &     830 &   -5.0 (  1.0) \\
     966 & NGC4421   & NGVSJ12:27:02.54+15:27:41.3  186.7605852 &   15.4614659 &    12.40 &  0.024 &    1551 &   -0.5 (  0.8) \\
     967 & PGC040787 & NGVSJ12:27:03.81+12:51:59.2  186.7658563 &   12.8664417 &    18.20 &  0.029 &    1135 &   -5.0 (  1.2) \\
     968 & PGC040792 & NGVSJ12:27:06.07+13:19:25.3  186.7752955 &   13.3236918 &    18.00 &  0.026 &    1172 &   -5.0 (  3.0) \\
     972 & PGC040798 & NGVSJ12:27:08.42+13:20:08.7  186.7850718 &   13.3357445 &    16.40 &  0.025 &   14999 &   -5.0 (  2.0) \\
     977 & PGC040806 & NGVSJ12:27:11.24+12:02:17.4  186.7968529 &   12.0381804 &    17.70 &  0.025 &      57 &   -5.0 (  1.2) \\
     978 & PGC040805 & NGVSJ12:27:11.20+12:06:52.3  186.7966853 &   12.1145416 &    18.00 &  0.026 &    1172 &   -5.0 (  3.0) \\
     979 & NGC4424   & NGVSJ12:27:11.67+09:25:14.8  186.7986301 &    9.4207733 &    12.30 &  0.021 &     437 &    1.3 (  1.6) \\
     984 & NGC4425   & NGVSJ12:27:13.34+12:44:05.2  186.8055801 &   12.7347647 &    12.30 &  0.029 &    1892 &   -0.6 (  1.2) \\
     987 & PGC040823 & NGVSJ12:27:15.46+12:39:41.4  186.8144228 &   12.6615036 &    17.90 &  0.030 &    1172 &   -5.0 (  3.0) \\
     990 & IC3369    & NGVSJ12:27:16.94+16:01:28.1  186.8205856 &   16.0244642 &    14.30 &  0.029 &    1704 &   -3.3 (  1.9) \\
     996 & PGC040838 & NGVSJ12:27:21.11+13:06:40.3  186.8379500 &   13.1111947 &    17.80 &  0.029 &     -28 &   -5.0 (  1.2) \\
     997 & PGC040840 & NGVSJ12:27:22.17+12:04:07.4  186.8423851 &   12.0687121 &    17.40 &  0.026 &    -171 &   -5.0 (  1.2) \\
     998 & PGC040841 & NGVSJ12:27:23.46+12:19:54.1  186.8477404 &   12.3317052 &    17.50 &  0.029 & \nodata &   -5.0 (  2.0) \\
    1000 & PGC040846 & NGVSJ12:27:24.71+11:14:17.8  186.8529524 &   11.2382779 &    18.20 &  0.035 & \nodata &   -5.0 (  2.0) \\
    1003 & NGC4429   & NGVSJ12:27:26.52+11:06:27.7  186.8604863 &   11.1076843 &    11.20 &  0.033 &    1104 &   -0.8 (  1.5) \\
    1010 & NGC4431   & NGVSJ12:27:27.38+12:17:25.0  186.8640813 &   12.2902790 &    13.40 &  0.028 &     930 &   -2.1 (  0.7) \\
    1017 & PGC040869 & NGVSJ12:27:31.55+09:35:44.3  186.8814384 &    9.5956422 &    14.90 &  0.022 &      32 &    9.9 (  1.4) \\
    1020 & PGC040872 & NGVSJ12:27:32.01+11:36:54.7  186.8833845 &   11.6151815 &    17.00 &  0.025 &    1379 &   -3.5 (  2.1) \\
    1025 & NGC4434   & NGVSJ12:27:36.68+08:09:15.6  186.9028317 &    8.1543420 &    13.10 &  0.023 &    1070 &   -4.7 (  0.7) \\
    1027 & PGC040890 & NGVSJ12:27:39.24+12:52:47.6  186.9134916 &   12.8798909 &    17.20 &  0.028 &      77 &   -5.0 (  1.2) \\
    1030 & NGC4435   & NGVSJ12:27:40.49+13:04:44.3  186.9187168 &   13.0789836 &    11.80 &  0.029 &     791 &   -2.1 (  0.5) \\
    1035 & PGC040906 & NGVSJ12:27:42.11+12:05:22.7  186.9254486 &   12.0896455 &    15.80 &  0.028 &     146 &   -4.3 (  1.6) \\
    1036 & NGC4436   & NGVSJ12:27:41.24+12:18:57.2  186.9218156 &   12.3158886 &    13.60 &  0.027 &    1113 &   -1.8 (  0.9) \\
    1040 & PGC040913 & NGVSJ12:27:44.52+12:59:01.3  186.9355189 &   12.9836833 &    15.50 &  0.028 &    -143 &   -5.0 (  1.2) \\
    1042 & PGC040915 & NGVSJ12:27:45.42+12:52:22.5  186.9392337 &   12.8729240 &    18.00 &  0.026 &     -62 &   -5.0 (  1.2) \\
    1043 & NGC4438   & NGVSJ12:27:45.65+13:00:31.9  186.9402024 &   13.0088742 &    10.50 &  0.028 &      71 &    0.6 (  1.5) \\
    1049 & UGC07580  & NGVSJ12:27:54.83+08:05:25.5  186.9784720 &    8.0904030 &    14.20 &  0.022 &     607 &   -4.2 (  2.0) \\
    1052 & PGC040932 & NGVSJ12:27:55.22+12:22:09.5  186.9800778 &   12.3692963 &    16.20 &  0.027 & \nodata &   -5.0 (  2.0) \\
    1059 & PGC040946 & NGVSJ12:28:00.44+11:56:59.6  187.0018514 &   11.9498934 &    17.80 &  0.026 &    2216 &   -5.0 (  1.2) \\
    1062 & NGC4442   & NGVSJ12:28:03.88+09:48:13.4  187.0161468 &    9.8037122 &    11.40 &  0.022 &     547 &   -1.9 (  0.4) \\
    1069 & PGC040958 & NGVSJ12:28:06.53+12:53:53.3  187.0272120 &   12.8981447 &    16.30 &  0.025 &    2326 &   -5.0 (  0.8) \\
    1073 & IC0794    & NGVSJ12:28:08.61+12:05:35.8  187.0358723 &   12.0932857 &    13.90 &  0.028 &    1921 &   -4.2 (  0.7) \\
    1075 & IC3383    & NGVSJ12:28:12.31+10:17:51.5  187.0513119 &   10.2976486 &    15.10 &  0.027 &    1808 &   -3.3 (  3.7) \\
    1076 & PGC040969 & NGVSJ12:28:12.84+10:31:33.7  187.0534826 &   10.5260342 &    16.80 &  0.029 &    1679 &   -5.0 (  1.4) \\
    1079 & PGC040972 & NGVSJ12:28:12.03+10:21:55.0  187.0501120 &   10.3652855 &    16.40 &  0.028 &    1354 &   -5.0 (  1.4) \\
    1087 & IC3381    & NGVSJ12:28:14.87+11:47:23.6  187.0619636 &   11.7898823 &    14.30 &  0.027 &     659 &   -4.1 (  0.8) \\
    1093 & PGC040995 & NGVSJ12:28:18.74+11:42:00.9  187.0780927 &   11.7002572 &    16.40 &  0.027 &    1476 &   -5.0 (  1.2) \\
    1100 & PGC041005 & NGVSJ12:28:23.37+11:34:46.9  187.0973594 &   11.5796867 &    17.90 &  0.028 & \nodata &   -5.0 (  3.0) \\
    1101 & PGC041007 & NGVSJ12:28:23.64+13:11:44.7  187.0985017 &   13.1957565 &    15.80 &  0.023 &    1670 &   -5.0 (  1.0) \\
    1104 & IC3388    & NGVSJ12:28:28.06+12:49:25.3  187.1169051 &   12.8236946 &    15.10 &  0.022 &    1707 &   -5.0 (  0.9) \\
    1110 & NGC4450   & NGVSJ12:28:29.59+17:05:06.1  187.1232946 &   17.0850198 &    10.90 &  0.028 &    1956 &    2.4 (  0.7) \\
    1115 & PGC041035 & NGVSJ12:28:32.40+11:44:40.7  187.1350073 &   11.7446286 &    17.00 &  0.030 &   30000 &   -5.0 (  2.0) \\
    1122 & IC3393    & NGVSJ12:28:41.71+12:54:57.2  187.1737961 &   12.9158877 &    14.50 &  0.020 &     465 &   -1.7 (  2.0) \\
    1123 & PGC041059 & NGVSJ12:28:42.66+12:32:59.4  187.1777602 &   12.5498411 &    16.40 &  0.022 &   30000 &   -5.0 (  1.2) \\
    1125 & NGC4452   & NGVSJ12:28:43.31+11:45:18.1  187.1804470 &   11.7550324 &    12.50 &  0.030 &     162 &   -1.9 (  0.8) \\
    1129 & PGC041068 & NGVSJ12:28:44.91+12:48:34.3  187.1871314 &   12.8095314 &    17.60 &  0.020 &      12 &   -5.0 (  1.2) \\
    1131 & PGC041071 & NGVSJ12:28:45.79+12:01:18.6  187.1907795 &   12.0218433 &    17.80 &  0.027 &    1172 &   -5.0 (  2.0) \\
    1136 & PGC041077 & NGVSJ12:28:49.11+12:07:54.5  187.2046093 &   12.1318006 &    18.00 &  0.027 &    1172 &   -5.0 (  3.0) \\
    1146 & NGC4458   & NGVSJ12:28:57.56+13:14:31.0  187.2398351 &   13.2419339 &    12.90 &  0.023 &     677 &   -4.9 (  0.4) \\
    1148 & PGC041098 & NGVSJ12:28:58.14+12:39:42.2  187.2422494 &   12.6617298 &    15.50 &  0.021 &    1417 &   -5.0 (  1.0) \\
    1149 & PGC041097 & NGVSJ12:28:58.84+12:54:28.8  187.2451828 &   12.9079984 &    17.40 &  0.020 &    1172 &   -5.0 (  1.4) \\
    1153 & PGC041102 & NGVSJ12:28:59.82+12:38:54.2  187.2492426 &   12.6483894 &    17.20 &  0.021 &   30000 &   10.0 (  2.0) \\
    1154 & NGC4459   & NGVSJ12:29:00.04+13:58:42.5  187.2501631 &   13.9784745 &    11.40 &  0.045 &    1192 &   -1.6 (  1.1) \\
    1158 & NGC4461   & NGVSJ12:29:03.01+13:11:01.7  187.2625503 &   13.1838010 &    11.50 &  0.023 &    1924 &   -0.7 (  1.3) \\
    1173 & PGC041136 & NGVSJ12:29:14.85+12:58:41.7  187.3118929 &   12.9782469 &    15.90 &  0.020 &    2416 &   -5.0 (  1.0) \\
    1177 & PGC041146 & NGVSJ12:29:19.28+12:22:37.2  187.3303288 &   12.3770123 &    18.20 &  0.023 &    1172 &   -5.0 (  3.0) \\
    1178 & NGC4464   & NGVSJ12:29:21.29+08:09:23.8  187.3387258 &    8.1566225 &    13.40 &  0.022 &    1243 &   -2.7 (  3.4) \\
    1185 & PGC041156 & NGVSJ12:29:23.52+12:27:02.9  187.3479850 &   12.4508043 &    15.70 &  0.023 &     448 &   -5.0 (  1.0) \\
    1190 & NGC4469   & NGVSJ12:29:28.03+08:44:59.3  187.3667933 &    8.7498027 &    12.20 &  0.020 &     588 &    0.3 (  0.7) \\
    1191 & PGC041167 & NGVSJ12:29:28.67+12:29:46.3  187.3694547 &   12.4962070 &    17.40 &  0.022 &       5 &   -5.0 (  1.2) \\
    1192 & NGC4467   & NGVSJ12:29:30.25+07:59:34.3  187.3760471 &    7.9928597 &    15.00 &  0.023 &    1390 &   -4.8 (  0.7) \\
    1199 & PGC041180 & NGVSJ12:29:34.99+08:03:28.8  187.3958061 &    8.0580083 &    15.50 &  0.022 &    1392 &   -5.0 (  1.2) \\
    1205 & NGC4470   & NGVSJ12:29:37.82+07:49:24.1  187.4075732 &    7.8233726 &    13.00 &  0.024 &    2340 &    1.9 (  2.1) \\
    1212 & PGC041197 & NGVSJ12:29:39.06+11:38:00.3  187.4127358 &   11.6334149 &    16.70 &  0.036 & \nodata &   -5.0 (  2.0) \\
    1213 & PGC041195 & NGVSJ12:29:39.24+12:32:53.7  187.4135137 &   12.5482441 &    16.10 &  0.022 &    1092 &   -5.0 (  1.2) \\
    1216 & PGC041203 & NGVSJ12:29:41.28+12:02:45.9  187.4220147 &   12.0460966 &    18.20 &  0.028 &    1172 &   -5.0 (  2.0) \\
    1219 & PGC041209 & NGVSJ12:29:44.09+12:48:19.6  187.4337238 &   12.8054536 &    18.00 &  0.020 &   30000 &   -5.0 (  1.2) \\
    1226 & NGC4472   & NGVSJ12:29:46.77+08:00:01.8  187.4448543 &    8.0004899 &     9.30 &  0.022 &     981 &   -4.8 (  0.5) \\
    1231 & NGC4473   & NGVSJ12:29:48.87+13:25:46.0  187.4536246 &   13.4294361 &    11.10 &  0.028 &    2244 &   -4.7 (  0.7) \\
    1239 & PGC041238 & NGVSJ12:29:53.00+11:57:44.3  187.4708241 &   11.9622933 &    16.80 &  0.029 &    -400 &   -5.0 (  1.4) \\
    1242 & NGC4474   & NGVSJ12:29:53.55+14:04:06.9  187.4731182 &   14.0685841 &    12.60 &  0.041 &    1611 &   -1.9 (  0.9) \\
    1244 & PGC041245 & NGVSJ12:29:56.34+13:13:12.3  187.4847568 &   13.2200747 &    18.00 &  0.024 &    1172 &   -5.0 (  3.0) \\
    1250 & NGC4476   & NGVSJ12:29:59.08+12:20:55.4  187.4961534 &   12.3487189 &    12.90 &  0.027 &    1959 &   -2.9 (  1.0) \\
    1253 & NGC4477   & NGVSJ12:30:02.20+13:38:11.5  187.5091719 &   13.6365327 &    11.30 &  0.032 &    1338 &   -1.7 (  0.7) \\
    1259 & PGC041268 & NGVSJ12:30:06.08+12:22:37.9  187.5253517 &   12.3772044 &    17.80 &  0.028 &    1172 &   -5.0 (  2.0) \\
    1261 & NGC4482   & NGVSJ12:30:10.33+10:46:46.2  187.5430470 &   10.7794918 &    13.60 &  0.029 &    1825 &   -4.8 (  0.6) \\
    1264 & PGC041273 & NGVSJ12:30:10.88+12:11:43.6  187.5453319 &   12.1954334 &    16.40 &  0.025 &   30000 &   -5.0 (  1.2) \\
    1271 & PGC041287 & NGVSJ12:30:15.27+12:30:57.3  187.5636331 &   12.5159145 &    19.00 &  0.022 &    1172 &   -5.0 (  2.0) \\
    1279 & NGC4478   & NGVSJ12:30:17.42+12:19:42.8  187.5725711 &   12.3285593 &    12.20 &  0.023 &    1349 &   -4.9 (  0.4) \\
    1283 & NGC4479   & NGVSJ12:30:18.38+13:34:39.5  187.5765820 &   13.5776497 &    13.40 &  0.029 &     848 &   -1.9 (  0.5) \\
    1289 & PGC041313 & NGVSJ12:30:24.48+13:19:55.8  187.6019909 &   13.3321702 &    18.00 &  0.026 & \nodata &   -5.0 (  2.0) \\
    1297 & NGC4486B  & NGVSJ12:30:31.97+12:29:24.6  187.6332079 &   12.4901631 &    14.30 &  0.021 &    1555 &   -5.0 (  0.8) \\
    1298 & PGC041329 & NGVSJ12:30:33.32+12:54:02.3  187.6388495 &   12.9006515 &    17.80 &  0.020 &    1172 &   -5.0 (  2.0) \\
    1300 & PGC041331 & NGVSJ12:30:34.65+12:27:29.2  187.6443597 &   12.4581190 &    17.40 &  0.021 &    1172 &   -5.0 (  3.0) \\
    1303 & NGC4483   & NGVSJ12:30:40.64+09:00:56.4  187.6693449 &    9.0156724 &    13.10 &  0.020 &     884 &   -1.4 (  0.7) \\
    1308 & IC3437    & NGVSJ12:30:45.91+11:20:35.5  187.6912832 &   11.3431951 &    15.20 &  0.035 &    1739 &   -5.0 (  1.0) \\
    1313 & PGC041360 & NGVSJ12:30:48.58+12:02:42.7  187.7024092 &   12.0451886 &    16.70 &  0.027 &    1254 &   10.0 (  1.4) \\
    1314 & PGC041358 & NGVSJ12:30:49.03+13:13:25.8  187.7043010 &   13.2238351 &    16.70 &  0.025 &      35 &    0.2 (  6.9) \\
    1316 & NGC4486   & NGVSJ12:30:49.42+12:23:28.0  187.7059365 &   12.3911224 &     9.60 &  0.023 &    1284 &   -4.3 (  0.6) \\
    1317 & PGC041362 & NGVSJ12:30:50.59+12:44:11.7  187.7107846 &   12.7365860 &    17.80 &  0.023 &    1172 &   -5.0 (  2.0) \\
    1318 & NGC4488   & NGVSJ12:30:51.37+08:21:36.0  187.7140590 &    8.3600070 &    12.90 &  0.021 &     980 &   -0.1 (  0.6) \\
    1321 & NGC4489   & NGVSJ12:30:52.25+16:45:31.8  187.7177136 &   16.7588428 &    12.80 &  0.027 &     940 &   -4.7 (  0.9) \\
    1324 & PGC041375 & NGVSJ12:30:55.66+13:20:53.8  187.7319358 &   13.3482714 &    17.90 &  0.025 &   30000 &   -5.0 (  2.0) \\
    1327 & NGC4486A  & NGVSJ12:30:57.77+12:16:15.5  187.7407131 &   12.2709806 &    13.30 &  0.023 &     758 &   -5.0 (  0.4) \\
    1331 & PGC041384 & NGVSJ12:30:58.81+11:42:30.8  187.7450512 &   11.7085529 &    17.40 &  0.031 & \nodata &   -5.0 (  2.0) \\
    1336 & PGC041398 & NGVSJ12:31:03.98+11:50:10.2  187.7665675 &   11.8361640 &    17.40 &  0.028 & \nodata &   -5.0 (  3.0) \\
    1340 & PGC041411 & NGVSJ12:31:10.42+13:05:50.5  187.7934070 &   13.0973532 &    17.90 &  0.023 &    1540 &   -5.0 (  1.4) \\
    1341 & PGC041414 & NGVSJ12:31:11.64+13:06:51.7  187.7984812 &   13.1143508 &    18.00 &  0.024 & \nodata &   -5.0 (  2.0) \\
    1343 & PGC041416 & NGVSJ12:31:12.69+13:07:27.4  187.8028829 &   13.1242729 &    18.00 &  0.024 &    1900 &   -5.0 (  1.4) \\
    1348 & IC3443    & NGVSJ12:31:15.73+12:19:54.4  187.8155531 &   12.3317700 &    15.20 &  0.022 &    1019 &   -5.0 (  1.2) \\
    1352 & PGC041433 & NGVSJ12:31:19.57+12:36:41.5  187.8315239 &   12.6115153 &    17.00 &  0.022 &    1766 &   -4.0 (  1.8) \\
    1353 & PGC041432 & NGVSJ12:31:19.43+12:44:16.9  187.8309531 &   12.7380408 &    16.10 &  0.024 &    -380 &   -4.4 (  1.5) \\
    1354 & PGC041431 & NGVSJ12:31:18.87+13:19:54.7  187.8286445 &   13.3318665 &    18.40 &  0.025 & \nodata &   -5.0 (  2.0) \\
    1355 & IC3442    & NGVSJ12:31:20.20+14:06:54.6  187.8341502 &   14.1151537 &    14.30 &  0.035 &    1245 &   -5.0 (  0.4) \\
    1356 & IC3446    & NGVSJ12:31:22.98+11:29:33.2  187.8457595 &   11.4925479 &    15.20 &  0.045 &    1252 &    9.6 (  1.3) \\
    1366 & PGC041454 & NGVSJ12:31:31.68+11:36:11.1  187.8820201 &   11.6030707 &    17.10 &  0.047 &   30000 &   -5.0 (  1.4) \\
    1368 & NGC4497   & NGVSJ12:31:32.54+11:37:29.1  187.8855752 &   11.6247460 &    12.70 &  0.042 &    1042 &   -1.1 (  1.1) \\
    1369 & PGC041458 & NGVSJ12:31:33.35+12:03:49.7  187.8889577 &   12.0638064 &    16.50 &  0.029 &     797 &   -4.3 (  1.6) \\
    1379 & NGC4498   & NGVSJ12:31:39.43+16:51:10.5  187.9142868 &   16.8529154 &    12.60 &  0.029 &    1507 &    6.4 (  0.9) \\
    1386 & IC3457    & NGVSJ12:31:51.33+12:39:25.2  187.9638828 &   12.6569935 &    14.40 &  0.026 &    1297 &   -4.7 (  1.7) \\
    1389 & PGC041495 & NGVSJ12:31:52.01+12:28:54.5  187.9667127 &   12.4818113 &    15.80 &  0.025 &     877 &   -5.0 (  1.2) \\
    1392 & IC3459    & NGVSJ12:31:55.93+12:10:27.0  187.9830351 &   12.1741628 &    14.60 &  0.027 &     385 &    9.8 (  0.5) \\
    1396 & PGC041508 & NGVSJ12:31:56.40+11:58:21.7  187.9849804 &   11.9726948 &    17.00 &  0.029 &    1094 &   -5.0 (  2.0) \\
    1399 & PGC041516 & NGVSJ12:32:00.75+12:37:13.2  188.0031452 &   12.6203250 &    16.50 &  0.026 &     493 &   -5.0 (  1.2) \\
    1407 & IC3461    & NGVSJ12:32:02.74+11:53:24.3  188.0114114 &   11.8900782 &    15.50 &  0.033 &    1007 &   -5.0 (  0.9) \\
    1411 & IC3466    & NGVSJ12:32:05.63+11:49:03.6  188.0234745 &   11.8176581 &    15.40 &  0.033 &     909 &   10.0 (  1.4) \\
    1412 & NGC4503   & NGVSJ12:32:06.23+11:10:35.0  188.0259744 &   11.1763897 &    12.10 &  0.051 &    1334 &   -1.7 (  1.8) \\
    1414 & PGC041541 & NGVSJ12:32:09.31+12:50:20.2  188.0388115 &   12.8389402 &    16.80 &  0.024 &     192 &   -5.0 (  1.0) \\
    1417 & PGC041544 & NGVSJ12:32:09.58+15:18:03.3  188.0399339 &   15.3009169 &    15.80 &  0.031 &    1577 &   -5.0 (  1.4) \\
    1418 & PGC041545 & NGVSJ12:32:11.36+12:30:24.9  188.0473303 &   12.5069279 &    17.10 &  0.028 &   30000 &   -5.0 (  3.0) \\
    1419 & NGC4506   & NGVSJ12:32:10.50+13:25:09.7  188.0437355 &   13.4193556 &    13.20 &  0.028 &     561 &    1.1 (  0.9) \\
    1420 & IC3465    & NGVSJ12:32:12.24+12:03:41.5  188.0510100 &   12.0615256 &    16.10 &  0.029 &     985 &   -4.3 (  1.6) \\
    1422 & IC3468    & NGVSJ12:32:14.22+10:15:05.3  188.0592337 &   10.2514606 &    13.60 &  0.032 &    1300 &   -4.8 (  0.6) \\
    1426 & PGC041570 & NGVSJ12:32:23.58+11:53:36.1  188.0982667 &   11.8933691 &    15.40 &  0.033 &     833 &   10.0 (  2.0) \\
    1431 & IC3470    & NGVSJ12:32:23.38+11:15:46.7  188.0974316 &   11.2629600 &    14.50 &  0.051 &    1489 &   -4.8 (  0.9) \\
    1438 & PGC041588 & NGVSJ12:32:34.71+12:38:21.1  188.1446063 &   12.6391986 &    17.40 &  0.026 &    1172 &   -5.0 (  3.0) \\
    1440 & IC0798    & NGVSJ12:32:33.41+15:24:55.4  188.1391948 &   15.4153952 &    15.20 &  0.028 &     429 &   -5.0 (  1.2) \\
    1448 & IC3475    & NGVSJ12:32:40.80+12:46:15.9  188.1700092 &   12.7710848 &    13.70 &  0.026 &    2583 &   -4.6 (  1.9) \\
    1449 & PGC041604 & NGVSJ12:32:39.13+13:19:47.5  188.1630433 &   13.3298656 &    17.60 &  0.026 & \nodata &   -5.0 (  2.0) \\
    1463 & PGC041637 & NGVSJ12:32:54.11+12:48:27.2  188.2254464 &   12.8075653 &    18.20 &  0.028 & \nodata &   -5.0 (  2.0) \\
    1475 & NGC4515   & NGVSJ12:33:04.97+16:15:55.9  188.2707092 &   16.2655230 &    13.40 &  0.031 &     955 &   -3.2 (  0.7) \\
    1477 & PGC041659 & NGVSJ12:33:06.41+13:18:11.1  188.2766994 &   13.3030724 &    18.40 &  0.026 & \nodata &   -5.0 (  2.0) \\
    1488 & IC3487    & NGVSJ12:33:13.43+09:23:50.4  188.3059683 &    9.3973326 &    14.80 &  0.021 &    1074 &   -3.5 (  2.1) \\
    1489 & IC3490    & NGVSJ12:33:13.91+10:55:42.9  188.3079662 &   10.9285760 &    15.90 &  0.032 &     268 &   -5.0 (  1.2) \\
    1491 & IC3486    & NGVSJ12:33:14.01+12:51:28.2  188.3083811 &   12.8578220 &    14.70 &  0.031 &    1986 &   -3.6 (  2.0) \\
    1499 & IC3492    & NGVSJ12:33:19.79+12:51:12.5  188.3324580 &   12.8534644 &    14.80 &  0.030 &    -541 &   -3.8 (  1.6) \\
    1502 & PGC041705 & NGVSJ12:33:25.21+13:24:58.5  188.3550571 &   13.4162553 &    18.20 &  0.029 & \nodata &   -5.0 (  2.0) \\
    1508 & NGC4519   & NGVSJ12:33:30.26+08:39:17.2  188.3760725 &    8.6547664 &    12.30 &  0.020 &    1218 &    6.9 (  0.4) \\
    1509 & PGC041720 & NGVSJ12:33:31.65+09:27:33.2  188.3818570 &    9.4592142 &    16.30 &  0.023 &     808 &   -5.0 (  1.4) \\
    1512 & PGC041723 & NGVSJ12:33:34.65+11:15:43.0  188.3943603 &   11.2619480 &    15.70 &  0.051 &     839 &   -3.0 (  1.8) \\
    1514 & PGC041726 & NGVSJ12:33:37.70+07:52:15.8  188.4070872 &    7.8710636 &    15.00 &  0.020 &     538 &   -4.3 (  1.6) \\
    1516 & NGC4522   & NGVSJ12:33:39.71+09:10:30.1  188.4154727 &    9.1750335 &    12.70 &  0.021 &    2329 &    5.9 (  0.6) \\
    1517 & PGC041730 & NGVSJ12:33:40.81+12:34:16.4  188.4200532 &   12.5712341 &    17.60 &  0.029 &   10188 &   -5.0 (  2.0) \\
    1518 & PGC041731 & NGVSJ12:33:40.91+12:22:56.7  188.4204721 &   12.3824222 &    18.40 &  0.030 & \nodata &   -5.0 (  2.0) \\
    1522 & PGC041740 & NGVSJ12:33:47.06+11:46:53.8  188.4460735 &   11.7816189 &    17.90 &  0.041 & \nodata &   -5.0 (  2.0) \\
    1523 & PGC041744 & NGVSJ12:33:48.67+12:46:48.1  188.4528030 &   12.7800364 &    17.30 &  0.030 &    1108 &   -5.0 (  1.4) \\
    1528 & IC3501    & NGVSJ12:33:51.62+13:19:20.9  188.4650793 &   13.3224639 &    14.50 &  0.028 &    1615 &   -4.4 (  1.5) \\
    1535 & NGC4526   & NGVSJ12:34:02.98+07:41:57.5  188.5124331 &    7.6993100 &    10.00 &  0.022 &     617 &   -1.9 (  0.4) \\
    1536 & PGC041775 & NGVSJ12:34:06.56+11:50:12.1  188.5273235 &   11.8367030 &    17.90 &  0.038 & \nodata &   -5.0 (  2.0) \\
    1537 & NGC4528   & NGVSJ12:34:06.08+11:19:16.5  188.5253210 &   11.3212533 &    12.70 &  0.046 &    1378 &   -2.0 (  0.5) \\
    1539 & PGC041782 & NGVSJ12:34:06.74+12:44:29.7  188.5280977 &   12.7415714 &    15.70 &  0.032 &    1508 &   -5.0 (  1.0) \\
    1541 & PGC041787 & NGVSJ12:34:08.98+12:44:24.8  188.5374062 &   12.7402195 &    18.10 &  0.032 & \nodata & \nodata (\nodata) \\
    1545 & IC3509    & NGVSJ12:34:11.53+12:02:56.3  188.5480615 &   12.0489659 &    15.00 &  0.041 &    2065 &   -5.0 (  1.0) \\
    1552 & NGC4531   & NGVSJ12:34:15.88+13:04:31.1  188.5661639 &   13.0753139 &    12.60 &  0.043 &      90 &   -0.1 (  2.4) \\
    1554 & NGC4532   & NGVSJ12:34:19.53+06:27:58.9  188.5813616 &    6.4663628 &    12.30 &  0.021 &    2011 &    9.7 (  0.8) \\
    1561 & PGC041818 & NGVSJ12:34:25.05+12:54:12.8  188.6043594 &   12.9035629 &    15.50 &  0.032 &    -582 &   -5.0 (  3.0) \\
    1563 & PGC041822 & NGVSJ12:34:26.05+11:55:01.4  188.6085262 &   11.9170464 &    16.10 &  0.039 &    2249 &   -5.0 (  1.4) \\
    1588 & NGC4540   & NGVSJ12:34:50.85+15:33:05.9  188.7118891 &   15.5516418 &    12.50 &  0.035 &    1291 &    6.2 (  0.9) \\
    1615 & NGC4548   & NGVSJ12:35:26.46+14:29:46.9  188.8602505 &   14.4963502 &    11.00 &  0.038 &     486 &    3.1 (  0.5) \\
    1619 & NGC4550   & NGVSJ12:35:30.58+12:13:14.7  188.8774282 &   12.2207530 &    12.50 &  0.040 &     459 &   -2.0 (  0.7) \\
    1627 & PGC041959 & NGVSJ12:35:37.25+12:22:55.4  188.9052169 &   12.3820489 &    15.20 &  0.038 &     282 &   -5.0 (  0.9) \\
    1630 & NGC4551   & NGVSJ12:35:37.95+12:15:50.4  188.9081312 &   12.2639882 &    12.90 &  0.039 &    1176 &   -4.9 (  0.4) \\
    1632 & NGC4552   & NGVSJ12:35:39.81+12:33:22.9  188.9158835 &   12.5563645 &    10.80 &  0.041 &     340 &   -4.6 (  0.9) \\
    1661 & PGC042046 & NGVSJ12:36:24.78+10:23:04.8  189.1032517 &   10.3846789 &    16.00 &  0.020 &    1419 &   -5.0 (  1.2) \\
    1664 & NGC4564   & NGVSJ12:36:26.98+11:26:21.2  189.1124336 &   11.4392282 &    12.00 &  0.034 &    1142 &   -4.6 (  0.7) \\
    1690 & NGC4569   & NGVSJ12:36:49.86+13:09:46.7  189.2077334 &   13.1629785 &    10.20 &  0.046 &    -235 &    2.4 (  0.7) \\
    1692 & NGC4570   & NGVSJ12:36:53.38+07:14:47.7  189.2224185 &    7.2465803 &    11.80 &  0.022 &    1787 &   -1.9 (  1.0) \\
    1695 & IC3586    & NGVSJ12:36:54.86+12:31:12.5  189.2285916 &   12.5201265 &    14.50 &  0.045 &    1717 &   -3.0 (  1.8) \\
    1696 & NGC4571   & NGVSJ12:36:56.39+14:13:02.4  189.2349379 &   14.2173437 &    11.80 &  0.046 &     332 &    6.4 (  0.8) \\
    1720 & NGC4578   & NGVSJ12:37:30.56+09:33:18.4  189.3773344 &    9.5550995 &    12.30 &  0.020 &    2292 &   -2.1 (  0.6) \\
    1727 & NGC4579   & NGVSJ12:37:43.53+11:49:05.5  189.4313892 &   11.8182052 &    10.60 &  0.041 &    1517 &    2.8 (  0.6) \\
    1730 & NGC4580   & NGVSJ12:37:48.39+05:22:06.7  189.4516186 &    5.3685208 &    12.60 &  0.024 &    1035 &    1.6 (  0.7) \\
    1743 & IC3602    & NGVSJ12:38:06.79+10:04:56.6  189.5282773 &   10.0823858 &    15.50 &  0.019 &    1279 &   -3.0 (  1.8) \\
    1779 & IC3612    & NGVSJ12:39:04.69+14:43:51.9  189.7695433 &   14.7310745 &    14.80 &  0.027 &    1251 &   -1.7 (  1.2) \\
    1809 & IC3631    & NGVSJ12:39:48.01+12:58:26.2  189.9500562 &   12.9739543 &    13.80 &  0.037 &    2828 &   -1.2 (  1.7) \\
    1811 & NGC4595   & NGVSJ12:39:51.91+15:17:52.0  189.9663104 &   15.2977805 &    12.90 &  0.037 &     631 &    4.0 (  1.9) \\
    1813 & NGC4596   & NGVSJ12:39:55.96+10:10:34.1  189.9831538 &   10.1761470 &    11.50 &  0.021 &    1892 &   -0.8 (  0.8) \\
    1826 & IC3633    & NGVSJ12:40:11.25+09:53:46.0  190.0468834 &    9.8961198 &    15.70 &  0.017 &    1973 &   -5.0 (  1.2) \\
    1828 & IC3635    & NGVSJ12:40:13.39+12:52:29.2  190.0557887 &   12.8747695 &    15.30 &  0.037 &    1560 &    4.3 (  4.0) \\
    1833 & PGC042442 & NGVSJ12:40:19.68+15:56:07.0  190.0820095 &   15.9352811 &    14.50 &  0.036 &    1705 &   -2.7 (  1.8) \\
    1851 & PGC042487 & NGVSJ12:40:43.60+10:24:28.1  190.1816754 &   10.4078114 &    18.00 &  0.023 & \nodata &   -5.0 (  3.0) \\
    1857 & IC3647    & NGVSJ12:40:53.12+10:28:32.2  190.2213279 &   10.4756088 &    14.10 &  0.025 &     634 &    9.8 (  0.5) \\
    1859 & NGC4606   & NGVSJ12:40:57.55+11:54:43.8  190.2398109 &   11.9121733 &    12.70 &  0.032 &    1649 &    0.6 (  1.4) \\
    1861 & IC3652    & NGVSJ12:40:58.56+11:11:04.2  190.2439935 &   11.1844975 &    14.40 &  0.030 &     630 &   -4.8 (  0.6) \\
    1869 & NGC4608   & NGVSJ12:41:13.29+10:09:20.3  190.3053852 &   10.1556511 &    12.10 &  0.017 &    1850 &   -1.7 (  0.8) \\
    1870 & PGC042547 & NGVSJ12:41:15.35+11:17:54.5  190.3139453 &   11.2984787 &    15.80 &  0.028 &    1652 &   -5.0 (  1.4) \\
    1871 & IC3653    & NGVSJ12:41:15.73+11:23:14.1  190.3155405 &   11.3872469 &    13.90 &  0.031 &     557 &   -5.0 (  1.0) \\
    1879 & PGC042566 & NGVSJ12:41:27.39+11:08:45.0  190.3641447 &   11.1458370 &    16.80 &  0.029 &    1070 &   -5.0 (  3.0) \\
    1883 & NGC4612   & NGVSJ12:41:32.75+07:18:53.6  190.3864549 &    7.3148793 &    12.60 &  0.025 &    1775 &   -2.0 (  0.4) \\
    1886 & PGC042586 & NGVSJ12:41:39.41+12:14:50.9  190.4142274 &   12.2474618 &    15.50 &  0.033 &     927 &   -5.0 (  1.4) \\
    1895 & UGC07854  & NGVSJ12:41:51.97+09:24:10.6  190.4665489 &    9.4029504 &    14.90 &  0.017 &     970 &   -3.0 (  1.8) \\
    1903 & NGC4621   & NGVSJ12:42:02.26+11:38:49.0  190.5094276 &   11.6469455 &    10.80 &  0.033 &     467 &   -4.8 (  0.4) \\
    1910 & IC0809    & NGVSJ12:42:08.67+11:45:15.4  190.5361351 &   11.7542664 &    14.20 &  0.032 &     196 &   -4.9 (  0.4) \\
    1938 & NGC4638   & NGVSJ12:42:47.43+11:26:33.0  190.6976235 &   11.4425074 &    12.10 &  0.025 &    1152 &   -2.6 (  0.7) \\
    1943 & NGC4639   & NGVSJ12:42:52.37+13:15:26.5  190.7182196 &   13.2573609 &    12.20 &  0.026 &    1018 &    3.6 (  0.7) \\
    1948 & PGC042754 & NGVSJ12:42:58.06+10:40:55.1  190.7418971 &   10.6819602 &    15.10 &  0.025 &    1610 &   -5.0 (  1.2) \\
    1978 & NGC4649   & NGVSJ12:43:39.97+11:33:09.7  190.9165323 &   11.5527000 &     9.80 &  0.026 &    1110 &   -4.6 (  0.9) \\
    1987 & NGC4654   & NGVSJ12:43:56.58+13:07:36.2  190.9857679 &   13.1267090 &    11.10 &  0.026 &    1036 &    5.9 (  0.5) \\
    1993 & PGC042884 & NGVSJ12:44:12.02+12:56:30.6  191.0501035 &   12.9418399 &    15.30 &  0.025 &     847 &   -4.0 (  1.8) \\
    1999 & NGC4659   & NGVSJ12:44:29.40+13:29:54.8  191.1224887 &   13.4985566 &    13.10 &  0.026 &     469 &   -0.1 (  0.6) \\
    2000 & NGC4660   & NGVSJ12:44:31.98+11:11:25.8  191.1332587 &   11.1905008 &    11.90 &  0.034 &    1083 &   -4.6 (  0.7) \\
    2019 & IC3735    & NGVSJ12:45:20.42+13:41:33.6  191.3350829 &   13.6926720 &    14.60 &  0.022 &    1819 &   -3.9 (  1.7) \\
    2048 & IC3773    & NGVSJ12:47:15.30+10:12:13.1  191.8137560 &   10.2036290 &    13.60 &  0.032 &    1086 &   -4.5 (  1.1) \\
    2050 & IC3779    & NGVSJ12:47:20.64+12:09:59.2  191.8359814 &   12.1664348 &    15.20 &  0.023 &    1165 &   -4.0 (  1.8) \\
    2058 & NGC4689   & NGVSJ12:47:45.56+13:45:46.1  191.9398462 &   13.7628078 &    11.60 &  0.023 &    1604 &    4.7 (  0.9) \\
    2066 & NGC4694   & NGVSJ12:48:15.12+10:58:59.8  192.0630072 &   10.9832842 &    12.20 &  0.039 &    1160 &   -1.8 (  0.7) \\
    2087 & NGC4733   & NGVSJ12:51:06.78+10:54:43.5  192.7782371 &   10.9120966 &    12.20 &  0.019 &     925 &   -3.6 (  1.3) \\
    2092 & NGC4754   & NGVSJ12:52:17.50+11:18:49.9  193.0729000 &   11.3138628 &    11.50 &  0.030 &    1351 &   -2.4 (  1.1) \\
    2095 & NGC4762   & NGVSJ12:52:55.97+11:13:51.5  193.2332268 &   11.2309755 &    10.80 &  0.023 &     986 &   -1.8 (  0.9) \\
 \nodata    &\nodata      & NGVSJ12:31:52.90+12:15:59.1  187.9703966 &   12.2664053 &    17.80 &  0.025 & \nodata & \nodata (\nodata) \\
 \nodata    &\nodata      & NGVSJ12:29:33.61+13:11:44.6  187.3900510 &   13.1957155 &    18.10 &  0.024 & \nodata & \nodata (\nodata) \\
 \nodata    &\nodata      & NGVSJ12:33:40.31+12:44:13.6  188.4179553 &   12.7371155 &    18.30 &  0.029 & \nodata & \nodata (\nodata) \\
\\
\enddata
\end{deluxetable}
\label{tab_all}
\tablecomments{This table is available in its entirety in a machine-readable form in the online journal. A portion is shown here for guidance regarding its form and content. All magnitudes are in $AB$ mag.}




==> table_data_ref_full_clean.tex <==
\startlongtable
\begin{deluxetable}{lllcccccc}
%\tabletypesize{\footnotesize}
\tabletypesize{\scriptsize}
\tablecaption{List of targets with SBF measurements}
\tablehead{
  \colhead{VCC} &
  \colhead{Alt. Name} &
  \colhead{IAU Name} &
  \colhead{RA (J2000)} &
  \colhead{Dec (J2000)} &
  \colhead{$B_T$} &
  \colhead{\tiny{$E(B{-}V)$}} &
  \colhead{$v_{Helio}$} &
  \colhead{$T_{Type}$} &
  \\
  \colhead{   } &
  \colhead{         } &
  \colhead{   (deg)  } &
  \colhead{  (deg)    } &
  \colhead{(mag)} &
  \colhead{ (mag)           } &
  \colhead{\kms       } &
  \colhead{          } &
  } \startdata 
      (1)&   (2)      &     (3)      &        (4)   &    (5)   &  (6)   &    (7)  &      (8)     \\   
\hline
      32 & IC0767    & NGVSJ12:11:02.73+12:06:14.4  182.7613724 &   12.1039918 &    14.00 &  0.027 &    1877 &   -5.0 (  1.0) \\
      33 & IC3032    & NGVSJ12:11:07.76+14:16:29.3  182.7823394 &   14.2748006 &    14.70 &  0.038 &    1179 &   -4.0 (  1.8) \\
      49 & NGC4168   & NGVSJ12:12:17.26+13:12:18.7  183.0719332 &   13.2051960 &    12.20 &  0.037 &    2273 &   -4.9 (  0.4) \\
      66 & NGC4178   & NGVSJ12:12:46.57+10:51:59.8  183.1940241 &   10.8666242 &    11.90 &  0.028 &     374 &    6.9 (  1.2) \\
      89 & NGC4189   & NGVSJ12:13:47.24+13:25:29.5  183.4468247 &   13.4248521 &    12.50 &  0.033 &    2098 &    5.9 (  0.9) \\
      92 & NGC4192   & NGVSJ12:13:48.29+14:54:01.8  183.4512262 &   14.9005060 &    10.90 &  0.035 &    -142 &    2.6 (  0.8) \\
     107 & PGC039071 & NGVSJ12:14:09.75+13:14:00.5  183.5406147 &   13.2334632 &    19.40 &  0.030 & \nodata &   -5.0 (  2.0) \\
     140 & IC3065    & NGVSJ12:15:12.56+14:25:58.4  183.8023507 &   14.4328799 &    14.30 &  0.036 &     995 &   -2.2 (  1.2) \\
     145 & NGC4206   & NGVSJ12:15:16.82+13:01:26.4  183.8200770 &   13.0239966 &    12.80 &  0.032 &     703 &    4.0 (  0.3) \\
     157 & NGC4212   & NGVSJ12:15:39.34+13:54:05.4  183.9138976 &   13.9015055 &    11.90 &  0.033 &     -88 &    4.9 (  0.8) \\
     167 & NGC4216   & NGVSJ12:15:54.39+13:08:58.0  183.9766077 &   13.1494566 &    11.00 &  0.032 &     131 &    3.0 (  0.5) \\
     199 & NGC4224   & NGVSJ12:16:33.79+07:27:43.4  184.1407813 &    7.4620674 &    12.90 &  0.024 &    2584 &    1.0 (  0.3) \\
     200 & PGC039331 & NGVSJ12:16:33.71+13:01:53.7  184.1404477 &   13.0315970 &    14.70 &  0.030 &       8 &   -4.3 (  1.6) \\
     220 & NGC4233   & NGVSJ12:17:07.68+07:37:27.4  184.2820056 &    7.6242759 &    13.00 &  0.024 &    2275 &   -2.0 (  0.5) \\
     222 & NGC4235   & NGVSJ12:17:09.88+07:11:29.7  184.2911844 &    7.1915747 &    12.70 &  0.019 &    2263 &    1.0 (  0.4) \\
     226 & NGC4237   & NGVSJ12:17:11.43+15:19:26.5  184.2976068 &   15.3240384 &    12.50 &  0.030 &     864 &    4.0 (  0.5) \\
     230 & IC3101    & NGVSJ12:17:19.65+11:56:36.5  184.3318761 &   11.9434644 &    15.20 &  0.028 &    1430 &   -5.0 (  1.4) \\
     263 & PGC039475 & NGVSJ12:17:56.83+11:59:45.7  184.4868025 &   11.9960324 &    18.20 &  0.030 & \nodata &   -5.0 (  3.0) \\
     308 & IC3131    & NGVSJ12:18:50.89+07:51:43.1  184.7120270 &    7.8619797 &    13.70 &  0.021 &    1530 &   -3.5 (  1.8) \\
     315 & PGC039606 & NGVSJ12:19:00.55+06:05:40.6  184.7523115 &    6.0946187 &    14.80 &  0.023 &    1589 &    0.5 (  1.0) \\
     341 & NGC4260   & NGVSJ12:19:22.25+06:05:55.2  184.8427241 &    6.0986724 &    12.70 &  0.023 &    1776 &    1.0 (  0.5) \\
     345 & NGC4261   & NGVSJ12:19:23.22+05:49:29.6  184.8467458 &    5.8248971 &    11.30 &  0.018 &    2177 &   -4.8 (  0.4) \\
     355 & NGC4262   & NGVSJ12:19:30.57+14:52:39.6  184.8773845 &   14.8776534 &    12.40 &  0.036 &    1359 &   -2.6 (  0.7) \\
     369 & NGC4267   & NGVSJ12:19:45.28+12:47:53.7  184.9386693 &   12.7982620 &    11.80 &  0.047 &    1021 &   -2.7 (  0.7) \\
     397 & PGC039772 & NGVSJ12:20:12.18+06:37:23.5  185.0507418 &    6.6231923 &    14.90 &  0.019 &    2442 &   -5.0 (  1.2) \\
     465 & NGC4294   & NGVSJ12:21:17.84+11:30:38.4  185.3243502 &   11.5106643 &    12.60 &  0.034 &     355 &    5.9 (  0.5) \\
     483 & NGC4298   & NGVSJ12:21:32.77+14:36:22.1  185.3865368 &   14.6061371 &    12.10 &  0.035 &    1124 &    5.1 (  0.6) \\
     490 & IC0783    & NGVSJ12:21:38.77+15:44:42.4  185.4115379 &   15.7451112 &    13.40 &  0.022 &    1267 &   -0.2 (  0.8) \\
     491 & NGC4299   & NGVSJ12:21:40.32+11:30:11.4  185.4180145 &   11.5031588 &    12.90 &  0.033 &     237 &    8.4 (  1.3) \\
     497 & NGC4302   & NGVSJ12:21:42.40+14:35:41.8  185.4266475 &   14.5949500 &    12.60 &  0.035 &    1098 &    5.3 (  0.8) \\
     523 & NGC4306   & NGVSJ12:22:04.12+12:47:15.0  185.5171828 &   12.7874979 &    13.10 &  0.042 &    1524 &   -2.0 (  0.8) \\
     524 & NGC4307   & NGVSJ12:22:05.66+09:02:37.2  185.5235656 &    9.0436564 &    12.80 &  0.023 &    1055 &    3.2 (  0.7) \\
     538 & PGC040059 & NGVSJ12:22:14.74+07:10:01.7  185.5614014 &    7.1671499 &    15.40 &  0.020 &     755 &   -5.0 (  1.2) \\
     543 & UGC07436  & NGVSJ12:22:19.53+14:45:38.8  185.5813776 &   14.7607696 &    14.40 &  0.031 &     977 &   -2.7 (  2.3) \\
     559 & NGC4312   & NGVSJ12:22:31.34+15:32:16.5  185.6305649 &   15.5379150 &    12.60 &  0.027 &     158 &    2.1 (  0.9) \\
     570 & NGC4313   & NGVSJ12:22:38.54+11:48:03.2  185.6606025 &   11.8008999 &    12.70 &  0.036 &    1431 &    2.1 (  0.4) \\
     571 & PGC040115 & NGVSJ12:22:41.10+07:57:01.4  185.6712666 &    7.9503803 &    14.70 &  0.022 &    1101 &   -1.8 (  1.3) \\
     575 & NGC4318   & NGVSJ12:22:43.29+08:11:53.8  185.6803578 &    8.1982639 &    14.10 &  0.025 &    1203 &   -4.7 (  0.9) \\
     596 & NGC4321   & NGVSJ12:22:54.91+15:49:20.2  185.7287922 &   15.8222817 &    10.10 &  0.026 &    1571 &    4.0 (  0.3) \\
     613 & NGC4324   & NGVSJ12:23:06.17+05:15:01.2  185.7757201 &    5.2503454 &    12.60 &  0.024 &    1667 &   -0.8 (  1.2) \\
     648 & NGC4339   & NGVSJ12:23:34.95+06:04:54.4  185.8956063 &    6.0817747 &    12.30 &  0.026 &    1266 &   -4.6 (  1.0) \\
     654 & NGC4340   & NGVSJ12:23:35.28+16:43:20.4  185.8970174 &   16.7223449 &    11.60 &  0.026 &     933 &   -1.2 (  0.6) \\
     657 & NGC4342   & NGVSJ12:23:39.00+07:03:14.4  185.9125041 &    7.0539981 &    12.60 &  0.020 &     761 &   -3.2 (  1.0) \\
     685 & NGC4350   & NGVSJ12:23:57.84+16:41:36.0  185.9910099 &   16.6933384 &    11.20 &  0.028 &    1210 &   -1.8 (  0.9) \\
     692 & NGC4351   & NGVSJ12:24:01.52+12:12:17.2  186.0063131 &   12.2047665 &    13.00 &  0.028 &    2325 &    2.8 (  1.7) \\
     698 & NGC4352   & NGVSJ12:24:05.03+11:13:05.1  186.0209443 &   11.2180718 &    13.60 &  0.026 &    2083 &   -2.0 (  0.4) \\
     731 & NGC4365   & NGVSJ12:24:28.26+07:19:04.0  186.1177300 &    7.3177697 &    10.50 &  0.021 &    1243 &   -4.8 (  0.4) \\
     750 & PGC040428 & NGVSJ12:24:49.57+06:45:34.4  186.2065252 &    6.7595615 &    14.80 &  0.028 &    1059 &   -5.0 (  1.0) \\
     759 & NGC4371   & NGVSJ12:24:55.43+11:42:15.1  186.2309734 &   11.7041966 &    11.80 &  0.036 &     933 &   -1.3 (  0.6) \\
     763 & NGC4374   & NGVSJ12:25:03.74+12:53:13.1  186.2656026 &   12.8869755 &    10.30 &  0.042 &    1017 &   -4.4 (  1.2) \\
     778 & NGC4377   & NGVSJ12:25:12.34+14:45:43.8  186.3014104 &   14.7621692 &    12.70 &  0.039 &    1338 &   -2.6 (  0.6) \\
     784 & NGC4379   & NGVSJ12:25:14.75+15:36:26.7  186.3114423 &   15.6074215 &    12.70 &  0.023 &    1074 &   -2.7 (  0.6) \\
     785 & NGC4378   & NGVSJ12:25:18.10+04:55:30.5  186.3254153 &    4.9251457 &    12.20 &  0.016 &    2559 &    1.0 (  0.3) \\
     792 & NGC4380   & NGVSJ12:25:22.17+10:01:00.5  186.3423910 &   10.0167929 &    12.40 &  0.024 &     963 &    2.4 (  0.9) \\
     801 & NGC4383   & NGVSJ12:25:25.46+16:28:11.8  186.3560921 &   16.4699454 &    12.70 &  0.024 &    1710 &    0.8 (  0.8) \\
     828 & NGC4387   & NGVSJ12:25:41.68+12:48:37.9  186.4236734 &   12.8105171 &    12.80 &  0.032 &     538 &   -4.8 (  0.6) \\
     836 & NGC4388   & NGVSJ12:25:46.72+12:39:42.9  186.4446712 &   12.6619044 &    11.80 &  0.033 &    2524 &    2.8 (  0.7) \\
     856 & IC3328    & NGVSJ12:25:57.92+10:03:13.6  186.4913357 &   10.0537778 &    14.20 &  0.024 &    1001 &   -3.8 (  1.7) \\
     865 & NGC4396   & NGVSJ12:25:59.15+15:40:13.6  186.4964753 &   15.6704560 &    13.00 &  0.026 &    -125 &    6.8 (  0.8) \\
     873 & NGC4402   & NGVSJ12:26:07.14+13:06:43.2  186.5297661 &   13.1119969 &    12.60 &  0.029 &     237 &    3.2 (  0.8) \\
     874 & NGC4405   & NGVSJ12:26:07.15+16:10:51.5  186.5298124 &   16.1809713 &    13.00 &  0.024 &    1735 &    0.3 (  1.1) \\
     881 & NGC4406   & NGVSJ12:26:11.76+12:56:46.5  186.5489811 &   12.9462404 &    10.10 &  0.029 &    -224 &   -4.8 (  0.5) \\
     896 & PGC040679 & NGVSJ12:26:22.61+12:47:11.0  186.5942075 &   12.7863945 &    17.70 &  0.030 &    2114 &   -5.0 (  1.2) \\
     898 & PGC040686 & NGVSJ12:26:23.64+13:22:24.7  186.5984901 &   13.3735172 &    18.30 &  0.030 &    1172 &   -5.0 (  3.0) \\
     912 & NGC4413   & NGVSJ12:26:32.25+12:36:38.5  186.6343910 &   12.6107082 &    12.40 &  0.032 &      69 &    2.1 (  1.1) \\
     916 & PGC040707 & NGVSJ12:26:33.21+12:44:34.7  186.6383646 &   12.7429799 &    15.60 &  0.030 &    1298 &   -5.0 (  1.2) \\
     928 & PGC040723 & NGVSJ12:26:39.81+12:30:48.8  186.6658930 &   12.5135530 &    15.90 &  0.032 &    -288 &   -5.0 (  1.0) \\
     929 & NGC4415   & NGVSJ12:26:40.49+08:26:08.5  186.6686939 &    8.4356972 &    13.10 &  0.022 &     907 &   -0.9 (  2.1) \\
     930 & PGC040725 & NGVSJ12:26:41.15+12:50:43.5  186.6714522 &   12.8454060 &    17.80 &  0.029 &    1172 &   -5.0 (  1.4) \\
     938 & NGC4416   & NGVSJ12:26:46.75+07:55:08.4  186.6947720 &    7.9189879 &    12.90 &  0.025 &    1399 &    5.9 (  0.5) \\
     939 & NGC4411B  & NGVSJ12:26:47.23+08:53:04.5  186.6968095 &    8.8845903 &    12.90 &  0.029 &    1272 &    6.2 (  0.9) \\
     940 & IC3349    & NGVSJ12:26:47.06+12:27:14.3  186.6961004 &   12.4539694 &    14.60 &  0.030 &    1392 &   -5.0 (  0.9) \\
     942 & PGC040753 & NGVSJ12:26:48.49+12:23:59.6  186.7020527 &   12.3998780 &    19.50 &  0.027 &    1172 &   -5.0 (  2.0) \\
     944 & NGC4417   & NGVSJ12:26:50.61+09:35:03.3  186.7108668 &    9.5842588 &    12.10 &  0.025 &     828 &   -1.9 (  0.5) \\
     950 & IC3356    & NGVSJ12:26:50.74+11:33:27.5  186.7114036 &   11.5576470 &    14.90 &  0.031 &    1100 &    9.7 (  1.0) \\
     951 & IC3358    & NGVSJ12:26:54.36+11:39:50.2  186.7265030 &   11.6639359 &    14.00 &  0.026 &    2106 &   -5.0 (  1.4) \\
     958 & NGC4419   & NGVSJ12:26:56.43+15:02:50.3  186.7351069 &   15.0473025 &    12.10 &  0.033 &    -261 &    1.2 (  0.9) \\
     962 & PGC040782 & NGVSJ12:26:59.05+12:30:20.5  186.7460570 &   12.5056882 &    16.90 &  0.028 &    1172 &   -5.0 (  2.0) \\
     965 & IC3363    & NGVSJ12:27:03.08+12:33:38.8  186.7628443 &   12.5607787 &    15.10 &  0.030 &     830 &   -5.0 (  1.0) \\
     966 & NGC4421   & NGVSJ12:27:02.54+15:27:41.3  186.7605852 &   15.4614659 &    12.40 &  0.024 &    1551 &   -0.5 (  0.8) \\
     967 & PGC040787 & NGVSJ12:27:03.81+12:51:59.2  186.7658563 &   12.8664417 &    18.20 &  0.029 &    1135 &   -5.0 (  1.2) \\
     968 & PGC040792 & NGVSJ12:27:06.07+13:19:25.3  186.7752955 &   13.3236918 &    18.00 &  0.026 &    1172 &   -5.0 (  3.0) \\
     972 & PGC040798 & NGVSJ12:27:08.42+13:20:08.7  186.7850718 &   13.3357445 &    16.40 &  0.025 &   14999 &   -5.0 (  2.0) \\
     977 & PGC040806 & NGVSJ12:27:11.24+12:02:17.4  186.7968529 &   12.0381804 &    17.70 &  0.025 &      57 &   -5.0 (  1.2) \\
     978 & PGC040805 & NGVSJ12:27:11.20+12:06:52.3  186.7966853 &   12.1145416 &    18.00 &  0.026 &    1172 &   -5.0 (  3.0) \\
     979 & NGC4424   & NGVSJ12:27:11.67+09:25:14.8  186.7986301 &    9.4207733 &    12.30 &  0.021 &     437 &    1.3 (  1.6) \\
     984 & NGC4425   & NGVSJ12:27:13.34+12:44:05.2  186.8055801 &   12.7347647 &    12.30 &  0.029 &    1892 &   -0.6 (  1.2) \\
     990 & IC3369    & NGVSJ12:27:16.94+16:01:28.1  186.8205856 &   16.0244642 &    14.30 &  0.029 &    1704 &   -3.3 (  1.9) \\
     996 & PGC040838 & NGVSJ12:27:21.11+13:06:40.3  186.8379500 &   13.1111947 &    17.80 &  0.029 &     -28 &   -5.0 (  1.2) \\
     997 & PGC040840 & NGVSJ12:27:22.17+12:04:07.4  186.8423851 &   12.0687121 &    17.40 &  0.026 &    -171 &   -5.0 (  1.2) \\
     998 & PGC040841 & NGVSJ12:27:23.46+12:19:54.1  186.8477404 &   12.3317052 &    17.50 &  0.029 & \nodata &   -5.0 (  2.0) \\
    1000 & PGC040846 & NGVSJ12:27:24.71+11:14:17.8  186.8529524 &   11.2382779 &    18.20 &  0.035 & \nodata &   -5.0 (  2.0) \\
    1003 & NGC4429   & NGVSJ12:27:26.52+11:06:27.7  186.8604863 &   11.1076843 &    11.20 &  0.033 &    1104 &   -0.8 (  1.5) \\
    1010 & NGC4431   & NGVSJ12:27:27.38+12:17:25.0  186.8640813 &   12.2902790 &    13.40 &  0.028 &     930 &   -2.1 (  0.7) \\
    1017 & PGC040869 & NGVSJ12:27:31.55+09:35:44.3  186.8814384 &    9.5956422 &    14.90 &  0.022 &      32 &    9.9 (  1.4) \\
    1020 & PGC040872 & NGVSJ12:27:32.01+11:36:54.7  186.8833845 &   11.6151815 &    17.00 &  0.025 &    1379 &   -3.5 (  2.1) \\
    1025 & NGC4434   & NGVSJ12:27:36.68+08:09:15.6  186.9028317 &    8.1543420 &    13.10 &  0.023 &    1070 &   -4.7 (  0.7) \\
    1027 & PGC040890 & NGVSJ12:27:39.24+12:52:47.6  186.9134916 &   12.8798909 &    17.20 &  0.028 &      77 &   -5.0 (  1.2) \\
    1030 & NGC4435   & NGVSJ12:27:40.49+13:04:44.3  186.9187168 &   13.0789836 &    11.80 &  0.029 &     791 &   -2.1 (  0.5) \\
    1035 & PGC040906 & NGVSJ12:27:42.11+12:05:22.7  186.9254486 &   12.0896455 &    15.80 &  0.028 &     146 &   -4.3 (  1.6) \\
    1036 & NGC4436   & NGVSJ12:27:41.24+12:18:57.2  186.9218156 &   12.3158886 &    13.60 &  0.027 &    1113 &   -1.8 (  0.9) \\
    1040 & PGC040913 & NGVSJ12:27:44.52+12:59:01.3  186.9355189 &   12.9836833 &    15.50 &  0.028 &    -143 &   -5.0 (  1.2) \\
    1043 & NGC4438   & NGVSJ12:27:45.65+13:00:31.9  186.9402024 &   13.0088742 &    10.50 &  0.028 &      71 &    0.6 (  1.5) \\
    1049 & UGC07580  & NGVSJ12:27:54.83+08:05:25.5  186.9784720 &    8.0904030 &    14.20 &  0.022 &     607 &   -4.2 (  2.0) \\
    1052 & PGC040932 & NGVSJ12:27:55.22+12:22:09.5  186.9800778 &   12.3692963 &    16.20 &  0.027 & \nodata &   -5.0 (  2.0) \\
    1059 & PGC040946 & NGVSJ12:28:00.44+11:56:59.6  187.0018514 &   11.9498934 &    17.80 &  0.026 &    2216 &   -5.0 (  1.2) \\
    1062 & NGC4442   & NGVSJ12:28:03.88+09:48:13.4  187.0161468 &    9.8037122 &    11.40 &  0.022 &     547 &   -1.9 (  0.4) \\
    1069 & PGC040958 & NGVSJ12:28:06.53+12:53:53.3  187.0272120 &   12.8981447 &    16.30 &  0.025 &    2326 &   -5.0 (  0.8) \\
    1073 & IC0794    & NGVSJ12:28:08.61+12:05:35.8  187.0358723 &   12.0932857 &    13.90 &  0.028 &    1921 &   -4.2 (  0.7) \\
    1075 & IC3383    & NGVSJ12:28:12.31+10:17:51.5  187.0513119 &   10.2976486 &    15.10 &  0.027 &    1808 &   -3.3 (  3.7) \\
    1076 & PGC040969 & NGVSJ12:28:12.84+10:31:33.7  187.0534826 &   10.5260342 &    16.80 &  0.029 &    1679 &   -5.0 (  1.4) \\
    1079 & PGC040972 & NGVSJ12:28:12.03+10:21:55.0  187.0501120 &   10.3652855 &    16.40 &  0.028 &    1354 &   -5.0 (  1.4) \\
    1087 & IC3381    & NGVSJ12:28:14.87+11:47:23.6  187.0619636 &   11.7898823 &    14.30 &  0.027 &     659 &   -4.1 (  0.8) \\
    1093 & PGC040995 & NGVSJ12:28:18.74+11:42:00.9  187.0780927 &   11.7002572 &    16.40 &  0.027 &    1476 &   -5.0 (  1.2) \\
    1100 & PGC041005 & NGVSJ12:28:23.37+11:34:46.9  187.0973594 &   11.5796867 &    17.90 &  0.028 & \nodata &   -5.0 (  3.0) \\
    1101 & PGC041007 & NGVSJ12:28:23.64+13:11:44.7  187.0985017 &   13.1957565 &    15.80 &  0.023 &    1670 &   -5.0 (  1.0) \\
    1104 & IC3388    & NGVSJ12:28:28.06+12:49:25.3  187.1169051 &   12.8236946 &    15.10 &  0.022 &    1707 &   -5.0 (  0.9) \\
    1110 & NGC4450   & NGVSJ12:28:29.59+17:05:06.1  187.1232946 &   17.0850198 &    10.90 &  0.028 &    1956 &    2.4 (  0.7) \\
    1115 & PGC041035 & NGVSJ12:28:32.40+11:44:40.7  187.1350073 &   11.7446286 &    17.00 &  0.030 &   30000 &   -5.0 (  2.0) \\
    1122 & IC3393    & NGVSJ12:28:41.71+12:54:57.2  187.1737961 &   12.9158877 &    14.50 &  0.020 &     465 &   -1.7 (  2.0) \\
    1123 & PGC041059 & NGVSJ12:28:42.66+12:32:59.4  187.1777602 &   12.5498411 &    16.40 &  0.022 &   30000 &   -5.0 (  1.2) \\
    1125 & NGC4452   & NGVSJ12:28:43.31+11:45:18.1  187.1804470 &   11.7550324 &    12.50 &  0.030 &     162 &   -1.9 (  0.8) \\
    1129 & PGC041068 & NGVSJ12:28:44.91+12:48:34.3  187.1871314 &   12.8095314 &    17.60 &  0.020 &      12 &   -5.0 (  1.2) \\
    1131 & PGC041071 & NGVSJ12:28:45.79+12:01:18.6  187.1907795 &   12.0218433 &    17.80 &  0.027 &    1172 &   -5.0 (  2.0) \\
    1136 & PGC041077 & NGVSJ12:28:49.11+12:07:54.5  187.2046093 &   12.1318006 &    18.00 &  0.027 &    1172 &   -5.0 (  3.0) \\
    1146 & NGC4458   & NGVSJ12:28:57.56+13:14:31.0  187.2398351 &   13.2419339 &    12.90 &  0.023 &     677 &   -4.9 (  0.4) \\
    1148 & PGC041098 & NGVSJ12:28:58.14+12:39:42.2  187.2422494 &   12.6617298 &    15.50 &  0.021 &    1417 &   -5.0 (  1.0) \\
    1149 & PGC041097 & NGVSJ12:28:58.84+12:54:28.8  187.2451828 &   12.9079984 &    17.40 &  0.020 &    1172 &   -5.0 (  1.4) \\
    1153 & PGC041102 & NGVSJ12:28:59.82+12:38:54.2  187.2492426 &   12.6483894 &    17.20 &  0.021 &   30000 &   10.0 (  2.0) \\
    1154 & NGC4459   & NGVSJ12:29:00.04+13:58:42.5  187.2501631 &   13.9784745 &    11.40 &  0.045 &    1192 &   -1.6 (  1.1) \\
    1158 & NGC4461   & NGVSJ12:29:03.01+13:11:01.7  187.2625503 &   13.1838010 &    11.50 &  0.023 &    1924 &   -0.7 (  1.3) \\
    1173 & PGC041136 & NGVSJ12:29:14.85+12:58:41.7  187.3118929 &   12.9782469 &    15.90 &  0.020 &    2416 &   -5.0 (  1.0) \\
    1177 & PGC041146 & NGVSJ12:29:19.28+12:22:37.2  187.3303288 &   12.3770123 &    18.20 &  0.023 &    1172 &   -5.0 (  3.0) \\
    1178 & NGC4464   & NGVSJ12:29:21.29+08:09:23.8  187.3387258 &    8.1566225 &    13.40 &  0.022 &    1243 &   -2.7 (  3.4) \\
    1185 & PGC041156 & NGVSJ12:29:23.52+12:27:02.9  187.3479850 &   12.4508043 &    15.70 &  0.023 &     448 &   -5.0 (  1.0) \\
    1190 & NGC4469   & NGVSJ12:29:28.03+08:44:59.3  187.3667933 &    8.7498027 &    12.20 &  0.020 &     588 &    0.3 (  0.7) \\
    1191 & PGC041167 & NGVSJ12:29:28.67+12:29:46.3  187.3694547 &   12.4962070 &    17.40 &  0.022 &       5 &   -5.0 (  1.2) \\
    1192 & NGC4467   & NGVSJ12:29:30.25+07:59:34.3  187.3760471 &    7.9928597 &    15.00 &  0.023 &    1390 &   -4.8 (  0.7) \\
    1199 & PGC041180 & NGVSJ12:29:34.99+08:03:28.8  187.3958061 &    8.0580083 &    15.50 &  0.022 &    1392 &   -5.0 (  1.2) \\
    1205 & NGC4470   & NGVSJ12:29:37.82+07:49:24.1  187.4075732 &    7.8233726 &    13.00 &  0.024 &    2340 &    1.9 (  2.1) \\
    1212 & PGC041197 & NGVSJ12:29:39.06+11:38:00.3  187.4127358 &   11.6334149 &    16.70 &  0.036 & \nodata &   -5.0 (  2.0) \\
    1213 & PGC041195 & NGVSJ12:29:39.24+12:32:53.7  187.4135137 &   12.5482441 &    16.10 &  0.022 &    1092 &   -5.0 (  1.2) \\
    1216 & PGC041203 & NGVSJ12:29:41.28+12:02:45.9  187.4220147 &   12.0460966 &    18.20 &  0.028 &    1172 &   -5.0 (  2.0) \\
    1219 & PGC041209 & NGVSJ12:29:44.09+12:48:19.6  187.4337238 &   12.8054536 &    18.00 &  0.020 &   30000 &   -5.0 (  1.2) \\
    1226 & NGC4472   & NGVSJ12:29:46.77+08:00:01.8  187.4448543 &    8.0004899 &     9.30 &  0.022 &     981 &   -4.8 (  0.5) \\
    1231 & NGC4473   & NGVSJ12:29:48.87+13:25:46.0  187.4536246 &   13.4294361 &    11.10 &  0.028 &    2244 &   -4.7 (  0.7) \\
    1239 & PGC041238 & NGVSJ12:29:53.00+11:57:44.3  187.4708241 &   11.9622933 &    16.80 &  0.029 &    -400 &   -5.0 (  1.4) \\
    1242 & NGC4474   & NGVSJ12:29:53.55+14:04:06.9  187.4731182 &   14.0685841 &    12.60 &  0.041 &    1611 &   -1.9 (  0.9) \\
    1244 & PGC041245 & NGVSJ12:29:56.34+13:13:12.3  187.4847568 &   13.2200747 &    18.00 &  0.024 &    1172 &   -5.0 (  3.0) \\
    1250 & NGC4476   & NGVSJ12:29:59.08+12:20:55.4  187.4961534 &   12.3487189 &    12.90 &  0.027 &    1959 &   -2.9 (  1.0) \\
    1253 & NGC4477   & NGVSJ12:30:02.20+13:38:11.5  187.5091719 &   13.6365327 &    11.30 &  0.032 &    1338 &   -1.7 (  0.7) \\
    1259 & PGC041268 & NGVSJ12:30:06.08+12:22:37.9  187.5253517 &   12.3772044 &    17.80 &  0.028 &    1172 &   -5.0 (  2.0) \\
    1261 & NGC4482   & NGVSJ12:30:10.33+10:46:46.2  187.5430470 &   10.7794918 &    13.60 &  0.029 &    1825 &   -4.8 (  0.6) \\
    1264 & PGC041273 & NGVSJ12:30:10.88+12:11:43.6  187.5453319 &   12.1954334 &    16.40 &  0.025 &   30000 &   -5.0 (  1.2) \\
    1279 & NGC4478   & NGVSJ12:30:17.42+12:19:42.8  187.5725711 &   12.3285593 &    12.20 &  0.023 &    1349 &   -4.9 (  0.4) \\
    1283 & NGC4479   & NGVSJ12:30:18.38+13:34:39.5  187.5765820 &   13.5776497 &    13.40 &  0.029 &     848 &   -1.9 (  0.5) \\
    1289 & PGC041313 & NGVSJ12:30:24.48+13:19:55.8  187.6019909 &   13.3321702 &    18.00 &  0.026 & \nodata &   -5.0 (  2.0) \\
    1297 & NGC4486B  & NGVSJ12:30:31.97+12:29:24.6  187.6332079 &   12.4901631 &    14.30 &  0.021 &    1555 &   -5.0 (  0.8) \\
    1298 & PGC041329 & NGVSJ12:30:33.32+12:54:02.3  187.6388495 &   12.9006515 &    17.80 &  0.020 &    1172 &   -5.0 (  2.0) \\
    1300 & PGC041331 & NGVSJ12:30:34.65+12:27:29.2  187.6443597 &   12.4581190 &    17.40 &  0.021 &    1172 &   -5.0 (  3.0) \\
    1303 & NGC4483   & NGVSJ12:30:40.64+09:00:56.4  187.6693449 &    9.0156724 &    13.10 &  0.020 &     884 &   -1.4 (  0.7) \\
    1308 & IC3437    & NGVSJ12:30:45.91+11:20:35.5  187.6912832 &   11.3431951 &    15.20 &  0.035 &    1739 &   -5.0 (  1.0) \\
    1314 & PGC041358 & NGVSJ12:30:49.03+13:13:25.8  187.7043010 &   13.2238351 &    16.70 &  0.025 &      35 &    0.2 (  6.9) \\
    1316 & NGC4486   & NGVSJ12:30:49.42+12:23:28.0  187.7059365 &   12.3911224 &     9.60 &  0.023 &    1284 &   -4.3 (  0.6) \\
    1317 & PGC041362 & NGVSJ12:30:50.59+12:44:11.7  187.7107846 &   12.7365860 &    17.80 &  0.023 &    1172 &   -5.0 (  2.0) \\
    1318 & NGC4488   & NGVSJ12:30:51.37+08:21:36.0  187.7140590 &    8.3600070 &    12.90 &  0.021 &     980 &   -0.1 (  0.6) \\
    1321 & NGC4489   & NGVSJ12:30:52.25+16:45:31.8  187.7177136 &   16.7588428 &    12.80 &  0.027 &     940 &   -4.7 (  0.9) \\
    1324 & PGC041375 & NGVSJ12:30:55.66+13:20:53.8  187.7319358 &   13.3482714 &    17.90 &  0.025 &   30000 &   -5.0 (  2.0) \\
    1327 & NGC4486A  & NGVSJ12:30:57.77+12:16:15.5  187.7407131 &   12.2709806 &    13.30 &  0.023 &     758 &   -5.0 (  0.4) \\
    1331 & PGC041384 & NGVSJ12:30:58.81+11:42:30.8  187.7450512 &   11.7085529 &    17.40 &  0.031 & \nodata &   -5.0 (  2.0) \\
    1336 & PGC041398 & NGVSJ12:31:03.98+11:50:10.2  187.7665675 &   11.8361640 &    17.40 &  0.028 & \nodata &   -5.0 (  3.0) \\
    1340 & PGC041411 & NGVSJ12:31:10.42+13:05:50.5  187.7934070 &   13.0973532 &    17.90 &  0.023 &    1540 &   -5.0 (  1.4) \\
    1341 & PGC041414 & NGVSJ12:31:11.64+13:06:51.7  187.7984812 &   13.1143508 &    18.00 &  0.024 & \nodata &   -5.0 (  2.0) \\
    1343 & PGC041416 & NGVSJ12:31:12.69+13:07:27.4  187.8028829 &   13.1242729 &    18.00 &  0.024 &    1900 &   -5.0 (  1.4) \\
    1348 & IC3443    & NGVSJ12:31:15.73+12:19:54.4  187.8155531 &   12.3317700 &    15.20 &  0.022 &    1019 &   -5.0 (  1.2) \\
    1352 & PGC041433 & NGVSJ12:31:19.57+12:36:41.5  187.8315239 &   12.6115153 &    17.00 &  0.022 &    1766 &   -4.0 (  1.8) \\
    1353 & PGC041432 & NGVSJ12:31:19.43+12:44:16.9  187.8309531 &   12.7380408 &    16.10 &  0.024 &    -380 &   -4.4 (  1.5) \\
    1355 & IC3442    & NGVSJ12:31:20.20+14:06:54.6  187.8341502 &   14.1151537 &    14.30 &  0.035 &    1245 &   -5.0 (  0.4) \\
    1366 & PGC041454 & NGVSJ12:31:31.68+11:36:11.1  187.8820201 &   11.6030707 &    17.10 &  0.047 &   30000 &   -5.0 (  1.4) \\
    1368 & NGC4497   & NGVSJ12:31:32.54+11:37:29.1  187.8855752 &   11.6247460 &    12.70 &  0.042 &    1042 &   -1.1 (  1.1) \\
    1369 & PGC041458 & NGVSJ12:31:33.35+12:03:49.7  187.8889577 &   12.0638064 &    16.50 &  0.029 &     797 &   -4.3 (  1.6) \\
    1379 & NGC4498   & NGVSJ12:31:39.43+16:51:10.5  187.9142868 &   16.8529154 &    12.60 &  0.029 &    1507 &    6.4 (  0.9) \\
    1386 & IC3457    & NGVSJ12:31:51.33+12:39:25.2  187.9638828 &   12.6569935 &    14.40 &  0.026 &    1297 &   -4.7 (  1.7) \\
    1389 & PGC041495 & NGVSJ12:31:52.01+12:28:54.5  187.9667127 &   12.4818113 &    15.80 &  0.025 &     877 &   -5.0 (  1.2) \\
    1392 & IC3459    & NGVSJ12:31:55.93+12:10:27.0  187.9830351 &   12.1741628 &    14.60 &  0.027 &     385 &    9.8 (  0.5) \\
    1396 & PGC041508 & NGVSJ12:31:56.40+11:58:21.7  187.9849804 &   11.9726948 &    17.00 &  0.029 &    1094 &   -5.0 (  2.0) \\
    1399 & PGC041516 & NGVSJ12:32:00.75+12:37:13.2  188.0031452 &   12.6203250 &    16.50 &  0.026 &     493 &   -5.0 (  1.2) \\
    1407 & IC3461    & NGVSJ12:32:02.74+11:53:24.3  188.0114114 &   11.8900782 &    15.50 &  0.033 &    1007 &   -5.0 (  0.9) \\
    1411 & IC3466    & NGVSJ12:32:05.63+11:49:03.6  188.0234745 &   11.8176581 &    15.40 &  0.033 &     909 &   10.0 (  1.4) \\
    1412 & NGC4503   & NGVSJ12:32:06.23+11:10:35.0  188.0259744 &   11.1763897 &    12.10 &  0.051 &    1334 &   -1.7 (  1.8) \\
    1414 & PGC041541 & NGVSJ12:32:09.31+12:50:20.2  188.0388115 &   12.8389402 &    16.80 &  0.024 &     192 &   -5.0 (  1.0) \\
    1417 & PGC041544 & NGVSJ12:32:09.58+15:18:03.3  188.0399339 &   15.3009169 &    15.80 &  0.031 &    1577 &   -5.0 (  1.4) \\
    1418 & PGC041545 & NGVSJ12:32:11.36+12:30:24.9  188.0473303 &   12.5069279 &    17.10 &  0.028 &   30000 &   -5.0 (  3.0) \\
    1419 & NGC4506   & NGVSJ12:32:10.50+13:25:09.7  188.0437355 &   13.4193556 &    13.20 &  0.028 &     561 &    1.1 (  0.9) \\
    1420 & IC3465    & NGVSJ12:32:12.24+12:03:41.5  188.0510100 &   12.0615256 &    16.10 &  0.029 &     985 &   -4.3 (  1.6) \\
    1422 & IC3468    & NGVSJ12:32:14.22+10:15:05.3  188.0592337 &   10.2514606 &    13.60 &  0.032 &    1300 &   -4.8 (  0.6) \\
    1426 & PGC041570 & NGVSJ12:32:23.58+11:53:36.1  188.0982667 &   11.8933691 &    15.40 &  0.033 &     833 &   10.0 (  2.0) \\
    1431 & IC3470    & NGVSJ12:32:23.38+11:15:46.7  188.0974316 &   11.2629600 &    14.50 &  0.051 &    1489 &   -4.8 (  0.9) \\
    1438 & PGC041588 & NGVSJ12:32:34.71+12:38:21.1  188.1446063 &   12.6391986 &    17.40 &  0.026 &    1172 &   -5.0 (  3.0) \\
    1440 & IC0798    & NGVSJ12:32:33.41+15:24:55.4  188.1391948 &   15.4153952 &    15.20 &  0.028 &     429 &   -5.0 (  1.2) \\
    1448 & IC3475    & NGVSJ12:32:40.80+12:46:15.9  188.1700092 &   12.7710848 &    13.70 &  0.026 &    2583 &   -4.6 (  1.9) \\
    1449 & PGC041604 & NGVSJ12:32:39.13+13:19:47.5  188.1630433 &   13.3298656 &    17.60 &  0.026 & \nodata &   -5.0 (  2.0) \\
    1463 & PGC041637 & NGVSJ12:32:54.11+12:48:27.2  188.2254464 &   12.8075653 &    18.20 &  0.028 & \nodata &   -5.0 (  2.0) \\
    1475 & NGC4515   & NGVSJ12:33:04.97+16:15:55.9  188.2707092 &   16.2655230 &    13.40 &  0.031 &     955 &   -3.2 (  0.7) \\
    1488 & IC3487    & NGVSJ12:33:13.43+09:23:50.4  188.3059683 &    9.3973326 &    14.80 &  0.021 &    1074 &   -3.5 (  2.1) \\
    1489 & IC3490    & NGVSJ12:33:13.91+10:55:42.9  188.3079662 &   10.9285760 &    15.90 &  0.032 &     268 &   -5.0 (  1.2) \\
    1491 & IC3486    & NGVSJ12:33:14.01+12:51:28.2  188.3083811 &   12.8578220 &    14.70 &  0.031 &    1986 &   -3.6 (  2.0) \\
    1499 & IC3492    & NGVSJ12:33:19.79+12:51:12.5  188.3324580 &   12.8534644 &    14.80 &  0.030 &    -541 &   -3.8 (  1.6) \\
    1509 & PGC041720 & NGVSJ12:33:31.65+09:27:33.2  188.3818570 &    9.4592142 &    16.30 &  0.023 &     808 &   -5.0 (  1.4) \\
    1512 & PGC041723 & NGVSJ12:33:34.65+11:15:43.0  188.3943603 &   11.2619480 &    15.70 &  0.051 &     839 &   -3.0 (  1.8) \\
    1514 & PGC041726 & NGVSJ12:33:37.70+07:52:15.8  188.4070872 &    7.8710636 &    15.00 &  0.020 &     538 &   -4.3 (  1.6) \\
    1516 & NGC4522   & NGVSJ12:33:39.71+09:10:30.1  188.4154727 &    9.1750335 &    12.70 &  0.021 &    2329 &    5.9 (  0.6) \\
    1522 & PGC041740 & NGVSJ12:33:47.06+11:46:53.8  188.4460735 &   11.7816189 &    17.90 &  0.041 & \nodata &   -5.0 (  2.0) \\
    1523 & PGC041744 & NGVSJ12:33:48.67+12:46:48.1  188.4528030 &   12.7800364 &    17.30 &  0.030 &    1108 &   -5.0 (  1.4) \\
    1528 & IC3501    & NGVSJ12:33:51.62+13:19:20.9  188.4650793 &   13.3224639 &    14.50 &  0.028 &    1615 &   -4.4 (  1.5) \\
    1535 & NGC4526   & NGVSJ12:34:02.98+07:41:57.5  188.5124331 &    7.6993100 &    10.00 &  0.022 &     617 &   -1.9 (  0.4) \\
    1536 & PGC041775 & NGVSJ12:34:06.56+11:50:12.1  188.5273235 &   11.8367030 &    17.90 &  0.038 & \nodata &   -5.0 (  2.0) \\
    1537 & NGC4528   & NGVSJ12:34:06.08+11:19:16.5  188.5253210 &   11.3212533 &    12.70 &  0.046 &    1378 &   -2.0 (  0.5) \\
    1539 & PGC041782 & NGVSJ12:34:06.74+12:44:29.7  188.5280977 &   12.7415714 &    15.70 &  0.032 &    1508 &   -5.0 (  1.0) \\
    1545 & IC3509    & NGVSJ12:34:11.53+12:02:56.3  188.5480615 &   12.0489659 &    15.00 &  0.041 &    2065 &   -5.0 (  1.0) \\
    1552 & NGC4531   & NGVSJ12:34:15.88+13:04:31.1  188.5661639 &   13.0753139 &    12.60 &  0.043 &      90 &   -0.1 (  2.4) \\
    1561 & PGC041818 & NGVSJ12:34:25.05+12:54:12.8  188.6043594 &   12.9035629 &    15.50 &  0.032 &    -582 &   -5.0 (  3.0) \\
    1563 & PGC041822 & NGVSJ12:34:26.05+11:55:01.4  188.6085262 &   11.9170464 &    16.10 &  0.039 &    2249 &   -5.0 (  1.4) \\
    1588 & NGC4540   & NGVSJ12:34:50.85+15:33:05.9  188.7118891 &   15.5516418 &    12.50 &  0.035 &    1291 &    6.2 (  0.9) \\
    1615 & NGC4548   & NGVSJ12:35:26.46+14:29:46.9  188.8602505 &   14.4963502 &    11.00 &  0.038 &     486 &    3.1 (  0.5) \\
    1619 & NGC4550   & NGVSJ12:35:30.58+12:13:14.7  188.8774282 &   12.2207530 &    12.50 &  0.040 &     459 &   -2.0 (  0.7) \\
    1627 & PGC041959 & NGVSJ12:35:37.25+12:22:55.4  188.9052169 &   12.3820489 &    15.20 &  0.038 &     282 &   -5.0 (  0.9) \\
    1630 & NGC4551   & NGVSJ12:35:37.95+12:15:50.4  188.9081312 &   12.2639882 &    12.90 &  0.039 &    1176 &   -4.9 (  0.4) \\
    1632 & NGC4552   & NGVSJ12:35:39.81+12:33:22.9  188.9158835 &   12.5563645 &    10.80 &  0.041 &     340 &   -4.6 (  0.9) \\
    1661 & PGC042046 & NGVSJ12:36:24.78+10:23:04.8  189.1032517 &   10.3846789 &    16.00 &  0.020 &    1419 &   -5.0 (  1.2) \\
    1664 & NGC4564   & NGVSJ12:36:26.98+11:26:21.2  189.1124336 &   11.4392282 &    12.00 &  0.034 &    1142 &   -4.6 (  0.7) \\
    1690 & NGC4569   & NGVSJ12:36:49.86+13:09:46.7  189.2077334 &   13.1629785 &    10.20 &  0.046 &    -235 &    2.4 (  0.7) \\
    1692 & NGC4570   & NGVSJ12:36:53.38+07:14:47.7  189.2224185 &    7.2465803 &    11.80 &  0.022 &    1787 &   -1.9 (  1.0) \\
    1695 & IC3586    & NGVSJ12:36:54.86+12:31:12.5  189.2285916 &   12.5201265 &    14.50 &  0.045 &    1717 &   -3.0 (  1.8) \\
    1696 & NGC4571   & NGVSJ12:36:56.39+14:13:02.4  189.2349379 &   14.2173437 &    11.80 &  0.046 &     332 &    6.4 (  0.8) \\
    1720 & NGC4578   & NGVSJ12:37:30.56+09:33:18.4  189.3773344 &    9.5550995 &    12.30 &  0.020 &    2292 &   -2.1 (  0.6) \\
    1727 & NGC4579   & NGVSJ12:37:43.53+11:49:05.5  189.4313892 &   11.8182052 &    10.60 &  0.041 &    1517 &    2.8 (  0.6) \\
    1730 & NGC4580   & NGVSJ12:37:48.39+05:22:06.7  189.4516186 &    5.3685208 &    12.60 &  0.024 &    1035 &    1.6 (  0.7) \\
    1743 & IC3602    & NGVSJ12:38:06.79+10:04:56.6  189.5282773 &   10.0823858 &    15.50 &  0.019 &    1279 &   -3.0 (  1.8) \\
    1779 & IC3612    & NGVSJ12:39:04.69+14:43:51.9  189.7695433 &   14.7310745 &    14.80 &  0.027 &    1251 &   -1.7 (  1.2) \\
    1809 & IC3631    & NGVSJ12:39:48.01+12:58:26.2  189.9500562 &   12.9739543 &    13.80 &  0.037 &    2828 &   -1.2 (  1.7) \\
    1811 & NGC4595   & NGVSJ12:39:51.91+15:17:52.0  189.9663104 &   15.2977805 &    12.90 &  0.037 &     631 &    4.0 (  1.9) \\
    1813 & NGC4596   & NGVSJ12:39:55.96+10:10:34.1  189.9831538 &   10.1761470 &    11.50 &  0.021 &    1892 &   -0.8 (  0.8) \\
    1826 & IC3633    & NGVSJ12:40:11.25+09:53:46.0  190.0468834 &    9.8961198 &    15.70 &  0.017 &    1973 &   -5.0 (  1.2) \\
    1828 & IC3635    & NGVSJ12:40:13.39+12:52:29.2  190.0557887 &   12.8747695 &    15.30 &  0.037 &    1560 &    4.3 (  4.0) \\
    1833 & PGC042442 & NGVSJ12:40:19.68+15:56:07.0  190.0820095 &   15.9352811 &    14.50 &  0.036 &    1705 &   -2.7 (  1.8) \\
    1851 & PGC042487 & NGVSJ12:40:43.60+10:24:28.1  190.1816754 &   10.4078114 &    18.00 &  0.023 & \nodata &   -5.0 (  3.0) \\
    1857 & IC3647    & NGVSJ12:40:53.12+10:28:32.2  190.2213279 &   10.4756088 &    14.10 &  0.025 &     634 &    9.8 (  0.5) \\
    1859 & NGC4606   & NGVSJ12:40:57.55+11:54:43.8  190.2398109 &   11.9121733 &    12.70 &  0.032 &    1649 &    0.6 (  1.4) \\
    1861 & IC3652    & NGVSJ12:40:58.56+11:11:04.2  190.2439935 &   11.1844975 &    14.40 &  0.030 &     630 &   -4.8 (  0.6) \\
    1869 & NGC4608   & NGVSJ12:41:13.29+10:09:20.3  190.3053852 &   10.1556511 &    12.10 &  0.017 &    1850 &   -1.7 (  0.8) \\
    1870 & PGC042547 & NGVSJ12:41:15.35+11:17:54.5  190.3139453 &   11.2984787 &    15.80 &  0.028 &    1652 &   -5.0 (  1.4) \\
    1871 & IC3653    & NGVSJ12:41:15.73+11:23:14.1  190.3155405 &   11.3872469 &    13.90 &  0.031 &     557 &   -5.0 (  1.0) \\
    1879 & PGC042566 & NGVSJ12:41:27.39+11:08:45.0  190.3641447 &   11.1458370 &    16.80 &  0.029 &    1070 &   -5.0 (  3.0) \\
    1883 & NGC4612   & NGVSJ12:41:32.75+07:18:53.6  190.3864549 &    7.3148793 &    12.60 &  0.025 &    1775 &   -2.0 (  0.4) \\
    1886 & PGC042586 & NGVSJ12:41:39.41+12:14:50.9  190.4142274 &   12.2474618 &    15.50 &  0.033 &     927 &   -5.0 (  1.4) \\
    1895 & UGC07854  & NGVSJ12:41:51.97+09:24:10.6  190.4665489 &    9.4029504 &    14.90 &  0.017 &     970 &   -3.0 (  1.8) \\
    1903 & NGC4621   & NGVSJ12:42:02.26+11:38:49.0  190.5094276 &   11.6469455 &    10.80 &  0.033 &     467 &   -4.8 (  0.4) \\
    1910 & IC0809    & NGVSJ12:42:08.67+11:45:15.4  190.5361351 &   11.7542664 &    14.20 &  0.032 &     196 &   -4.9 (  0.4) \\
    1938 & NGC4638   & NGVSJ12:42:47.43+11:26:33.0  190.6976235 &   11.4425074 &    12.10 &  0.025 &    1152 &   -2.6 (  0.7) \\
    1943 & NGC4639   & NGVSJ12:42:52.37+13:15:26.5  190.7182196 &   13.2573609 &    12.20 &  0.026 &    1018 &    3.6 (  0.7) \\
    1948 & PGC042754 & NGVSJ12:42:58.06+10:40:55.1  190.7418971 &   10.6819602 &    15.10 &  0.025 &    1610 &   -5.0 (  1.2) \\
    1978 & NGC4649   & NGVSJ12:43:39.97+11:33:09.7  190.9165323 &   11.5527000 &     9.80 &  0.026 &    1110 &   -4.6 (  0.9) \\
    1987 & NGC4654   & NGVSJ12:43:56.58+13:07:36.2  190.9857679 &   13.1267090 &    11.10 &  0.026 &    1036 &    5.9 (  0.5) \\
    1993 & PGC042884 & NGVSJ12:44:12.02+12:56:30.6  191.0501035 &   12.9418399 &    15.30 &  0.025 &     847 &   -4.0 (  1.8) \\
    1999 & NGC4659   & NGVSJ12:44:29.40+13:29:54.8  191.1224887 &   13.4985566 &    13.10 &  0.026 &     469 &   -0.1 (  0.6) \\
    2000 & NGC4660   & NGVSJ12:44:31.98+11:11:25.8  191.1332587 &   11.1905008 &    11.90 &  0.034 &    1083 &   -4.6 (  0.7) \\
    2019 & IC3735    & NGVSJ12:45:20.42+13:41:33.6  191.3350829 &   13.6926720 &    14.60 &  0.022 &    1819 &   -3.9 (  1.7) \\
    2048 & IC3773    & NGVSJ12:47:15.30+10:12:13.1  191.8137560 &   10.2036290 &    13.60 &  0.032 &    1086 &   -4.5 (  1.1) \\
    2050 & IC3779    & NGVSJ12:47:20.64+12:09:59.2  191.8359814 &   12.1664348 &    15.20 &  0.023 &    1165 &   -4.0 (  1.8) \\
    2058 & NGC4689   & NGVSJ12:47:45.56+13:45:46.1  191.9398462 &   13.7628078 &    11.60 &  0.023 &    1604 &    4.7 (  0.9) \\
    2066 & NGC4694   & NGVSJ12:48:15.12+10:58:59.8  192.0630072 &   10.9832842 &    12.20 &  0.039 &    1160 &   -1.8 (  0.7) \\
    2087 & NGC4733   & NGVSJ12:51:06.78+10:54:43.5  192.7782371 &   10.9120966 &    12.20 &  0.019 &     925 &   -3.6 (  1.3) \\
    2092 & NGC4754   & NGVSJ12:52:17.50+11:18:49.9  193.0729000 &   11.3138628 &    11.50 &  0.030 &    1351 &   -2.4 (  1.1) \\
    2095 & NGC4762   & NGVSJ12:52:55.97+11:13:51.5  193.2332268 &   11.2309755 &    10.80 &  0.023 &     986 &   -1.8 (  0.9) \\
 \nodata    &\nodata      & NGVSJ12:31:52.90+12:15:59.1  187.9703966 &   12.2664053 &    17.80 &  0.025 & \nodata & \nodata (\nodata) \\
 \nodata    &\nodata      & NGVSJ12:29:33.61+13:11:44.6  187.3900510 &   13.1957155 &    18.10 &  0.024 & \nodata & \nodata (\nodata) \\
 \nodata    &\nodata      & NGVSJ12:33:40.31+12:44:13.6  188.4179553 &   12.7371155 &    18.30 &  0.029 & \nodata & \nodata (\nodata) \\
\\
\enddata
\end{deluxetable}
\label{tab_all}
\tablecomments{This table is available in its entirety in a machine-readable form in the online journal. A portion is shown here for guidance regarding its form and content. All magnitudes are in $AB$ mag.}



